Cluster-Based Social Reinforcement Learning

Social Reinforcement Learning methods, which model agents in large networks, are useful for fake news mitigation, personalized teaching/healthcare, and viral marketing, but it is challenging to incorporate inter-agent dependencies into the models effectively due to network size and sparse interaction data. Previous social RL approaches either ignore agents dependencies or model them in a computationally intensive manner. In this work, we incorporate agent dependencies efficiently in a compact model by clustering users (based on their payoff and contribution to the goal) and combine this with a method to easily derive personalized agent-level policies from cluster-level policies. We also propose a dynamic clustering approach that captures changing user behavior. Experiments on real-world datasets illustrate that our proposed approach learns more accurate policy estimates and converges more quickly, compared to several baselines that do not use agent correlations or only use static clusters.

==> ARXIV_Dynamic Cluster-based Policy Learning for Social RL/01-abstract.tex <==
\textit{Social Reinforcement Learning} methods, which model agents in large networks, % with large numbers of agents, %and relatively few interactions between them 
are useful for fake news mitigation, personalized teaching/healthcare, and viral marketing, but it is challenging to incorporate %higher-order 
inter-agent \textit{dependencies} into the models effectively due to network size and sparse interaction data.
%It is thus, challenging due to \textit{high-dimensional search space}, and \textit{sparse} agent interactions, 
%and inter-agent dependencies, 
%resulting in high computational complexity, and insufficient data to capture higher-order inter-agent \textit{dependencies}. %Traditional approaches do not scale for large number of agents, and 
Previous social RL approaches either ignore agents dependencies 
%, resulting in inaccurate estimates, 
or model them in a computationally intensive manner. % using insufficient information, leading to increased variance. 
%To overcome these challenges, we present a \textit{Dynamic Cluster-based Social RL} approach that utilizes the properties of the social network structure, agent interactions and correlations to obtain a compact model to represent the network dynamics. 
In this work, we %develop an efficient approach to 
incorporate agent dependencies efficiently in a compact model by 
clustering users (based on their \textit{payoff} and \textit{contribution} to the goal) and combine this with a method to easily derive personalized agent-level \textit{policies} from cluster-level policies. %
%It is important to update the cluster dynamically along with policy learning, and thus, we propose 
%Since agent interactions are dynamic, 
We also propose a dynamic clustering approach that captures changing user behavior. %, we propose a \textit{Dynamic Cluster-based Social RL} approach that addresses the problem of cluster alignment at different times.
%Our method utilizes properties of the social network structure, agent interactions, and correlations to obtain a compact model to represent the network dynamics that can efficiently capture agent dependencies. 
%learn a cluster-based intervention policy (from which individual interventions can be easily derived).
%We evaluate our approach %with an application of Fake News Mitigation. 
%using real-world datasets. 
Experiments on real-world datasets 
%Results demonstrate 
illustrate that our proposed approach learns more accurate policy estimates and converges more quickly,  
%and achieves 
%faster convergence, 
compared to several baselines that do not use agent correlations or only use static clusters. 


%\mahak{Mention in comments when uploading on arxiv? -- ``Comments: submitted to IJCAI 2020"}


 



==> ARXIV_Dynamic Cluster-based Policy Learning for Social RL/02-introduction.tex <==
\section{INTRODUCTION} \label{intro}

Much of the existing work on multi-agent reinforcement learning (MARL) focuses on small number of agents. 
However, there are various applications that involve large number of interacting agents, for e.g., %social networks, urban system optimization problems like 
fleet management systems \cite{dejax1987survey}, urban transportation system consisting of a large number of vehicles, online advertising bidding agents \cite{wang2017display}, social networks with thousands of users who interact with each other (\cite{farajtabar2017fake, goindanisocial, upadhyay2018deep}). Thus, it is important to consider multi-agent systems with large number of interacting agents. 
%
Real-world social networks consist of thousands of users who interact with each other 
and are related in various ways (eg. \cite{farajtabar2017fake}). There is an opportunity to %use the relationship and/or similarity between the users in order to share information between them. 
%We take inspiration from relational RL and 
use the social network structure, which characterizes the relations and correlation between agents, to develop RL approaches that can scale for large number of agents. However, each user typically only interacts with a small number of other users in the network. This means the network interactions are overall sparse. 

We define \textit{Social Reinforcement Learning} as a sub-class of Multi-Agent Reinforcement Learning (MARL) for domains with large number of agents with relatively few (sparse) relations and interactions between them.
%
\iffalse
{\em Social reinforcement} refers to the process where acceptance and praise from others reinforces behaviors/preferences of an individual (eg. \cite{jones2011behavioral}). With the increased use of social media, response from peers plays an important role in shaping the behavior and decision-making of individuals (eg. \cite{lee2015understanding}) \cite{goindanisocial}.
%policy learning for individual agents is challenging in social networks 
\fi
%
The objective is to learn a \textit{policy} $\pi$ that maps the network \textit{state} (over $N$ users) to \textit{actions} (over $N$ users). 
%Real-world social networks consist of thousands of users who 
In a real-world social network, users
interact with each other, which  
%are related in various ways %(e.g. \cite{farajtabar2017fake}). 
%Traditional MARL approaches do not scale for large numbers of agents \cite{goindani2020social}.
leads to \textit{dependencies} between their \textit{actions} (due to peer-influence). For example, if one user tweets more, that may influence their followers to tweet more as well.
It is important to capture inter-agent dependencies
%dependencies between agents actions' 
to learn accurate policies for social RL systems \cite{goindanisocial2020_workshop}. Thus, to learn the policy for a single user, we need to consider the actions of all $N$ users, resulting in at least $N^2$ parameters to learn $N$ user policies with $N$ actions per policy. 
%\mahak{use O or $\Omega$ or $\sim$?. Remark from reviews: Using the O notation, a sparse network is a dense network too. And using $\Omega$, a dense network is also a sparse network.}
However, at the same time social networks are typically \textit{sparse} where agents only interact with a constant number of other agents, i.e., $O(N)$ interactions, as opposed to dense networks where all agents interact, i.e., $\Omega(N^2)$ interactions. 
Therefore, learning accurate policies, given $O(N)$ (sparse) interactions, is difficult since there are insufficient observations to capture ${\sim}N^2$ agent dependencies. %\mahak{${\sim} N^2$ dependencies or $N^2$ dependencies?}
%Thus, the challenge is to capture ${\sim}N^2$ agent dependencies to learn accurate policy estimates, given these sparse interactions.
%as the estimates have high variance for large $N$, 
%due to the curse of dimensionality.
This is, particularly, more challenging for large $N$ due to the curse of dimensionality, resulting in increased variance. 
%per user.
%For this, we need to consider the actions of all $N$ users to learn the policy for a single user, resulting in atleast $N^2$ parameters for learning policies for all $N$ users with $N$ actions per user.
%However, this requires estimating atleast $N^2$ parameters to model the $N \times N$ dependencies across all users, that is computationally very inefficient. 

%
%Additionally, joint learning that considers the actions of all agents for learning the policy i.e., ${\sim}N^2$ dependencies, is computationally intensive %since this requires estimating atleast $N^3$ parameters to model the $N \times N^2$ dependencies between all users. 
%the joint action space grows larger with $N$. %the increase in the number of agents,
%resulting in high computational complexity.
%
%Learning jointly with the full state and action spaces across all $N$ users (e.g., \cite{mannion2016dynamic}) to capture ${\sim}N^2$ dependencies requires estimating ${\sim}N^2$ parameters \cite{farajtabar2017fake}, \cite{goindanisocial}. %to capture $O(N^2)$ dependencies between all pairs of agents.  
%
%Thus, joint learning becomes computationally intensive, 
%Also, the impact of an individual's state features in learning her own policy diminishes with increase in $N$, which can result in noisy estimates as the policy parameters overfit to a single type of users who may be in majority.
%
%Additionally, independent learning requires training $N$ models, that is impractical for thousands of agents.
%This is impractical for thousands of agents, especially, when the policy function approximators are complex (e.g. Deep Neural Networks).
%
%Our goal is to learn a policy $\pi$ that maps the state representation (over $N$ users) to actions over ($N^2$ user pairs). This requires estimating atleast $N^3$ parameters to model the $N \times N^2$ dependencies between all users. 
%Since this is computationally intensive, we propose to cluster users into $\mathcal{G}$ clusters, so that we can learn a policy $\pi_G$ that maps the state representation of $\mathcal{G}$ clusters to $\mathcal{G}^2$ actions, where $\mathcal{G} \ll N$. We then combine this with a method to easily derive user-level actions from the cluster actions.
%



%In this work, we primarily consider real-world social networks with thousands of users who interact with each other (e.g. \cite{farajtabar2017fake}). 

%Because users interact in the network, actions taken for one user may impact the state (i.e., activity) of other users. More specifically due to peer-influence, changes in the activity of user $i$ may influence the likelihood of user $j$'s activities in the future if $i$ and $j$ are connected in $G$, either directly (i.e., $E_{ij}=1$) or through a longer path. For example, if one user tweets more, that may influence their followers to tweet more as well.
\iffalse
There is an opportunity to %use the relationship and/or similarity between the users in order to share information between them. 
%We take inspiration from relational RL and 
use the social network structure, which characterizes the relations and correlation between agents, to develop RL approaches that can scale for large number of agents.
\fi
%
%(e.g. \cite{yang2018mean_MFRL}).
%However, each user typically only interacts with a small number of other users in the network. This means the network interactions are overall sparse. 
%Since, users interact in the network, \textit{actions} taken for one user may impact the \textit{state} (i.e., activity) of other users due to peer-influence.
%Thus, agent interactions lead to \textit{dependencies} among agents' actions and state transitions. 
%
%in estimates.
%
%resulting in large variance in policy estimates.
%that results in insufficient information %samples/data 
%to capture higher-order agent \textit{dependencies} for learning accurate policies. 

Traditional MARL approaches do not scale for large numbers of agents. Learning a separate model for each user independently \cite{He2016OpponentMI, Battaglia2016InteractionNF, Hausknecht2016DeepRL, Yliniemi2016MultiobjectiveMC, Dusparic2009DistributedWM, cao2018emergent, leibo2017multi, Hughes2018InequityAI, jin2018real, mason2016applying, Kim2019MessageDropoutAE, Jaques2018IntrinsicSM, zhang2018fully, shu2018m, sukhbaatar2017intrinsic, Lazaridou2017MultiAgentCA, Mannion2017MultiagentCA, raileanu2018modeling, omidshafiei2017deep, Palmer2018NegativeUI, mannion2015learning, Kumar2017FederatedCW, yang2018mean_MFRL, sen2007emergence}
without considering agent dependencies results in less accurate policy estimates, and in addition, requires learning $N$ complex models that is infeasible for large $N$. 
Some recent work employed joint policy learning \cite{farajtabar2017fake,goindanisocial,sukhbaatar2016learning_commnet} to capture agent dependencies. However, these do not address the problem of sparse user interactions, and still estimate ${\sim}N^2$ parameters resulting in high computational cost. %that results in insufficient information to capture higher-order agent \textit{dependencies}. %for learning accurate policies.
Also, due to the high-dimensionality of joint state/actions representation in these methods, 
%an individual has less impact on her own policy compared to others and policy parameters may overfit to the agents in majority. 
the impact of an individual's state features in learning her own policy diminishes with increase in $N$, resulting in noisy estimates as the policy parameters overfit to a single type of users who may be in majority.
%Additionally, these still estimate ${\sim}N^3$ parameters resulting in high computational cost.
%
%Also, the impact of an individual's state features in learning her own policy diminishes with increase in $N$, which can result in noisy estimates as the policy parameters overfit to a single type of users who may be in majority.
%the policy estimates may be biased towards the users who are in the majority, as individual agents have less impact on their policies compared to others (due to the high-dimensionality of joint state/actions representation). Moreover, they still learn ${\sim}N^2$ parameters, which is computationally inefficient.
\iffalse
\cite{farajtabar2017fake,goindanisocial} employ joint policy learning %considering the states/actions of all users, 
where
%And, due to large $N$ and high dimensional state/action spaces %in joint learning, 
an individual has less impact on her own policy compared to others and policy parameters may overfit to the agents in majority. Additionally, it requires estimating ${\sim}N^2$ parameters that results in high computational cost.
\fi
%\mahak{
In addition, it makes it infeasible to model the reciprocity in agent interactions, because $N^2$ agent \textit{pairs} would lead to at least  $N \!\times\! N^2\!=\!N^3$ parameters. %and  to learn actions per agent pairs (i.e. ${\sim}N^2$) actions. However, this leads to an increase in the number of parameters to be estimated to ${\sim}N^3$, which is computationally very intensive. 
To avoid this, the above approaches considered only 
individual (i.e. $N$) actions per user.
%individual (i.e. ${\sim}N$) actions. %(eg. \cite{farajtabar2017fake,goindanisocial}).
%}


%We utilize agent correlations %Clustering similar agents helps to 
%to cluster the agents and reduce model dimensionality (i.e., number of parameters) from $O(N^2)$ to $O(\mathcal{G}^2), \mathcal{G} \ll N$, and thus computational cost, while still facilitating joint learning to capture agent \textit{dependencies}.
To address these challenges, we propose a \textit{Dynamic Cluster-based Policy Learning} approach \MethodName that utilizes the properties of the social network structure and agent correlations to obtain a compact model to represent the system dynamics.
%that can scale for large number of agents, and overcome sparsity in agent interactions. 
%
%Since similar users have similar behavior, our key idea is to reduce model dimensionality by learning similar policies/actions for similar users. 
Specifically, we propose to cluster similar users in order to reduce the effective number of policies to be learned, and overcome the problem of sparse data by aggregating the interactions of similar users. We then develop a method to easily derive personalized agent-level actions from cluster-level policies by exploiting %the similarity and 
variability in agents' behavior. 
%To overcome this, we propose to cluster users based on the observation that similar users have similar behavior, and thus, we can learn similar incentives for similar users. %Thus, we can apply the incentive learnt for the clusters to their respective members.
Thus, we reduce the problem of learning policies for $N$ users to that for $\mathcal{C}$ clusters $(\mathcal{C} \ll N)$,
%However, our approach can efficiently learn actions per agent pairs (i.e. ${\sim}N^2$) actions , to capture the reciprocity in agent interactions.
%we consider actions per agent pairs (i.e. ${\sim}N^2$) actions. However, 
and hence, the model dimensionality 
%is greatly reduced 
from ${\sim}N^3$ (with pairwise agent interactions) to ${\sim}\mathcal{C}^3$, %allowing 
to allow efficient and effective \textit{joint} policy learning considering all users. % (via the clusters).
\iffalse
Specifically, we propose to cluster users
%with latent features, and
and learn policies for the clusters, and develop a method to easily derive personalized agent-level actions from cluster-level policies by exploiting the similarity and variability in agents' behavior. 
\fi
%such that user-level actions are easily obtained from the cluster policy. %This helps to greatly reduce the computational cost while still facilitating joint learning to capture agent \textit{dependencies}.
%We obtain the interventions to be applied to the users based on their variability from their cluster. 
%Specifically, we propose to cluster similar users in order to reduce the effective number of policies to be learnt, and overcome the problem of sparse data by aggregating the interactions of similar users. We then develop a method to easily derive personalized agent-level actions from cluster-level policies by exploiting the similarity and variability in agents' behavior. 
%Thus, we can obtain more accurate policy estimates along with faster convergence due to large reduction in dimensionality and the variance.
\iffalse
This leads to a great reduction in the dimensionality of the state and action spaces,
%With this approach, the dimensionality of the state and action spaces reduces greatly, 
allowing efficient and effective \textit{joint} policy learning considering all users (via the clusters). %\mahak{approximate learning?} %considering all users in an indirect way. 
\fi

Learning policies from the global system reward alone, without considering individual contributions, can result in noisy estimates. %as an agent may be rewarded for performing poorly if other agents are performing well \cite{malialis2016resource}. Thus, we consider a user's contribution in a Difference Reward \cite{devlin2014potential} signal to shape the global reward and reduce noise in policy estimates.
To address this, we design clustering features, motivated by \textit{Difference Reward} \cite{devlin2014potential}. %for effective credit assignment and resource allocation under fixed budget.
%to capture users' \textit{payoff} and \textit{contribution} in maximizing the system reward. 
%that help in effective credit assignment for resource allocation.
%
Specifically, we define \textit{contribution} features to measure a user's efficacy given other agents' actions, and, \textit{payoff} features to determine how responsive an agent is to the policy applied in the past. %whether providing incentive to a user is beneficial based on her past actions. 
%These help in effective credit assignment for resource allocation under fixed budget. 
We use these features (via clusters) 
to learn agents' effectiveness early on, for better exploring the action space, without increasing the state space, in order to
%and thus, achieve faster convergence of policies.
speed-up convergence. %of policy leanring.
%Clustering users with the above defined features allows the global reward and agent contributions to be used to learn a joint policy more efficiently than independent learning. 
%We effectively use DR to cluster users, we are able to avoid learning a separate model for each user, as in the standard reward shaping techniques. 
%
%
%It is important to regulate policies at different time-steps to capture dynamic user behavior \cite{goindanisocial}. %to reflect changes in user behavior. 
Moreover, agent interactions in a social network are dynamic, and thus, we update the policy after regular time-intervals.
%to capture dynamic user behavior.
%we consider multi-stage policy learning, in which the policy is updated after regular time-intervals. %, to reflect changes in user behavior. %, and cluster assignments. 
%\mahak{controls at regular time-intervals?}
%The policy applied previously leads to a change in user behavior,
%This rresulting in a change in cluster assignments, across different stages. 
%We want the clusters to reflect the effects of applying the updated policy. Thus, we propose to dynamically update cluster memberships along with policy learning, while still accounting for aligning the clusters at different time-steps.
%leading leads to a change in agents' behavior due
Since we want clusters to reflect the effects of applying the updated
policy, we need to dynamically update cluster memberships while
learning the policy. However to learn across time steps, it is important to ensure that the clusters
are aligned---to achieve this, we propose a
\textit{weighted centroid} clustering approach. %described as follows.
%Thus, we propose an RL framework for interventions in social network interactions that uses a dynamic, cluster-based policy learning approach.
\iffalse
For this, it is important to ensure that the clusters are aligned at different time-steps. Thus, we propose to use \textit{weighted centroids} in our clustering approach to overcome this challenge.
\fi
To our best knowledge, our proposed approach is the first to consider policy learning while dynamically clustering users in MARL for social networks.

%Furthermore, we highlighted the problem of cluster alignment across multiple stages associated with the dynamic clustering of agents, and we proposed a weighted centroid approach to overcome this challenge.


We evaluate performance compared to different static clustering and non-clustering policy learning methods, using real-world Twitter datasets.
Results show that compared to other baselines, our dynamic cluster-based approach %based on \textit{payoff} features 
is able to 
learn better \textit{resource allocation} and  %of incentives among users, and \textit{credit assignment} 
achieve higher \textit{reward}, %in terms of maximizing the number of people reached by true news. 
by learning users' effectiveness via \textit{payoff} and \textit{contribution} features.
Clustering enables faster convergence of policy learning, by reducing the effective number of policies and producing a compact model with lower dimensionality.
%and thus the dimensionality of state/action spaces. 
In addition, our approach has lower variance, which indicates that clustering is able to overcome sparsity in agent interactions, and learn personalized policies that are not biased towards the majority type of users. %do not overfit to majority class/type of users.

%Due to large number of users and high-dimensional continuous spaces, joint learning becomes computationally inefficient. To overcome this, we propose a \textit{cluster-based policy learning} approach that utilizes the correlation between the agents to reduce the dimensionality of state/action spaces along with avoiding noisy estimates. %Our key idea is to first learn interventions for clusters that are then used to easily obtain interventions for users.
%We cluster users dynamically, and first learn interventions for clusters that are then used to easily obtain interventions for users.
%The approach is able to achieve faster convergence along with learning better policy compared to approaches that either do not use clusters, or only use static clusters. 

\iffalse
To summarize, our work makes the following major contributions:
%The main contributions of our approach can be summarized as follows. 
\begin{itemize}
    
    %\item Overcome the problem of sparsity by aggregating the interactions of correlated agents, that also reduces noise in estimates. 
    
    %The clustering features motivated from Difference Reward (DR) allow to measure the efficacy of users that is helpful in credit assignment for resource allocation under fixed budget. Additionally, by using the DR as clustering features, we can perform joint learning and avoid learning a separate model for each user that is infeasible for thousands of users. 
    
    %In our task, a user’s policy corresponds to the amount of incentive that should be allocated to her in the future (based on the network state). And a user’s contribution to maximizing reward governs the amount of incentive that is provided to her. Contribution is widely used in Multi-Agent Credit Assignment and Resource Allocation Problems (e.g.\cite{devlin2014potential}) because it determines a user’s efficacy, given the actions of other users.
    
    %Additionally, learning policies from the global system reward alone, without considering individual contributions, can result in noisy estimates, as an agent may be rewarded for performing poorly if other agents are performing well \cite{malialis2016resource}. Thus, we consider a user's contribution in a Difference Reward \cite{devlin2014potential} signal to shape the global reward and reduce noise in policy estimates.
    
    %Also, we assume that a user’s behavior may change over time and thus, the policy should be responsive to whether providing incentive to a user was beneficial. To capture this, we measure the change in a user’s individual reward as a result of applying the policy in the past (i.e. payoff).
    
    %Thus we design our clustering features, called PF, to more efficiently learn how to allocate incentive over time and to reduce noise in estimates. Contribution determines how useful is it to provide incentive to a user given the actions of other users, and payoff determines how likely a user will utilize the incentive provided based on her past actions. Clustering users with PF allows the global reward and agent contributions to be used to learn a joint policy more efficiently than independent learning.

    \item %The \textit{contribution} features measure user's efficacy given other agents' actions. And, \textit{payoff} features determine how responsive is an agent to the policy applied in the past. %whether providing incentive to a user is beneficial based on her past actions. 
    We design DR-based clustering features to help in effective credit assignment for resource allocation. % under fixed budget. %We use these efficiently to first cluster users and then learn a joint policy by incorporating both the global reward and agent contributions. With this, we avoid learning a separate model for each agent as in standard reward shaping techniques \cite{devlin2014potential}). % since it is impractical for thousands of agents. 
    %the policy, so that both the global reward and agent contributions are used to learn a joint policy and than independent learning (as in the standard reward shaping techniques \cite{devlin2014potential}). %, and reduce noisy estimates. 
    %
    %Using PF for clustering agents allows to effectively incorporate both global reward and individual agent contributions for joint policy learning that is more efficient than independent learning (in standard reward shaping approaches). 
    %
    %Although these are motivated from Difference Reward (DR), our approach is different from standard reward shaping techniques that consider learning separate model for each user (e.g. \cite{devlin2014potential}). Since, this is infeasible for thousands of agents, we use the DR based features to cluster users, and then learn the policy. This allows both the global reward and agent contributions to be used to learn a joint policy more efficiently %than independent learning, 
    %and reduce noisy estimates.
    We use these features (via clusters) to learn agents' effectiveness early on, for better exploring the action space, without increasing the state space, and thus the policies converge faster. 

    %Included in results: In C-PF, the information about agents' payoff and contribution via clusters, helps in better exploration over the action space without increasing the state space. This helps the model to learn agents' effectiveness early on and converge faster to the optimal policy.
    
    %We cluster users dynamically, and first learn interventions for clusters that are then used to easily obtain interventions for users.
    %The approach is able to achieve faster convergence along with learning better policy compared to approaches that either do not use clusters, or only use static clusters. 
    \item We utilize agent correlations %Clustering similar agents helps to 
    to cluster the agents and reduce model dimensionality (i.e., number of parameters) from $O(N^2)$ to $O(\mathcal{G}^2), \mathcal{G} \ll N$, and thus computational cost, while still facilitating joint learning to capture agent \textit{dependencies}. %between all agents. 
    %
    
    \item We propose a dynamic clustering approach that facilitates learning of policies that are responsive to change in agent behavior.
    %
    %Due to the reduced dimensionality, 
    %Reduced dimensionality enables a cluster and thus, 
    %By this, we enable a cluster, and thus,
    %a cluster has more contribution/impact in learning its own policy compared to other clusters, due to the reduced model dimensionality. In this way, 
    %any agent to have relatively more impact in learning her own policy compared to other agents, %, who would otherwise dominate. %the joint learning process.
    %
    %Additionally, in the joint state and action spaces that are used for learning policy in Chapter \ref{ch_1}, the effect of an individual's own state features is much less compared to other agents due to the presence of large number of agents. Clustering helps to avoid this problem by reducing the effective number of policies to be learnt, while still considering the state features of all users for joint learning.
    %
    %Due to the reduced model dimensionality, a cluster and thus,
    %a cluster has more contribution/impact in learning its own policy compared to other clusters, due to the reduced model dimensionality. In this way, 
    %any user has more impact in learning her own policy compared to other agents, who would otherwise dominate the joint learning process. 
    %
    %and avoid biased estimates that can otherwise be obtained due to overfitting of policy parameters to the majority type of agents, especially in joint learning.
    %can learn more accurate policy estimates that are responsive to the change in agent behavior.
    %
    We combine this with a method to easily derive personalized agent-level actions from cluster-level policies by exploiting the similarity and variability in agents' behavior. 
    %based on their distance from the centroid. This helps to capture both the similarity and variability in agents' behavior.
    %
    %Joint Learning can result in biased policy estimates as the policy parameters overfit to a single type of users who may be in majority. 
    %Additionally, joint learning can also result in biased estimates as the policy parameters overfit (learning becomes biased) to a single type of users who may be in majority. 
    %can be biased towards only a single type of users who may be in majority.
    %
    %By clustering users, we are able to learn personalized policies, and thus overcome the above problem, along with learning very less number of policy functions,
    %compared to learning a separate policy function for each user in independent learning. 
    %
    %Learn personalized policies by clustering similar agents together and avoid biased estimates that can result due to overfitting of policy parameters to the majority type of users in joint learning. %to a single type of users who may be in majority. 
    

\end{itemize}

\fi

==> ARXIV_Dynamic Cluster-based Policy Learning for Social RL/03-related-work.tex <==
\section{RELATED WORK} \label{related_work}

\begin{table*}[!t]
\centering
\caption{Comparison of Social RL approaches (highlighted) with existing MARL approaches. $`-'$ represents that a given attribute is not defined for the problem setting considered in the corresponding approach.}
%\hspace{-3mm}
%\vspace{-5mm}
%\scalebox{0.9}
{
\begin{tabular}{|c|c|c|c|c|c|}
    \toprule
    \multirow{4}{*}[-0.5\dimexpr \aboverulesep + \belowrulesep + \cmidrulewidth]{\textbf{Approach}} & \multicolumn{3}{|c|}{\textbf{Data/Environment}} & \multicolumn{2}{|c|}{\textbf{Model}} \\
    \cmidrule(l){2-6}
    {} & \textbf{\specialcell{Network \\Density}} & \textbf{\specialcell{Link \\Types ($d$)}} & \textbf{Space}  & \textbf{\specialcell{Maximum \\Dimensionality}} & \textbf{\specialcell{Effective \\ Dimensionality}}  \\
    \midrule
    \rowcolor{Yellow}  
    \cite{farajtabar2017fake} & $O(N)$ & 1 & C  & ${\sim}N^2$ & ${\sim}N^2$  \\
    \rowcolor{Yellow} 
    \cite{upadhyay2018deep} & $O(N)$ & 2 & C  & ${\sim}N$ & ${\sim}N$  \\
    \rowcolor{Yellow} 
    \cite{goindanisocial} & $O(N)$ & 2 & C  & ${\sim}N^2$ & ${\sim}N^2$  \\
    \rowcolor{Yellow} 
    %\cite{goindanisocial2020_aamas} & $O(N)$ & 3 & C  & ${\sim}N^3$ & ${\sim}k^3$  \\
    \cite{sukhbaatar2016learning_commnet} & $\Omega(N^2)$ & 1 & D  & ${\sim}N^2$ & ${\sim}N^2$ \\ 
    \cite{yang2018mean_MFRL} & $\Omega(N^2)$ & 1 & D  & ${\sim}N^2$ & ${\sim}N$ \\
    \cite{nguyen2017collective, Nguyen2018CreditAF} & $-$ & 1 & D  & ${\sim}N^2$ & ${\sim}N^2$  \\
    \cite{Lin2018EfficientLF} & $-$ & 1 & D  & ${\sim}N^2$ & ${\sim}k$ \\
    \cite{Leibo2018MalthusianRL} & $-$ & 1 & D  & ${\sim}kN$ & ${\sim}kN$ \\
    \bottomrule
\end{tabular}
}
\label{related_work_comparison_table}
%\vspace{-3mm}
\end{table*}

The number of agents in Social RL problems are large as opposed to much of previous work in MARL that considers small $N$
%number of agents 
\cite{malialis2015distributed, mason2016applying, Prolat2017AMR, Hausknecht2016DeepRL, Tampuu2017MultiagentCA, Liu2018EmergentCT, Taylor2014AcceleratingLI, He2016OpponentMI}.
Although, there are a few problems that involve large $N$  \cite{sukhbaatar2016learning_commnet, Nguyen2018CreditAF, nguyen2017collective, Lin2018EfficientLF, Leibo2018MalthusianRL},
they consider dense agent interactions %(i.e. ${\sim}N^2$) 
that allows to capture %${\sim}N^2$ 
agent dependencies more easily (e.g. \cite{yang2018mean_MFRL}). On the contrary, 
Social RL problems have sparse %network density (${\sim}N$ agent interactions)
interaction data \cite{farajtabar2017fake,goindanisocial,upadhyay2018deep} that makes it challenging to capture these dependencies for learning accurate policies \cite{goindanisocial2020_workshop}.
%(e.g. \cite{farajtabar2017fake}). %whereas other MARL problems consider a dense network 
%that results in insufficient information %samples/data 
%to capture higher-order dependencies for learning accurate policies. 
%Table 

We present a comparison of Social RL with state-of-the-art MARL approaches, based on different environment factors and model settings in Table \ref{related_work_comparison_table}. %, based on different environment factors and model assumptions/choices. 
The existing approaches that consider a small number of agents differed only on a few aspects. Thus, we focus on only those approaches that have considered a large number of agents. Learning policies for 
Continuous (C) spaces is more challenging than that for
Discrete (D) spaces, %is easier than that for , 
and much of the RL models are only applicable to discrete spaces %\cite{nguyen2018deep}. 
%For example, the state-of-the-art Deep Q-Network \cite{mnih2015human}, and
(e.g., \cite{Liu2018EmergentCT}). %, %\cite{Nguyen2018CreditAF}, \cite{nguyen2017collective}, \cite{yang2018mean_MFRL}). 
%are designed specifically for discrete action spaces. %However, it can be extended to high-dimensional continuous state spaces. 
%A possible solution is to discretize the continuous space, however, this can lead to multiple problems, specifically, the curse of dimensionality.
%From the table, we can see that much of the existing work considers discrete space. 
However, Social RL problems generally have continuous spaces describing %\cite{goindanisocial}, \cite{farajtabar2017fake}, \cite{upadhyay2018deep},
complex network activities. %in social networks, and the solutions for these can be easily extended/applied to the discrete problem settings. 
%
It is important to study the computational complexity (number of parameters required to learn policies for all agents) of different approaches. Based on the agent dependencies considered, each model has a maximum number of parameters required for learning the policy for all agents, referred to as the \textit{Maximum Dimensionality} in Table \ref{related_work_comparison_table}. %For example, considering $O(N^2)$ dependencies corresponds to joint learning in which the states and actions of all agents are used to learn the policy for any agent, and that requires $O(N^2)$ policy parameters. 
%Independent learning considers learning the policy for each agent based solely on their local observations and actions, thus requires $O(N)$ parameters in total for all agents (e.g., \cite{upadhyay2018deep}). 
\textit{Effective Dimensionality} corresponds to the effective (actual) number of parameters learned based on the approximations/assumptions made by the model. %to learn the policies. 
For example, \cite{Lin2018EfficientLF} considers an aggregate of agents to
obtain a smaller effective number of agents. %$k$. %to a constant $k$ 
%based on some aggregate statistic of agents. 
They learn policies using parameter sharing, resulting in effective number of parameters as ${\sim}k$. %However, since they do not condition on the actions of other agents to determine the actions for any agent, the policies obtained are non-stationary. Also,
However, their approach is designed for small restricted discrete action spaces \cite{nguyen2018deep}.
%
%\cite{nguyen2017collective}, \cite{Nguyen2018CreditAF} considers the problem of fleet management in a partially observable domain. 
%They assume that agents can observe the states of similar agents but not all agents
\cite{nguyen2017collective,Nguyen2018CreditAF} %simplify the problem by assuming that the interactions between the agents are not affected by the individual agents, but are instead influenced by some aggregate statistic (e.g., total number of agents), and 
use an aggregate statistic of agents' actions along with certain strong assumptions on the state-transition model, to capture ${\sim}N^2$ dependencies. 
%
%\cite{Lin2018EfficientLF} considers a partially observable fleet management system, in which they learn same policies for agents in same states, thus reducing the effective number of agents/policies. 
%However, these approaches are designed for small restricted discrete action spaces. %approach is limited to discrete spaces only, %, and is designed for problems in which the state transition depends only on some aggregate count of other agents and not the individual agents themselves. Thus, their approach makes strong assumptions on the state-transition model that is defined by them. 
%As opposed to this, we focus on developing solutions for the more challenging case when the underlying model for state-transition dynamics is not explicitly known, that is more likely to hold in the real-world tasks. 
%And, \cite{nguyen2017collective}, \cite{Nguyen2018CreditAF} defines their own state-transition model with strong assumptions.
%However, Social RL problems generally consider more challenging continuous spaces, and the complex state-transition dynamics are generally unknown.
%do not make strong assumptions on underlying state-transition dynamics.
%as these are more likely to occur in practice.
%
%However, the complex state-transition dynamics are generally unknown in Social RL problems.
However, Social RL problems usually have continuous spaces describing 
the intricate user interactions and network activities, and the complex state-transition dynamics are generally unknown.

There are several real-world applications involving social networks that can be modeled using Social RL. Social RL helps to estimate user responses (likes, comments, shares) considering effects of peer-influence \cite{goindanisocial}. It can be used to understand customer demands, and learn strategies to incentivize competing products by capturing changing user interests and feedback, e.g., recommender systems with thousands of users and very few user-user/user-item interactions such as news recommendation \cite{zheng2018drn},  recommending potential collaborators \cite{zhang2017dynamic}.
Also, it is important to learn credit assignment when multiple agents share a limited resource. Social RL can help identify \textit{influential} users for viral marketing or resource allocation under fixed budget. 
%This presents a need to study Social RL 
%
Social RL has been used to find solutions for critical problems involving social networks such as fake news mitigation and learning optimal intensities for news diffusion.
Thus, there is a need to develop efficient solutions for Social RL problems that can scale for large number of agents, and overcome the problem of sparse interaction data. 

\cite{farajtabar2017fake} proposed to 
%interventions using a Social RL framework to 
mitigate fake news by spreading more true news, %, especially among people who are already exposed to fake news.
on Twitter that is a sparse network with thousands of users. 
%They considered user interactions in the form of tweets and 
They integrated user activities and interactions (via tweets), characterized using Multivariate Hawkes Process (MHP) in a RL framework, and learned interventions for the MHP via policy optimization in a Markov Decision Process (MDP). % (\cite{bellman1957markovian_MDP}). 
%and learnt incentives to be provided to users to tweet more true news, via policy optimization in a Markov Decision Process (MDP).
%in a reinforcement learning framework. 
\cite{goindanisocial} extended their approach and proposed to model another form of user interactions, i.e. feedback, quantified as the number of likes received on sharing a post. The feedback is integrated in a Social RL framework that helps %learn effective incentivization strategy for 
appropriate selection of users and efficient allocation of incentives among them under budget constraints.
%reciprocity in user interactions in a social network, 
%by effectively learning .
\cite{upadhyay2018deep} considers %a Social RL problem with 
agent interactions via tweet and feedback for learning optimal strategies in personalized teaching and viral marketing domains, to increase the recall probability among learners, and \textit{visibility} among followers on Twitter, respectively.
%First, we propose an approximate learning approach that is efficient than both independent and full joint learning, to estimate incentives (interventions) required
%learn an intervention model 
%to promote the spread of true news in a social network---in order to mitigate the impact of fake news. We model news diffusion as a Multivariate Hawkes Process (MHP) and make interventions that are learnt via policy optimization in a Markov Decision Process (MDP).
%in a reinforcement learning framework. 
%The key insight is to estimate the response a user will get from the social network upon sharing a post, as it indicates her impact on diffusion, and will thus help in efficient allocation of incentive. %User responses also depend on political bias and peer-influence, which we model as a second MHP, interleaving it with the news diffusion process. 
%We evaluate our model on semi-synthetic and real-world Twitter data. %, comparing different models of news diffusion and investigating the impact of different network properties on performance. 
%The results demonstrate that our proposed model outperforms other alternatives that do not consider estimates of user responses and political bias when learning how to allocate incentives. %With real data, we measure the impact of nodes selected in the future and results show that it is beneficial to provide incentives earlier.
%
%how to allocate incentives among users so that they spread more true news,
%benefit from Social RL algorithms.

%Thus, it is essential to study Social RL problems that involve large number of interacting agents. %and deal with exponentially growing joint action space, for challenging dynamic environment comprising of high-dimensional and/or partially observable spaces, in collaborative and adversarial settings.
%
%We consider the important task of fake news mitigation as an example to demonstrate the real-world applicability of our proposed Social RL



%Some recent work employed Social RL setting.
\cite{farajtabar2017fake,goindanisocial} developed joint learning approaches for fake news mitigation on Twitter, by modeling agent interactions via tweets and \textit{likes}. 
%\mahak{
They consider individual (i.e. $N$) actions and estimate ${\sim}N^2$ parameters resulting in high computational cost for large networks. Also, they do not address the problem of sparse interactions that leads to increased variance in estimates. 
%
In contrast, %, and learn better resource allocation strategies, 
we reduce the model dimensionality by clustering similar users. % based on their payoff and contribution to the goal. 
This allows us to efficiently learn a more compact model and facilitates modeling actions per user {\em pair} (i.e. $N^2$ actions) to capture reciprocity. %, by effectively reducing the model dimensionality, and thus computational cost.
Moreover, it addresses the problem of sparse interaction data by aggregating the interactions of similar users.
\cite{upadhyay2018deep} %considered agent interactions via tweet and feedback, and
learned a separate model for each agent. However, this ignores inter-agent dependencies, and is infeasible for large $N$.
%}
\iffalse
Some recent work employed Social RL setting.
%Social RL has been used to find solutions for critical problems involving social networks such as fake news mitigation and learning optimal timings to share posts. %news diffusion.
\cite{farajtabar2017fake} proposed a joint learning approach for fake news mitigation, and considered only one type of agent interaction (via tweets). %considered a Social RL setting
%interventions using a Social RL framework to 
%mitigate fake news by learning interventions for news diffusion as a policy optimization problem in a Markov Decision Process.
%spreading more true news, %, especially among people who are already exposed to fake news.
%on Twitter 
%that is a sparse network with thousands of users 
%by considering a single type of agent interaction (via tweets).
\cite{goindanisocial} extended their approach and modeled another form of user interactions, i.e. feedback, 
%quantified as the number of likes received on sharing a post. The feedback is 
%to be integrated in a Social RL framework for %learn effective incentivization strategy for 
for appropriate agent selection and efficient resource allocation. %of incentives among them. %under fixed budget. %constraints.
However, these approaches do not address the problem of sparse interactions, and still estimate ${\sim}N^2$ parameters, resulting in high computational cost.
%
%However, these do not address the problem of sparse user interactions, resulting in noisy policy estimates, and still learn $O(N^2)$ parameters, that is computationally inefficient. Additionally, since they consider joint learning across all users, the policy estimates may be biased towards the users who are in majority, as individual agents have less impact on their policies compared to others as a result of the high-dimensionality of state/actions spaces. 
\cite{upadhyay2018deep} considered agent interactions via tweet and feedback, and learned a separate model for each agent, for personalized teaching and viral marketing domains. However, this ignores inter-agent dependencies, and is infeasible for large $N$.
\fi
%they do not consider inter-agent dependencies and 
%They learn a separate model for each agent, however, that is computationally intensive for large $N$.
%
%
%In this work, similar to \cite{goindanisocial}, we map the problem of learning interventions for MHPs as a policy optimization problem in a Multi-Agent Reinforcement Learning (MARL) framework, where the number of agents is large ($>\!1000$), with relatively few interactions between them. 
%In order to reduce the computational complexity, 
%Moreover, \cite{goindanisocial} considers only two types of agent interactions, i.e. tweet and feedback. They 
%Furthermore, 
%The above approaches 
%Additionally, they consider individual actions (i.e. ${\sim}N$)
\iffalse
Additionally, they do not distinguish between tweet and retweet activities,  %considered tweets and retweets as identical news sharing events,
and learn same action for both. %activities.
%the same type of interventions for a single process characterizing both types of events. 
%However, news diffusion patterns via tweets and retweets are nonidentical (Sec. \ref{introduction}).
%Modeling tweets and retweets separately.
%There are two ways in which information spreads in online social networks, one when a users shares their own posts (tweeting), and the other when users re-post the information shared by others (retweeting).
%However, the diffusion patterns of tweets and retweets are not identical. 
%However, the diffusion patterns of tweets and retweets are similar for true news, but have huge difference for fake news \cite{carchiolo2018terrorism}.
%However, the diffusion patterns of tweets and retweets have large differences, especially, for fake news \cite{carchiolo2018terrorism},
However, these have large differences in their diffusion patterns, %of tweets and retweets have large differences, 
especially, for fake news (e.g. \cite{carchiolo2018terrorism}).
%They also found that 
%analyzed the diffusion pattern of fake and true news on Twitter, and concluded
%that fake news spreads faster and stays longer than true news, and the number of retweets for fake news are much higher than that for true news. 
%it is due to the retweet events that the tweets are able to become widespread and reach a greater audience.
%analyzed the impact of retweets and 
%And, retweets play a major role in widespread and faster diffusion of news, compared to source tweets \cite{vosoughi2018spread}. %They found that the retweet network is very different from the followers network. %and most of the retweets are from users who do not follow the source user of the tweet.
%
%They observed that Twitter has a low level of reciprocity %and the influence between pair of users is asymmetric, 
%Moreover, 
\iffalse
and the retweet network is very different from the followers network on Twitter 
%with a low level of reciprocity 
\cite{vosoughi2018spread}.
\fi
%To capture these differences, we %extend the approach in \cite{goindanisocial} and 
%model the tweet and retweet events with separate %and feedback 
%processes, which increases the model dimensionality, particularly when the goal is to {\em jointly} learn user policies. %, and learn separate incentives for both. For the retweet events, we consider incentives for pairs of users to capture the asymmetry in the reciprocity of user interactions. %between them.
%
%and retweets play an important role in the widespread diffusion of fake news compared to true news. 
%Thus, we extend their approach by characterizing tweet and retweet events with separate processes
%To capture these differences, 
Thus, we consider tweet and retweet as separate network activities,
resulting in three different types of agent interactions. %network activities. 
In addition, we learn actions per user pair to capture the reciprocity in user interactions, i.e., ${\sim}N^2$ actions. 
%we learn interventions between pairs of users to capture the reciprocity in user interactions. 
%considering separate diffusion processes for tweet and retweet activities/events, and learning incentive for each user as well as pair of users, corresponding to tweet and retweet events, respectively. 
However, this leads to a large increase in model dimensionality, %of the state/action spaces, 
and thus, computational cost.
%particularly %when the goal is to {\em jointly} learn user policies, 
%for joint learning.
%resulting in large number of parameters (${\sim}N^3$), and 
%and thus increased computational complexity. %, by $O(N^2)$. 
%particularly when the goal is to {\em jointly} learn user policies.
%Thus, to reduce the %computational burden dimensionality 
%
To overcome this, %, and learn better resource allocation strategies, 
we will cluster users based on their payoff and contribution to the goal.
%with features reflecting their past behavior and contribution to the objective.
\fi
%
\iffalse
To reduce the computational complexity, previously %\cite{Lin2018EfficientLF} considered an aggregate of agents to obtain a smaller effective number of agents. %$k$. %to a constant $k$ 
%based on some aggregate statistic of agents. 
%They learn policies using parameter sharing, resulting in effective number of parameters as $O(k)$. However, since they do not condition on the actions of other agents to determine the actions for any agent, the policies obtained are non-stationary. Additionally, their approach is designed for small restricted discrete action spaces.
some approaches used an aggregate statistic of agents' actions along with certain strong assumptions on the state-transition model (e.g. \cite{Nguyen2018CreditAF}), and their approach is applicable to only small restricted discrete action spaces \cite{nguyen2018deep}.
%However, the complex state-transition dynamics are generally unknown in Social RL problems. 
However, Social RL problems usually have continuous spaces describing 
the intricate user interactions and network activities, and the complex state-transition dynamics are generally unknown.
\fi

\iffalse
Relational reinforcement learning (RRL) combines RL with relational learning %or inductive logic programming \cite{muggleton1994inductive} 
to represent states, actions, and policies using the relations that identify them \cite{ponsen2010learning}. %The structural representations facilitate solving problems at an abstract level, and thus RRL approaches provide better generalization.
%can be generalized better to unseen environment factors. 
%different instantiations of that abstract problem.
%abstractions from and generalizations over different states and actions. 
%RRL algorithms try to solve problems at an abstract level, and thus they can be generalized to different instantiations of that abstract problem.
%their solutions will often carry to different instantiations of that abstract problem. For example, resulting policies learned by an RRL system often generalize over domains with varying number of existing objects.
%
%Relational reinforcement learning (RRL) uses relational representations for states, actions, and learned value functions or policies to allow natural representations and abstractions of complex tasks. \cite{ponsen2010learning}. 
RRL has been used in multi-agent systems to share information among agents to learn better individual policies (e.g. \cite{grover2018evaluating}). %Additionally, information sharing among agents leads to great state space reduction \cite{ponsen2010learning}.
%RRL has been used in multi-agent systems to provide more knowledge to agents about the states, actions, policies of other agents that are useful in learning individual agent policies \cite{croonenborghs2005multi}. %, especially in partially observable settings where %agents do not have complete system information. 
%agents only have partial information about the environment.
%overcome the problem of large state spaces by utilizing agent interactions
%Information sharing among agents leads to great state space reduction and provides enhanced ability to generalize to new states \cite{ponsen2010learning}.  
%The abstraction and generalization abilities provided by relational representations allow the agents to easily generalize over unseen parts of the environment that helps them learn better policies, especially in settings when agents have only partial system information \cite{ponsen2010learning}.
%in partially observable settings, where agents only have partial information about the environment.
%
%Previous work used first-order representations to achieve effective state/action abstractions (e.g. \cite{dvzeroski2001relational,asgharbeygi2006relational,ponsen2010learning}).  %used RRL for learning communication policy among agents in a partially observable setting. 
%Some recent work has used relational interactions between agents for policy learning in multi-agent systems (e.g. \cite{grover2018evaluating}).
%in cooperative and competitive environments to accelerate multi-agent learning 
%(e.g. \cite{grover2018evaluating}).
%\cite{grover2018evaluating,grover2018learning,tacchetti2018relational,zambaldi2018relational}).
However, this adds extra complexity with increased state space as a result of the abstraction, informedness, and generalization abilities provided by RRL \cite{croonenborghs2005multi}.
Thus, these approaches are limited to discrete spaces and dense networks with small number of agents, %that have dense interactions between them, 
and previous RRL methods are not applicable in Social RL settings.
We take motivation from relational learning to capture agent relations and interactions, however, we do not directly use %the setting of 
RRL due to the above limitations. %described above.
\fi

\cite{goindanisocial} did not distinguish between tweets and retweets,  %considered tweets and retweets as identical news sharing events,
and learned the same action for both activities.
%the same type of interventions for a single process characterizing both types of events. 
%However, news diffusion patterns via tweets and retweets are nonidentical (Sec. \ref{introduction}).
%Modeling tweets and retweets separately.
%There are two ways in which information spreads in online social networks, one when a users shares their own posts (tweeting), and the other when users re-post the information shared by others (retweeting).
%However, the diffusion patterns of tweets and retweets are not identical. 
%However, the diffusion patterns of tweets and retweets are similar for true news, but have huge difference for fake news \cite{carchiolo2018terrorism}.
However, the diffusion patterns of tweets and retweets have large differences, especially, for fake news \cite{carchiolo2018terrorism}.
%They also found that 
%analyzed the diffusion pattern of fake and true news on Twitter, and concluded
%that fake news spreads faster and stays longer than true news, and the number of retweets for fake news are much higher than that for true news. 
%it is due to the retweet events that the tweets are able to become widespread and reach a greater audience.
%analyzed the impact of retweets and 
%And, retweets play a major role in widespread and faster diffusion of news, compared to source tweets \cite{vosoughi2018spread}. %They found that the retweet network is very different from the followers network. %and most of the retweets are from users who do not follow the source user of the tweet.
%
%They observed that Twitter has a low level of reciprocity %and the influence between pair of users is asymmetric, 
Moreover, retweet network is very different from followers network on Twitter with a low level of reciprocity \cite{vosoughi2018spread}.
%To capture these differences, we %extend the approach in \cite{goindanisocial} and 
%model the tweet and retweet events with separate %and feedback 
%processes, which increases the model dimensionality, particularly when the goal is to {\em jointly} learn user policies. %, and learn separate incentives for both. For the retweet events, we consider incentives for pairs of users to capture the asymmetry in the reciprocity of user interactions. %between them.
%
%and retweets play an important role in the widespread diffusion of fake news compared to true news. 
%Thus, we extend their approach by characterizing tweet and retweet events with separate processes
To capture these differences, we consider tweet and retweet as separate network activities,
resulting in three different types of agent interactions. %network activities. 
Also, we learn actions per user pair to capture the reciprocity in user interactions, i.e., $N^2$ actions. 
%we learn interventions between pairs of users to capture the reciprocity in user interactions. 
%considering separate diffusion processes for tweet and retweet activities/events, and learning incentive for each user as well as pair of users, corresponding to tweet and retweet events, respectively. 
However, this leads to an increase in the model dimensionality, %of the state/action spaces, 
particularly %when the goal is to {\em jointly} learn user policies, 
for joint learning,
resulting in large number of parameters (${\sim}N^3$), and high computational cost. %, by $O(N^2)$. 
%particularly when the goal is to {\em jointly} learn user policies.
%Thus, to reduce the %computational burden dimensionality 

To overcome this, and learn better resource allocation strategies, we propose to first cluster users with latent features (based on their past behavior and contribution to the objective).
%
\iffalse
To reduce the computational complexity, previously \cite{Lin2018EfficientLF} considered an aggregate of agents to obtain a smaller effective number of agents. %$k$. %to a constant $k$ 
%based on some aggregate statistic of agents. 
%They learn policies using parameter sharing, resulting in effective number of parameters as $O(k)$. However, since they do not condition on the actions of other agents to determine the actions for any agent, the policies obtained are non-stationary. Additionally, their approach is designed for small restricted discrete action spaces.
However, their approach is applicable to only small restricted discrete action spaces \cite{nguyen2018deep}. 
\cite{nguyen2017collective,Nguyen2018CreditAF} 
used an aggregate statistic of agents' actions along with certain strong assumptions on the state-transition model.  
%However, the complex state-transition dynamics are generally unknown in Social RL problems. 
However, Social RL problems usually have continuous spaces describing 
the intricate user interactions and network activities, and the complex state-transition dynamics are generally unknown.
\fi
%
Previous work utilized \textit{symmetry} between states and/or agents to reduce the size of the Markov Decision Process \cite{zinkevich2001symmetry, ravindran2002model, mahajan2017symmetry}.
%
%Our goal is to group together similar performing users, so that we can learn policies characterizing the performance level of the group of users. %personalized for similar performing groups of users.
Our clustering approach is based on the observation that 
%users are similar to some and dissimilar from others, and 
similar users tend to show similar behavior, and thus we propose to learn similar policies for them.
%our key insight is to utilize the correlations between agents to reduce the size of the Markov Decision Process (MDP).
This has also been utilized to cluster users in mobile health domain
\cite{zhu2018group,el2018personalization}. %, who clustered users in an RL application for mobile health data. %and learn interventions to encourage users to adopt healthier alternatives. %in their lifestyles. 
%
%\cite{el2018personalization} also used cluster-based reinforcement learning to learn health interventions and found that clustering speeds up the learning process and is useful provided a good clustering is obtained. 
%
%They cluster users only once with features based on user states and rewards obtained from
%by running a default policy on 
%historical data, and assume the cluster assignments remain fixed thereafter.
However, they did not consider user interactions and dependencies, clustered users only once, and assumed the cluster assignments remain fixed (\textit{static}) throughout policy learning. %thereafter.
%These fixed clusters obtained from historical data under the default policy are then used to learn the intervention policy (for the current data). 
%They learn the policies for the clusters and apply the same to their members.
%However, they do not test if the cluster memberships learnt under the default policy using historical data also hold for the intervention policy that they learn using current data. Additionally, if the cluster assignments are fixed, then the clusters might not be reflective of the policy applied.
%However, the cluster memberships obtained from historical data can change after the policy is applied, and do not capture the effect of the policy.
%
In our setting, we consider %multi-stage interventions and 
dynamic user interactions, and the policy is updated after regular time-intervals. 
Thus, there is a need to dynamically update cluster assignments, and we propose an approach %a \textit{weighted centroid clustering approach} 
to ensure cluster alignment at different time-steps.
%to capture the change in user behavior due to policy learning. 
%To our best knowledge, our proposed approach is the first to consider policy learning while dynamically clustering users in MARL for social networks.


%The purpose of this paper is to stimulate research in MARL methods for domains with large number of agents $(>1000)$ with relatively few (sparse) relations and interactions between them, which we refer to as \textit{Social Reinforcement Learning}. {\em Social reinforcement} refers to the process where acceptance and praise from others reinforces behaviors/preferences of an individual (e.g. \cite{jones2011behavioral}). With the increased use of social media, response from peers plays an important role in shaping the behavior and decision-making of individuals (e.g. \cite{lee2015understanding}). 


Relational reinforcement learning (RRL) combines RL with relational learning or inductive logic programming \cite{muggleton1994inductive} to represent states, actions, and policies using the structures and relations that identify them \cite{ponsen2010learning}. The structural representations facilitate 
solving problems at an abstract level, and thus RRL approaches provide better generalization.
%can be generalized better to unseen environment factors. 
%different instantiations of that abstract problem.
%abstractions from and generalizations over different states and actions. 
%RRL algorithms try to solve problems at an abstract level, and thus they can be generalized to different instantiations of that abstract problem.
%their solutions will often carry to different instantiations of that abstract problem. For example, resulting policies learned by an RRL system often generalize over domains with varying number of existing objects.
%
%Relational reinforcement learning (RRL) uses relational representations for states, actions, and learned value functions or policies to allow natural representations and abstractions of complex tasks. \cite{ponsen2010learning}. 
RRL has been used in multi-agent systems to share information among agents, to learn better individual policies \cite{croonenborghs2005multi}. %Additionally, information sharing among agents leads to great state space reduction \cite{ponsen2010learning}.
%RRL has been used in multi-agent systems to provide more knowledge to agents about the states, actions, policies of other agents that are useful in learning individual agent policies \cite{croonenborghs2005multi}. %, especially in partially observable settings where %agents do not have complete system information. 
%agents only have partial information about the environment.
%overcome the problem of large state spaces by utilizing agent interactions
%Information sharing among agents leads to great state space reduction and provides enhanced ability to generalize to new states \cite{ponsen2010learning}.  
%The abstraction and generalization abilities provided by relational representations allow the agents to easily generalize over unseen parts of the environment that helps them learn better policies, especially in settings when agents have only partial system information \cite{ponsen2010learning}.
%in partially observable settings, where agents only have partial information about the environment.
%
Previous work used first-order representations to achieve effective state/action abstractions \cite{dvzeroski2001relational,asgharbeygi2006relational,ponsen2010learning}.  %used RRL for learning communication policy among agents in a partially observable setting. 
Some recent work has also used relational interactions between agents 
for policy learning in multi-agent systems
%in cooperative and competitive environments to accelerate multi-agent learning 
\cite{grover2018evaluating,grover2018learning,tacchetti2018relational,zambaldi2018relational}.
%However, relational learning adds extra complexity with increased state space as a result of the abstraction, informedness, and generalization abilities provided by it \cite{croonenborghs2005multi}.
While relational languages facilitate compact state space representations, in multi-agent scenarios, relational interactions further increase the size of the state space and increase reasoning complexity~\cite{croonenborghs2005multi}.
Thus, these approaches are limited to discrete spaces with small number of agents that have dense interactions between them.
%Thus, these approaches are limited to discrete spaces with small number of agents that have dense interactions between them, and previous RRL methods are not applicable in a Social RL setting.
We take motivation from relational learning to capture agent relations and interactions, however, we do not directly use %the setting of 
RRL due to the limitations described above.


%The purpose of this paper is to stimulate research in MARL methods for domains with large number of agents $(>1000)$ with relatively few (sparse) relations and interactions between them, which we refer to as \textit{Social Reinforcement Learning}. {\em Social reinforcement} refers to the process where acceptance and praise from others reinforces behaviors/preferences of an individual (eg. \cite{jones2011behavioral}). With the increased use of social media, response from peers plays an important role in shaping the behavior and decision-making of individuals (eg. \cite{lee2015understanding}). 



==> ARXIV_Dynamic Cluster-based Policy Learning for Social RL/04-approach.tex <==
\iffalse
\section{Problem Statement}

We formulate the problem to combat fake news, as a policy optimization problem in a Markov Decision Process (MDP). %An MDP is a 5-tuple (S, A, P, R, $\gamma$), where S is  State Space, A is Action Space, P is State transition probability function, %$P_{ss'}^a = \mathbb{P}[S_{t+1}|S_t = s, A_t = a]$, where t is time or stage. 
%R is the reward function, %$R_s^a = E[R_t+1 | S_t = s|A_t = a]$
%$\gamma$ is the discount factor.%, which tells how much of the future rewards contribute to the reward obtained by taking an action from the current state. 

Our goal is to find a policy function $\pi: S \rightarrow A$ that maximizes the total reward in term of .... This policy function is the intervention added to the base exogenous intensity of the true news diffusion process.% that maximizes the diffusion of true news.

%\todo[inline]{clearly define the number of exposures}

\fi

\iffalse
\section{Data Description} \label{data_descp}

%We consider two types of information diffusion processes over a network of $N$ users, namely, Fake News Diffusion, and True News Diffusion. These are modeled as Multivariate Hawkes Process (MHP), where the dimensions are users in the network. 

We consider two types of news: Fake and True. The diffusion occurs over a network of $N$ users. 
For fake news diffusion, an event is said to occur when a user shares a post related to fake news, $e^F =  (t^F, i)$ where $t^F$ is the time at which user $i$ is shares posts related to fake news. Similarly, we have $e^T =  (t^T, i)$ for the true news diffusion process. We consider an observation time window of time length $T$ for the diffusion of news that is further divided into stages (intervals) with each stage of length $\Delta T$.
Let $D$ be an $N \times N$ user adjacency matrix representing the followers network (directed), $D_{ij} = 1$ if $j \neq i$ and $j$ follows $i$, and 0 otherwise. %Define $E$ as $N \times N$ user adjacency matrix representing the followers network (directed), $E_{ij} = 1$ if j follows i, and 0 otherwise.

%Let $H(t)$ be a $N \times N$ \textit{time-dependent} adjacency matrix representing the user retweet network. %$H_{ij}(t) = c$ if $j \neq i$ and $j$ follows $i$, and 0 otherwise. 
%$H_{ij}(t)$ is the number of times user $j$ retweets the post made by user $i$ upto time $t$, and $j \neq i$. Let $U$ be $N \times N$ adjacency matrix representing a multiplex network where users have more than one type of relation (follower, retweet). $U(t) = D + H(t) $ ($U_{ij}(t) \in \mathbb{Z}^+ \cup \{0\})$. %We take $U_{ii}(t) = 0$.
\fi

\section{SOCIAL REINFORCEMENT LEARNING}

\subsection{PROBLEM DEFINITION} \label{prob_def}

We define \textit{Social Reinforcement Learning} as a sub-class of Multi-Agent RL, that considers large number of agents with interactions between them. %\mahak{(i.e. the total number of interactions among agents is much less compared to the total number of users.)}
%
Specifically, we consider a social network setting with $N$ users. Each user $i \in \{1,...,N\}$ is an agent.  
Let $G = (V, E)$ represent the social network graph, where each node $v_i \in V$ corresponds to user $i$, and edge $E_{ij} = 1$ if there exists an edge between agent $i$ and $j$, and 0 otherwise.
%
In addition, users perform $d$ different activities (e.g., tweet, comment, like) in the social network. We say that the network is dense when all the agents interact, i.e., the  number of interactions is $\Omega(N^2)$, and the network is sparse when agents only interact with a constant number of other agents, i.e., $O(N)$ interactions. %Let there be $d$ activities that a user can perform.

Let $\textbf{s}_i \in \mathbb{R}^{d} \; (\textbf{s}_i \geq 0)$ be the state of user $i$. This corresponds to the $d$ activities the user performs. Then the state of the network represents the activities over the $N$ users, $\textbf{s} = \{\textbf{s}_i\}_{i=1}^N$. The network activities are dynamic in nature, and thus, we have different states of the network at different time-stamps. Let $\textbf{s}_t$ represent the network state at time $t$. We consider a finite horizon setting, i.e., we observe the activities up to time $T$.
%
An action $a_{d, i} \in \mathbb{R}$ corresponds to a modification to the $d$-th activity of user $i$. Let $\textbf{a}=\{a_{d, i}\}_{i=1}^N$ refer to a set of actions, one for each user in the network. 
Collective actions of all users lead to a change in the state of each user, and consequently, a change in the overall network state. Let $\mathcal{T}(\textbf{s}, \textbf{a}, \textbf{s}^\prime)$ be the probability of transitioning to the network state $\textbf{s}^\prime$ after performing actions $\textbf{a}$ in network state $\textbf{s}$. %where $\textbf{s}^\prime = \{\textbf{s}^\prime_i\}_{i=1}^N$ is the next state of the system. 
%
While there may be a reward for each agent $i$ and/or each activity $d$, for generality we will consider a network-based (i.e., common) reward $R(\textbf{s},\textbf{a}) \in \mathbb{R}$ that is based on the network state and collective actions of users. 
%\jen{Rewards are based on activities, which is the network state, not the actions, right?} \mahak{Actually, I again checked and confirmed that the reward is associated with both the state and actions. $R(s_t,a_t)$ is the reward obtained on taking action $a_t$ in state $s_t$, and the reward helps to determine whether the action taken is good or not.}
%joint actions $\{a_{t,i}\}_{i=1}^N$. 
The goal is to learn a policy that maps the network state at time $t$ to  actions for each user, i.e., $\pi: \textbf{s}_t \rightarrow \textbf{a}_t$ such that the total expected discounted reward $\sum\limits_{t=1}^T \gamma^{t-1} \mathbb{E}[R_{t}]$ is maximized, where $\gamma \in [0, 1)$ is the discount rate. %governing relative importance of immediate and future rewards. 

%Agents interact with each other by performing certain network activities, (e.g., tweet, comment, like). These interactions lead to an increase in the likelihood of certain actions in the future due to peer-influence and effect of past interactions, and this effect decays over time. 
%The interactions between users affects their activities in the future, and this effect decays over time. 
%Due to this, there is a temporal dependency between agents' states and actions, and hence, the data is not independent and identically distributed.

%Users perform different activities (e.g., tweet, comment, like) \mahak{resulting in interaction between the users, which lead to dependencies among user activities}. \mahak{Thus, there are $d \in \mathbb{Z}^+)$ types of interactions between users, that we call \textit{link type} between agents.}
%Each agent $i$ performs action $a_{d, i} \in \mathbb{R}$ corresponding to the $d$-th link type
Because users interact in the network, actions taken for one user may impact the state (i.e., activity) of other users. More specifically due to peer-influence, changes in the activity of user $i$ may influence the likelihood of user $j$'s activities in the future if $i$ and $j$ are connected in $G$, either directly (i.e., $E_{ij}=1$) or through a longer path. For example, if one user tweets more, that may influence their followers to tweet more as well. Fig. \ref{network_fig_workshop} shows a network of users who interact via tweeting news. 
%
Thus, agent interactions lead to dependencies among agent actions and state transitions. 
Specifically, the state transition distribution does not depend on the individual user activities $\textbf{s}$ and actions $\textbf{a}$ alone, but also depends on the network $G$,
i.e., $P(\textbf{s}^\prime | \textbf{s}, \textbf{a}, G) \neq P(\textbf{s}^\prime | \textbf{s}, \textbf{a})$.  Also note that the underlying state transition distribution is not always explicitly known as it depends on the network dynamics, which is the model-free RL setting. Since the network reward $R$ depends on the state transition distribution $\boldsymbol{\mathcal{T}}$, and  user $i$'s activity can be moderated both by actions taken with respect to $i$ and actions taken for other users $j\!\neq\! i$, it is important to consider the effect of network structure when learning the policy $\pi$. 
%
At the same time, social networks are typically sparse with only $O(N)$ interactions between agents. Thus, the challenge is to capture ${\sim}N^2$ agent dependencies 
given these sparse interactions. %that are only $O(N)$.

%These interactions between agents can be dense or sparse. We say that the system has dense interactions if the number of interactions is $O(N^2)$, where $N$ is the number of agents, and the system has sparse agent interactions when the number of interactions is $O(N)$.

%%There are $d \in \mathbb{Z}^+)$ types of interactions between users, that we call \textit{link type} between agents, corresponding to $d$ network activities.
%There is a change in the state of individual users, and hence the complete state of the network, due to the collective effect of user interactions. 


%where $s^\prime$ is the state of the network after agents jointly take actions $\{a_{d, i}\}_{i=1}^N$. To evaluate the effectiveness of taking action $a_{d}$ in state $s$, we measure a collective reward $R$ that again depends on the network structure $G$, i.e., $R(s) = f(s^\prime, G)$. The reward $R$ is dependent on the dependencies among the agents, and hence we need to account for those in the actions and state-transitions. 

%Each agent performs actions $\textbf{a}_i \in \mathbb{R}^{d}$ corresponding to $d$ network activities and receives reward $R_i \in $.
%We consider a finite horizon setting, i.e., we observe the activities upto time $T$.
%The network activities are dynamic in nature, and thus, we have different states of the network at different time-stamps. Let $\textbf{s}_t$ represent the network state at time $t$.
%
%Social RL involves multiple interacting agents. %However, it is different from existing work on Multi-Agent Reinforcement Learning (MARL) as it considers a large number of agents with long-range dependencies. %in which the actions of an agent can be effective after multiple transitions/time-steps. %of the environment. 
%that have long-range dependencies between their states and actions. 
%Agents interact with each other that further influences their actions in the future, and the effect of these interactions decays over time.
%Agents interact with each other by performing certain network activities, (e.g., tweet, comment, like). These interactions lead to an increase in the likelihood of certain actions in the future due to peer-influence and effect of past interactions, and this effect decays over time. 
%The interactions between users affects their activities in the future, and this effect decays over time. 
%Due to this, there is a temporal dependency between agents' states and actions, and hence, the data is not independent and identically distributed.
%Additionally, the effect of these interactions decays over time, and there are long-range dependencies, in which the actions of an agent are effective only after multiple transitions of the environment.

\begin{figure}[!t]
    \centering
    %\vspace{-2mm}
    \includegraphics[height=5cm]{figures/Social_RL.png}
    %\vspace{-2mm}
    \caption{\small{Social network with agent interactions. Colored nodes represent active users (darker shade for users who are tweeting, lighter shade for people exposed to tweets). State is given by the number of tweets for users [A,B,C,D,E], and reward is calculated as the number of users exposed. Users' collective actions of tweeting news lead to a transition from state $\textbf{s}$ to $\textbf{s}^\prime$.}}
    %\vspace{-4mm}
    \label{network_fig_workshop}
    %\mahak{incude this figure or the figure for fake news mitigation as this has a different reward than the one considered in the rest of the paper?}

\end{figure}
%\mahak{write s and r in figure in latex, and what to use r or $r^\prime$ for next state reward?}

\iffalse
There are $d \in \mathbb{Z}^+)$ types of interactions between users, that we call \textit{link type} between agents, corresponding to $d$ network activities.
The state of a user $i$ is given as $\textbf{s}_i \in \mathbb{R}^{d} (\textbf{s}_i \geq 0)$. The state of the network represents $d$ network activities (link types) over $N$ users, $\textbf{s} = \{\textbf{s}_i\}_{i=1}^N$ i.e., $s \in \mathbb{R}^{dN} (\textbf{s} \geq 0)$. 
%Each agent performs actions $\textbf{a}_i \in \mathbb{R}^{d}$ corresponding to $d$ network activities and receives reward $R_i \in $.
We consider a finite horizon setting, i.e., we observe the activities upto time $T$.
The network activities are dynamic in nature, and thus, we have different states of the network at different time-stamps. Let $\textbf{s}_t$ represent the network state at time $t$.
\fi

\subsection{CHALLENGES}

We present different challenges for learning Social RL models and discuss potential opportunities to address them using properties of the network structure and agent correlations. 

\subsubsection{High-Dimensionality}

The joint action space grows larger with $N$, %the increase in the number of agents,
as it considers the actions of all agents for learning the policy %for a single agent, 
i.e., $O(N^2)$ dependencies, resulting in high computational complexity.
%Thus, joint learning becomes computationally intensive, 
Also, the impact of an individual's state features in learning her own policy diminishes with increase in $N$, which can result in noisy estimates as the policy parameters overfit to a single type of users who may be in majority.
%
Additionally, independent learning requires training $N$ models. This is impractical for thousands of agents, especially, when the policy function approximators are complex (e.g. Deep Neural Networks).
%Thus, there is the problem of high computational complexity and large variances in policy estimates due to the high dimensional spaces. 

\iffalse
We can utilize the social networks structure, characteristics of user interactions, and agent correlation to develop policy learning approaches based on certain approximations that simplify the learning process, while still accounting for all agent dependencies given large number of users.
%
For e.g., \cite{goindanisocial} decouple the different processes governing user interactions to approximate the joint action space more efficiently. They dynamically optimize the policy corresponding to agent interactions via tweets, but only use historical data to estimate another type of interaction, i.e., feedback. This helps to reduce the number of parameters and avoid noisy policy estimates.
\fi


\subsubsection{Sparsity}

Typically, social networks are sparse with only $O(N)$ agent interactions. Thus, learning accurate policies becomes difficult as there are not sufficient samples available to capture $O(N^2)$ agent dependencies. %between the agents. 
This is particularly more challenging for large $N$ due to curse of dimensionality, resulting in large variance in estimates.

%We can avoid the problem of sparse data by aggregating the interactions of similar/correlated users \cite{goindanisocial2020_aamas}. This can also help to reduce the dimensionality of the search space, and thus the variance and the number of parameters.

Next, we present potential solutions to address the above challenges using properties of the network structure and agent correlations. Our key insight is to utilize the correlations between agents to reduce the size of the Markov Decision Process (MDP). Specifically, we propose to cluster similar users in order to reduce the effective number of policies to be learnt, and overcome the problem of sparse data by aggregating the interactions of similar users. Thus, we can obtain more accurate policy estimates along with faster convergence due to large reduction in dimensionality and the variance.
We demonstrate the utility of our proposed approach using the application of  
Fake News Mitigation in social networks as follows. 

\section{CLUSTER-BASED SOCIAL RL APPROACH} \label{approach}
%\mahak{Include method name here?}

\subsection{APPLICATION: FAKE NEWS MITIGATION} 

We consider a social network with $N$ users who interact via $d$ different
network activities (e.g. tweet, like).
%Users perform $d$ different network activities (e.g. tweet, retweet, like). %in the social network.
%that corresponds to a followers network.  
Each user $i \in \{1,...,N\}$ is an agent.  
%See Supplementary Material\footnote{\href{https://www.dropbox.com/s/ipqkhawu0joweel/Supplementary_Material_AAMAS_2020.pdf?dl=0}{Supplementary Material}: \\ \href{https://www.dropbox.com/s/ipqkhawu0joweel/Supplementary\_Material\_AAMAS\_2020.pdf?dl=0}{https://www.dropbox.com/s/ipqkhawu0joweel/Supplementary\_Material\_AAMAS\_2020.pdf?dl=0}} for a table summarizing all notations.
%, where users can follow other users, and share their own posts or circulate others' posts. %We represent the followers network with a matrix 
Let $\textbf{G}$ %\footnote{We use the bold font to represent vector and matrices.} 
represent the followers adjacency matrix for the social network graph, where $G_{ij} = 1$ if $j$ follows $i$, and 0 otherwise. %When a user shares a new post, we refer to this first instance (share) of the post as \textit{tweets}, and when other users share this tweet, we refer to those instances as \textit{retweets} of the source/original tweet. 
%
%We consider following three types of events characterizing user activities in the networks. A Tweet event occur when a user shares a new post, a Retweet event occurs when a user retweets the (re)tweets of other users, and a Like event occurs when a user likes the tweets of others.
%The network is dense when all the agents interact, i.e., the  number of interactions is $O(N^2)$, and the network is sparse when agents only interact with a constant number of other agents, i.e., $O(N)$ interactions.
%We consider a sparse network where agents only interact with a constant number of other agents, i.e., $O(N)$ interactions \cite{goindani2020social}.
%
%\mahak{$d$ or $z$ for network activities?}
Our data contains a temporal stream of events with the time horizon [0, $\mathcal{T}$) divided into $K$ stages, each of time-interval $\Delta T$, where stage $k \in [1, K]$ corresponds to the time-interval $[\tau_k, \tau_{k+1})$. %We consider (re)tweets that are labeled fake (F) or true (T).
We consider three types of events characterizing user activities, corresponding to tweets ($\mathscr{T}$), retweets ($\mathscr{R}$), and likes ($\mathscr{L}$). % \mahak{remove this? - that users receives on sharing a post.} %The type of event is indicated using $z$ = $\mathcal{T}$ or $\Re$ or $\mathcal{L}$.
We represent the tweet or retweet events using $e=(t, i, h, z)$ where $t$ is the time-stamp at which user $i$ shares a post of type $z$ = $\mathscr{T}$ or $\mathscr{R}$, with label $h$ = $F$ (Fake) or $T$ (True). %corresponding to fake or true news. %The retweet events are represented as $o=(t^{\prime}, i, e)$, where $t^{\prime}$ is the time-stamp at which user $i$ retweets tweet $e$.
(Note that our goal is not to detect, but to mitigate the impact 
%the mitigation and not detection 
of fake news. Thus, we consider the (re)tweets labeled fake/true apriori.)
Like events are represented as $l(u, i, t)$ indicating user $i$ likes user $u$'s post at time $t$. %These help to %quantitatively measure 
%quantify the response received by a user on sharing a post, to determine her efficacy. 
%
To enhance readability, we provide a list of symbols used in the paper along with their description in Table \ref{notations}. 

\begin{table*}[!h]
\centering
\caption{Notations}
%\vspace{-3mm}
\scalebox{0.85}
{
\begin{tabular}{lll}
    \toprule
    {} & \textbf{Symbol} & \textbf{Description} \\
    \midrule
    \multirow{6}{*}[-0.5\dimexpr \aboverulesep + \belowrulesep + \cmidrulewidth]{{\specialcell{\textbf{Data} \\ \textbf{Description}}}} & $N$ & Number of Agents (users) \\
    & $\textbf{G}$ & Social Network \\
    & $h$ & Label for news: Fake (F) or True (T) \\
    & $z$ & Type of network activity: Tweet ($z=\mathscr{T}$) or Retweet ($z=\mathscr{R}$) or Like ($z=\mathscr{L}$) \\
    & $\mathcal{T}$ & Time-Horizon \\
    & $K$ & Number of Stages \\
    & $k \in [1,K]$ & $k-$the Stage corresponds to Time-Interval $[\tau_k, \tau_{k+1})$ \\
    & $\Delta T$ & Time-interval Length, i.e., $\tau_{k+1} - \tau_k$ \\
    %$\upsilon$ & Type of user: True News Spreaders ($\mathscr{T}$) or Fake News Spreaders ($\mathscr{F}$) or Common Users ($\mathscr{C}$) \\
    %& $p_i$ & Indicates if user $i$ favors Republican (R) or Democrat (D) Parties  \\
    %& $b_{i}^{p_i}$& Political bias, i.e., degree of user $i$'s leaning towards $p_i = $ R (Republican) or D (Democrat) Parties \\
    \midrule
    \multirow{10}{*}[-0.5\dimexpr \aboverulesep + \belowrulesep + \cmidrulewidth]{{\specialcell{\textbf{Activity} \\ \textbf{Processes}}}} & $\lambda_{h, z, i}$& Intensity function for user $i$ to share a post with label $h$ = F or T, and type $z$ = $\mathscr{T}$ or $\mathscr{R}$ \\
    & $\mu_{h, z, i}$& \specialcell{Base Exogenous Intensity for user $i$ to share a post with label $h$ = F or T, type $z$ = $\mathscr{T}$ or $\mathscr{R}$, \\ whose intensity is governed by Multivariate Hawkes Process (MHP)} \\
    & $\boldsymbol{\Phi}_z$& Kernel Adjacency Matrix for MHP for network activity of type $z$\\
    & $\omega_{h, z}$& Kernel Decay Parameter for Exponential Hawkes Kernel \\
    %& $\psi_{k, v, i}$& Intensity function for user $i$ to \textit{like} the post of user $v$ in stage $k$ \\%the time-interval $[\tau_k, \tau_{k+1})$ \\
    %& $\chi_{i}$& Base Exogenous Intensity for user $i$ to \textit{like} a post, whose intensity is governed by MHP \\
     & 
    $\mathcal{N}_i(t,h,z)$ & Number of posts of label $h$ (= T or F), and type $z$ (= $\mathscr{T}$ or $\mathscr{R}$), made by user $i$ upto time $t$ \\
    & ${n}_{k, i}(h,z)$ & Number of posts of label $h$ (= T or F), and type $z$ (= $\mathscr{T}$ or $\mathscr{R}$), made by user $i$ in stage $k-1$ \\ %time-interval $[\tau_k, \tau_{k-1})$ \\
    & ${W}_i(t)$ & Number of likes received by user $i$ upto time $t$ \\
%$W_{ui}(t)$ be the number of times user $i$ likes the (re)tweets by user $u$ up to time $t$
    & ${w}_{k,i}$ & Number of likes received by user $i$ in stage $k-1$ \\ %time-interval $[\tau_k, \tau_{k-1})$ \\
    \midrule
    %\multirow{7}{*}[-0.5\dimexpr \aboverulesep + \belowrulesep + \cmidrulewidth]{{\specialcell{\textbf{Multi-Agent} \\ \textbf{Reinforcement} \\ \textbf{Learning}}} }
    %\midrule
    \multirow{20}{*}[-0.5\dimexpr \aboverulesep + \belowrulesep + \cmidrulewidth]{{\specialcell{\textbf{Cluster-based} \\ \textbf{Policy} \\ \textbf{Learning}}}} & 
    $\mathcal{C}$& Number of Clusters \\
    %& $g_{k,i}$ & Cluster of user $i$ at stage $k$ \\
    %& $G_k = \{g_{k,i}\}_{i=1}^N$ & Set of all cluster assignments at stage $k$\\
    & $\textbf{s}_{U,k, i}$ & State of User $i$ at stage $k$\\
    & $\textbf{s}_{U,k}$ & User-level Network State at stage $k$\\
    & $\textbf{s}_{C,k, m}$ & State of Cluster $m$ at stage $k$\\
    & $\textbf{s}_{C,k}$ & Cluster-level Network State at stage $k$\\
    & $\textbf{a}_{U, z, k, i}$ & Action of User $i$ at stage $k$ for activity $z$ = $\mathscr{T}$ or $\mathscr{R}$\\
    & $\textbf{a}_{C, z, k, m}$ & Action of Cluster $m$ at stage $k$ for activity $z$ = $\mathscr{T}$ or $\mathscr{R}$\\
    & $\boldsymbol{\mathcal{M}}_k \in \{0, 1\}^{N \times \mathcal{C}}$ & Cluster Membership Matrix at stage $k$\\
    & $\textbf{X}_{k,i}$ & Clustering Features for user $i$ at the start of stage $k$ \\
    & $\beta_{z, k, i}$ & \textit{Payoff} Feature for user $i$ for stage $k$, corresponding to activity of type  $z$ = $\mathscr{T}$ or $\mathscr{R}$ \\
    & $\Omega_{d, k,i}$ & \textit{Contribution} Feature for user $i$ for stage $k$, corresponding to activity of type  $z$ = $\mathscr{T}$ or $\mathscr{R}$ \\
    & $\textbf{Y}_{k, m}$ & Centroid of cluster $m$ at stage $k$ \\
    & $\pi_{C,m}$ & Policy for Cluster $m$\\
    & $\pi_{U}$ & Function to obtain User-level Actions from the Cluster-level Actions (Algorithm 2, Main Paper)\\
    & $d$ & Number of activities in the network\\
    %& $\textbf{s}$& State of the network  \\
    %$\textbf{o}_i$& Local observation of user $i$ \\
    %& ${a}_{z,i}$& Action for user $i$ corresponding to activity of type $z$ = $\mathscr{T}$ or $\mathscr{R}$\\
    & ${R}$& Reward \\
    & $V(\textbf{s}_{U,k})$& Value-function for network state $\textbf{s}_{U,k}$  \\
    %& $\pi$& Policy Function \\
    & $\gamma$& Discount rate governing the relative importance of immediate and future rewards \\
    \bottomrule 
\end{tabular}
}
\label{notations}
%\vspace{-5mm}
\end{table*}

A quantitative measure of the impact of fake and true news is the number of people exposed. %, that has also been used in \cite{goindanisocial}. %\cite{farajtabar2017fake}. %Let $\mathcal{N}_{i}(t)$ be the number of times user $i$ shares news/posts up to time $t$. 
Let $\mathcal{N}_i(t, h, z)$ represent the number of times user $i$ shares news of type z = $\mathscr{T}$ or $\mathscr{R}$, with label $h$ = $F$ or $T$, up to time $t$. %, where $c$ = F or T, corresponding to fake or true news, and z = $\mathcal{T}$ or $\Re$, corresponding to tweet or retweet event. 
Then the number of times a user $i$ is exposed to news up to time $t$ corresponds to $G_{ji} \cdot \mathcal{N}_j(t, h, z)$ ($j \in [1,N]$). 
Let $W_{i}(t)$ be the number of likes received by user $i$ upto time t.
%times user $i$ likes the tweets by user $u$ up to time $t$. %Since it is difficult to limit the spread of fake news, we incentivize users to increase sharing true news. We believe that an increased exposure to true news can increase skepticism for fake news, thus, reducing its impact, as explained in Sec \ref{introduction}.
%
%It is not feasible to control the diffusion of fake news. 
%Our goal is to reduce the impact of fake news. 
Our goal is to incentivize users to share true news---to ensure that users receive at least as much true as fake news. %(i.e., $G_{.i} \cdot \mathcal{N}(t,F) \simeq G_{.i} \cdot \mathcal{N}(t,T)$). 
%(i.e., $A_{.i} \mathcal{N}_i(t, F, z) \simeq A_{.i} \mathcal{N}_i(t, T, z)$). 
Algorithmically, we want to increase the probability of sharing true news in a targeted fashion %(for both tweets and retweets) 
by learning an efficient strategy to %appropriate selection of users and efficient 
allocate incentive among users, based on properties of the network $\textbf{G}$ and the effects of past user interactions.  
%From an algorithmic perspective, we want to learn an efficient strategy for allocation of incentives among users, assuming a budget constraint. (Rephrase:
%We assume a budget constraint on the amount of incentive that can be allocated, and aim to learn an efficient strategy for allocating incentives among users.
%
Specifically, given the network {\em state} $\textbf{s} \in \mathbb{R}^{dN}$ corresponding to $d$ user activities  
(described further in Sec. \ref{state_features}), %$\textbf{s} \in \mathbb{R}^{dN}$ $(\textbf{s} \geq 0, d \in \mathbb{Z}^+)$, which represents $d$ network activities over $N$ users, 
we want to learn an incentivization policy $\pi: \textbf{s} \rightarrow \textbf{a}$ to obtain incentive {\em actions} $\textbf{a} \in \mathbb{R}^{N + N^2} (\textbf{a} \geq 0)$, where tweet actions are per user (i.e., $N$) and retweet actions are per user pair (i.e., $N^2$).
Incentive corresponds to increasing the likelihood of users sharing true news, %In real world, these 
and can be realized (in real-world) %given to users to share more true news. 
by creating certain accounts whose sharing rate is increased according to the learnt policy or by using external motivation (eg. money). %in the form of money or \textit{reward points}.
%e.g. [Farajtabar et al., 2017] performed real-time interventions on Twitter by creating certain accounts whose sharing rate is increased according to the learned policy. 
%
 %\cite{shu2019studying_network_properties}, \cite{goindanisocial}.
Note that fake news mitigation is a multifaceted problem, and the reward function depends on the different applications. 
Thus, in contrast to the simple reward described in Sec. \ref{prob_def}, now we will consider \textit{reward} as the correlation between exposures to fake and true news. This is based on the idea that users exposed more to true news must be exposed more to fake news \cite{farajtabar2017fake}. 
%To overcome the above challenges, 

%we can utilize the symmetry between states and/or agents to reduce the size of the MDP (e.g. in \cite{mahajan2017symmetry}, \cite{zinkevich2001symmetry}).
%
%We can avoid the problem of sparse data by aggregating the interactions of similar/correlated users. This can also help to reduce the dimensionality of the search space, and thus the variance and the number of parameters.

\begin{figure*}[!t]
\centering %width=18cm
    {\includegraphics[width = 16.5cm]{figures/Flowchart_OmniGraffle_ARXIV.png}}
    \caption{Overview of Dynamic Cluster-Based Policy Learning and Evaluation} 
    \label{flowchart}
    %\mahak{update fig to map the section numbers later.}
\end{figure*}

\subsection{OVERVIEW} \label{overview}

%
%
Fig. \ref{flowchart} illustrates the different components of our system. %We use Multivariate Hawkes Processes (MHP) to characterize user activities corresponding to tweet, retweet and like events. 
Our key insight is to decouple the processes governing tweet, retweet and like activities. This helps to study the effect of different types of activities in news diffusion, and learn an \textit{approximate} model more efficiently than full joint learning. 
%We divide the real data into Training Data (TD) and Held-Out Data. %shown using labels `A' and `B', respectively, in the figure. %Training Data corresponds to the first $K$ stages, i.e., time $[\tau_0, \tau_{K})$, and Held-Out Data corresponds to the last $K$ stages, i.e., time $[\tau_{3K+1}, \tau_{4K})$.
%We use the 
%The spread of information in social networks can be captured using stochastic point processes that use \textit{intensity functions} governing the rate of sharing per user.
%
We map the excitation events to states in a Markov Decision Process (MDP), and learn how to incentivize users %interventions.
to increase the \textit{intensity function} for true news diffusion. 
%and learn different parameters governing the respective intensity functions.
%We use the Training Data to estimate different parameters that characterize the MHPs (Fig. \ref{flowchart}, arrow 1). %We use the MHPs to generate events and
%We obtain Simulated Training Data (STD) by simulating the MHPs to generate events %for $K$ stages corresponding to time $[\tau_{K+1}, \tau_{2K})$, that is 
%conditioned on the Training Data. 
%
%Using the events from the STD, 
%Our idea is to cluster users to reduce learn better estimates of the 
To further increase the efficiency, we cluster similar users together so that we can learn a smaller {\em cluster-level} policy, from which we can easily derive individual actions for the members of each cluster. 

Specifically, from the training data we learn a set of Multivariate Hawkes Processes (MHP), one for each type of activity event, and also cluster the users. We use the MHP models to simulate additional training data for learning the policy. While learning the policy function $\pi_C$, we compute the state features for each cluster (based on its current members) and compute the actions for clusters given the current policy, and use those to derive user-level actions. Then we calculate expected reward, and use this to further optimize the policy and update the cluster memberships.

%We obtain the initial clusters using the Training Data. We generate Simulated Training Data (STD), conditioned on Training Data, and  compute state features of the clusters using the state features of users. Then, we learn a policy function $\pi_G$, using STD, to obtain interventions for the clusters. %given $s_G$. %given the state features $s_G$ of the clusters, that are obtained using the 
%We use function $\pi_U$ to map interventions learnt for clusters to their members $\pi_G$. as a function of
%After this, we obtain the interventions for the users as a function of the interventions obtained for their clusters, 
%Then we map the interventions obtained for the clusters to their respective members (users), %for the users 
%After learning $\pi_G$, given the state $s_U$ and clusters $G$, we obtain the interventions $a$ for the users using function $\pi_U$, and 
%The interventions for the users are then used to 
%and calculate expected reward used to optimize the policy and re-cluster users. %We repeat these steps until convergence, as shown by the iterate loop in the figure. 

%At the end of the learning phase, we obtain the optimal policy $\pi_G$, and the updated clusters $G_K$.

%Under the assumption that clusters converge at the end of the learning phase, we can use the cluster assignments $G_k$ for evaluating the learnt policy. 
To evaluate the estimated policy $\hat{\pi}_C$, we simulate data again from the MHPs. %for $K$ stages corresponding to time $[\tau_{2K+1}, \tau_{3K})$, that is conditioned on the last stage of STD (arrow 4, label I). 
Using the final clusters $C_K$, we obtain actions from the policy to add to the MHP intensity functions and generate evaluation data to assess empirical reward. We also assess the effectiveness of the users selected by our model to promote true news by measuring their number of retweets in held out training data. Each component is described in more detail next.

\vspace{-2mm}
%\subsection{Processes characterizing User Activities} \label{processes}
\subsection{ACTIVITY PROCESSES} \label{processes}
\vspace{-1mm}

%UAI: A number of diffusion models have been developed to capture the spread of information in social networks. Many of these models are based on stochastic processes that use {\em intensity functions} governing the sharing rate per user. Some intensity functions depend only on network structure, while others take into account the effect of previous events and interactions between users. 

%Our goal is to evaluate the learnt policy in a dynamically changing environment where users post and generate feedback simultaneously, and 
 %And, we do not know apriori the response a user would receive on sharing news under the diffusion model. 
%To reduce the dimensionality of the MDP, we decouple the processes governing tweet, retweet and {like} activities. %, and do not want to include them in the MDP, to reduce its complexity. %of MDP.
%as that will make the MDP more complex to model. 
%Moreover, since we cannot make real-time interventions, we need a process to simulate the environment dynamics.
%
%For tweet and retweet events, we have separate intensities for fake and true news diffusion, whereas we do not differentiate the like events as they are a form of feedback that a user receives and do not aid the actual \textit{spread} of news. 
%We use MHP to model these events, and describe their intensities as follows. 
%
%The processes governing tweet, retweet and like events are inter-leaved, and 
%Thus, we use $N$-dimensional %Multivariate Hawkes Processes (MHP) 
%MHPs to characterize events. %(Fig.~\ref{flowchart}, `C'). %their intensity functions that we describe next. %where each dimension corresponds to a user.
%to be inter-leaved with the tweet and retweet diffusion processes,
%To model the intensities of these events/activities, we consider an $N$-dimensional Multivariate Hawkes Processes (MHP), where each dimension  corresponds to a user, based on the quantitative evaluation that assesses different candidate processes for news diffusion in \cite{goindanisocial}. %
%
%
%For tweet and retweet events, we have separate intensities for fake and true news diffusion. 
%
%Let $\mathcal{F}_{i}(t)$ and $\mathcal{T}_{i}(t)$ be the number of times a user $i$ tweets posts corresponding to fake and true news, respectively by time $t$. Similarly, we use $\Re^{F}_i(t)$ and $\Re^{T}_i(t)$ to represent the number of times user $i$ retweets posts corresponding to fake or true news by time $t$.  We use $\mathcal{N}_{i}(t)$ ($\Re_{i}(t)$) as a generic notation to represent the number of times user $i$ tweets (retweets) posts by time $t$ where $\mathcal{N} (\Re) = \mathcal{F} (\Re^{F})$ or $\mathcal{T} (\Re^{T})$ depending on the type/label of news (fake or true). %We use Ogata's Thinning Algorithm \cite{ogata_thinning} as the generative process to determine the time-stamps at which user $i$ makes posts, given their respective intensities, and compute $\mathcal{N} (\Re)$ 
%
%Let $\mathcal{N}_i(t, c, z)$ represent the number of times user $i$ shares news by time $t$, where $c$ = F or T, corresponding to fake or true news, and z = $\mathcal{T}$ or $\Re$, corresponding to tweet or retweet event. 
%See Supplementary Material for more details on MHP. 
%
%We describe the generative process to determine the time-stamps at which user $i$ makes posts corresponding to true news, given their respective intensities as follows. The process for fake news is analogous. 
%We use Ogata's Thinning Algorithm \cite{ogata_thinning} to generates event times by sampling inter-arrival times using rejection sampling.
%
%Since the mathematical form of the intensity functions for fake and true news diffusion is the same except for parameters, we provide a generic expression for the intensities as follows. %Let $\lambda_i^T$ be the intensity for user $i$ tweeting a post corresponding to true news. (The process for fake news is defined analogously.) 
%diffusion of both fake and true news in social networks. 
%As observed in the previous work that MHPs better characterize the diffusion of information in social networks, we use MHP based models to govern the diffusion of news as follows. 
%
%Also, we use the decaying exponential kernel to capture the diminishing influence of a post with time, in real-world social networks (e.g. \cite{farajtabar2015_event_prioritization}). 
%
%\subsection{User Activities}
%MHPs are counting processes used to model arrival of events such that the occurrence of events in the past increases the likelihood of event occurrences in the future, and an event in one dimension can affect the likelihood of event occurrences in other dimensions. MHPs are extensively used to model news diffusion in social networks as they capture the effect of peer-influence and past user interactions (e.g. [Farajtabar et al, 2017]). Also, [Goindani, and Neville, 2019] conducted extensive experiments and verified that MHPs better capture news diffusion, compared to several baselines, on the same Twitter data as ours. Thus, we used MHPs to characterize news diffusion, and create simulated data for training and evaluation. 
%
As in \cite{farajtabar2017fake, goindanisocial}, we use $N$-dimensional MHPs \cite{hawkes1971spectra} to model user activities and simulate the environment dynamics.
%
%MHPs \cite{hawkes1971spectra} are counting processes that model the arrival of events. They better capture news diffusion in social networks by considering history of events and user-interactions \cite{goindanisocial}.
%of peer-influence and %past user interactions 
%past events .
%Moreover, since we cannot make real-time interventions, we need a process to simulate the environment dynamics.
%Thus, we use $N$-dimensional MHPs to model user activities.
Let $\lambda_{h, z, i}$ be the intensity function governing the sharing rate of user $i$, where $h$ = $F$ or $T$, and $z$ = $\mathscr{T}$ or $\mathscr{R}$: %(\mahak{change notation for label c to h?})

\begin{small}
\begin{equation} \label{MHP_intensity}
%\hspace{-2mm}
\lambda_{h, z, i}(t) = \mu_{h, z, i}  + \sum\nolimits_{j=1}^N  \int_{0}^{t}  \Phi_{z, ji} \text{ } (\omega_{h,z} e^{-\omega_{h,z} t}) \text{ } d\mathcal{N}_j(s, h, z) \nonumber
\end{equation}
\end{small}

\noindent where, the integral is over time, and $s$ is used as placeholder for limits \{0,t\}. %\{$\tau_{k}, \tau_{k+1}$\}.
$\mu_{h, z, i}$ is the base exogenous intensity of user $i$, $\Phi_{z, ji}$ is a kernel adjacency matrix estimated from the training data, and %(Fig. \ref{flowchart}, Arrow 1).
%$\Im_j$ is the influence of user $j$ in the diffusion process, and 
$\omega_{h,z} e^{-\omega_{h,z}t}$ is exponential Hawkes kernel. %\cite{hawkes_tutorial}. %\cite{farajtabar2017fake}. %that is estimated from the data. 
%For the \textbf{Tweet MHP}, we consider $\Phi_{\mathscr{T}, ji} = \mathcal{I}_j \: A_{ji}$, where $\mathcal{I}_j$ is the influence of user $j$ in the diffusion process. %and is estimated from the data. 
For \textbf{Tweet MHP} and \textbf{Like MHP}, we use MHP models proposed in \cite{goindanisocial} to obtain $\mathcal{N}_i(t,h,\mathscr{T})$ and $W_i(t)$.
For the \textbf{Retweet MHP}, we need to estimate the (asymmetric) influence between all pair of users for $\Phi_{\mathscr{R}, ji}$ %since the follower and retweet networks do not overlap completely \cite{vosoughi2018spread}. 
to capture reciprocity.
This naively requires ${\sim}N^2$ parameters, but we use a low-rank approximation of the kernel matrix, proposed in 
%Scalable Low Rank Hawkes Process (SLRHP) 
\cite{lemonnier2017multivariate}, to improve efficiency. %\jen{What rank do you use?} %\mahak{2, assuming the influencer-influencee relationship between users}.\jen{State explicitly} 
%(In our experiments, we will use rank $o=2 \ll N$.)
%\mahak{Considering an influencer-influencee relation between users, we project $\Phi_{\Re} \in \mathbb{R}^{N \times N}$ %to obtain a projection matrix $\Xi \in \mathbb{R}^{\hbar \times \hbar}$ 
%in a lower dimensional space $\mathbb{R}^{\hbar \times \hbar}$, ($\hbar=2 \ll N$), where $\hbar$ is the rank of projection in lower dimensional space.}
%
Our policy will learn actions that correspond to \textit{interventions} to increase sharing of true news events ($h$= $T$) only.
Let $a_{z, k, i}$ be a constant intervention action for user $i$ at stage $k$ (time $t \in [\tau_k, \tau_{k+1})$), added to the her base intensity. %of user $i$. %Then for $c=$T, we obtain:
%After adding the intervention, we obtain, %the intensity for true news diffusion as follows,

\begin{equation} \label{general_equation}
\begin{aligned}
\hspace{-2mm}
    \lambda_{T, z, i}(t) &= \mu_{T, z, i} + a_{z, k, i} 
    \\ &+ \sum\limits_{j=1}^N  \int_{0}^{t}  \Phi_{z, ji} \text{ } (\omega_{T,z} e^{-\omega_{T,z} t}) \text{ } d\mathcal{N}_j(s, T, z)
\end{aligned} \nonumber
\end{equation}
%
%

\iffalse
\noindent
For the \textbf{Like MHP}, we use the \textit{User Response Model} proposed in \cite{goindanisocial}, that models pairwise-MHP to determine the number of likes, $W_i(t)$. % (Sec \ref{prob_def_fake_news}).
\fi

%
\iffalse
%The feedback that a user receives determines her effectiveness in the news diffusion process, and a quantitative measure of this feedback in online social networks is the number of likes received on sharing a post. 
For the \textbf{Like MHP}, we use the \textit{User Response Model} proposed in \cite{goindanisocial}, that models pairwise-MHP to determine the the total number of likes received by user $v$ during stage $k$, i.e., $W_{k,v}  = \sum \limits_{i=1, i \neq v}^N \int_{\tau_{k}}^{\tau_{k+1}} dW_{vi}(s)$.
% to characterize the process governing \textit{like} events between pairs of users. %with MHP as follows.
%to characterize the like events. %, that measures the response for a user at the end of each stage. 
%
%Let $\textbf{W}(t) = [W_{ui}(t)]_{u,i=1, u \neq i}^N$, where $W_{ui}(t)$ is the number of times user $i$ likes the (re)tweets by user $u$ up to time $t$. 
The total number of likes received by user $v$ during stage $k$ is $W_{k,v}  = \sum \limits_{i=1, i \neq v}^N \int_{\tau_{k}}^{\tau_{k+1}} dW_{vi}(s)$, %\jen{what is $s$ here? is it the integral over time?} \mahak{yes, s is used as placeholder for limits, it is integral over time.} \jen{State explicitly}
%
%\mahak{where the integral is over time, and s is used as placeholder for limits \{$\tau_{k}, \tau_{k+1}$\}}.
%\mahak{but the integral over time is also for tweet and retweet MHPs, so should I state that in the beginning of this section?} \jen{yes}
%Thus, the feature vector representing the number of likes received by users is given as $\textbf{w}_k = \{ W_{k,v}\}_{v=1}^N$ \jen{this doesn't appear to be used, canyou remove it?}, 
and the intensity function is, 
%
%the environment generating user responses using another MHP as described below.
%
%
\vspace{-4mm}
\begin{align}
    \psi_{k+1, v, i}(t) = \chi_{i} &+ \mathbb{I}(p_{k,i} \!=\! p_{k,v})b_{p_{k,i},k,i} -  \mathbb{I}(p_{k,i} \!\neq\! p_{k,v})b_{\neg p_{k,i},k,i} \nonumber
    \\ &+ \sum\limits_{j \in {A}_{.i}}^N \int_{0}^{t} A_{ji} \text{ } (\omega_{\mathscr{L}} e^{-\omega_{\mathscr{L}} t}) \text{ } dW_{vj}(s) \nonumber \label{response_intensity}
\end{align}
\vspace{-4mm}
%
%
\noindent where $t \in [\tau_k, \tau_{k+1})$, $\chi_i$ is the base intensity, %of a user $i$ to \textit{like} a post, estimated from the data, and is independent of the history, 
%and $(\omega e^{-\omega t})$ is the exponential Hawkes kernel. %The values of $\chi$ and $\omega^L$ are obtained using the same procedure as in the previous work (UAI Paper). ${A}_{.i}$ is the set of followees of $i$. 
%Change wording:{Using above, we try to accumulate the response a user receives from her direct and indirect followees, by aggregating the likes by followees of user $i$ to the post of user $u$. The more frequently the followees of $i$ like $u$'s posts, the more she tends to ``like" $u$'s posts. }
%Similar to the previous work (UAI Paper), we estimate $\chi$ from the data using Maximum Likelihood Estimation, and set $\omega = 1$ for simplicity.
%For simplicity, we set $\omega^L = 1$ as in the previous work (UAI Paper). 
%We use MHP$_\psi$ to denote the MHP for like events.
%For additional details, refer to \cite{goindanisocial}.
%\mahak{add description for bias and polarity, or move to supplementary?}
Here, $p_{i} = R$ or $D$ represents if user $i$ favors Republican (R) or Democrat (D) Parties, respectively, and $b_i$ represents user $i$'s degree of \textit{political bias} proposed in \cite{goindanisocial}.
%\footnote{Due to space constraints, we describe the Political Bias parameter and more details of the MHPs in \href{https://www.dropbox.com/s/ipqkhawu0joweel/Supplementary_Material_AAMAS_2020.pdf?dl=0}{Supplementary Material}.}. %towards the two parties. 
\fi
%
\noindent To simulate the event data, we interleave the MHPs to generate tweet events, then retweet events, and then like events. 


%\subsubsection{Learning Optimal Interventions}
\subsection{DYNAMIC CLUSTER-BASED POLICY} \label{dynamic_cluster_based_policy}

%We integrate the excitation events and the phenomenon of social reinforcement by mapping the problem of learning incentives as a policy optimization problem in an MDP. 
%a cooperative multi-agent reinforcement learning framework.
%Now, if we can reduce the dimensionality of the state and actions spaces, we can model tweet and retweet events separately with reduced computational cost. 
%Our idea is to first cluster users and learn policies for the clusters, that are then applied to their respective members. 
%
%We propose to learn a cluster-based policy to obtain interventions by clustering $N$ users into $\mathcal{G}$ clusters, %and model an $N$-dimensional (not $G$-dimensional) MHP. 
%We use clustering as an intermediate step to make 
%to make policy estimation faster, and reduce noise in estimates by combining similar users, and learning similar policies for them. % similar users (learning a single policy for all users in a cluster).
%performing users on the dynamically changing performance of users. 
%
Our goal is to learn a policy $\pi$ that maps the state representation (over $N$ users) to intervention actions for tweet and retweet intensities ($N +N^2$ actions). To lower the computational cost, our key insight is to utilize agent correlations to reduce the size of the MDP. %Markov Decision Process (MDP).
Specifically, we propose to cluster users into $\mathcal{C}$ clusters, so that we can learn a policy $\pi_C$ that maps the state representation of $\mathcal{C}$ clusters to $\mathcal{C} +\mathcal{C}^2$ actions, where $\mathcal{C} \ll N$. We %will combine this with 
then develop
a method to derive user-level actions from the cluster-level actions. % use these to easily determine the actions for users.
%then apply the actions for clusters to their respective members. 
%
%We cluster $N$ users into $\mathcal{G}$ clusters. Let the clusters be $\{G_1, G_2, ..., G_\mathcal{G}\}$.
%Let $\mathcal{M}^k \in \{0, 1\}^{N \times \mathcal{G}}$ be the cluster membership matrix, where $\mathcal{M}^k_{ig} = 1$ if user $i$ belongs to cluster $G_g$ at stage $k$, and $0$ otherwise. %Let $X^{k}_i = [\alpha^{1,k}_i, \alpha^{2,k}_i, \beta^{1,k}_i, \beta^{2,k}_i, \varrho_i^k, \Omega^k]$ represent user $i$'s \textit{performance feature vector} used for clustering. 
%For all stages, we assume that
%a hard assignment of users to clusters, that is, 
%a user can be assigned to only one cluster.
%
%We use line numbers of the algorithm inside yellow boxes to show the corresponding steps in Fig. \ref{flowchart}.
%To refer to the corresponding steps of the algorithm in Fig. \ref{flowchart}, we use line numbers inside yellow boxes in the figure.
%{General Description/Pseudo Code:}
%Consider the start of stage $k$.
%Let $\{s_{U,k,i}\}_{i=1}^N$ represent state features of $N$ users at stage $k$, as shown in the STD in Fig. \ref{flowchart}. %Let $\{X_i\}_{i=1}^N$ represent the features used for clustering users. 
%We obtain the state features of clusters as a functi the state features of users. %
%$\{X_{k,i}\}_{i=1}^N$. 
Let $c_{k,i}$ be the cluster of user $i$ at stage $k$, where $c_{k,i}\!=\! m \text{ } (m \in [1, \mathcal{C}]$), and $C_k \!=\! \{c_{k,i}\}_{i=1}^N$ is the set of all cluster assignments at stage $k$.
We define the cluster membership matrix, $\boldsymbol{\mathcal{M}}_k \in \{0, 1\}^{N \times \mathcal{C}}$, at stage $k$, such that $\mathcal{M}_{k, i, m} \!=\! 1$ if $m \!=\! c_{k,i}$, and 0 otherwise. %else 0. %(Initial cluster memberships ($\boldsymbol{\mathcal{M}}_1$) and clustering features $\textbf{X}$ will be described later in this section).
%and 0 otherwise. %(hard assignment).
%if user $i$ belongs to cluster $G_g$ at stage $k$, and $0$ otherwise.
%Let $\boldsymbol{\mathcal{M}}_k \in \{0, 1\}^{N \times \mathcal{G}}$ be the cluster membership matrix, where $\mathcal{M}_{k, ig} = 1$ if user $i$ belongs to cluster $G_g$ at stage $k$, and $0$ otherwise. %Let $X^{k}_i = [\alpha^{1,k}_i, \alpha^{2,k}_i, \beta^{1,k}_i, \beta^{2,k}_i, \varrho_i^k, \Omega^k]$ represent user $i$'s \textit{performance feature vector} used for clustering. 

%For all stages, we assume that
%a hard assignment of users to clusters, that is, 
%a user can be assigned to only one cluster.
%After this, we obtain the state features for the clusters  $\{s_{G,g,k}\}_{g=1}^\mathcal{G}$ as the average of the state features of its members. 
%Let $\{s_{G,k,g}\}_{g=1}^\mathcal{G}$ represent the state features of $\mathcal{G}$ clusters at stage $k$ obtained using the state features of users, as shown in line 6 of the Alg. \ref{cluster_based_policy}, and label F in Fig. \ref{flowchart}.
%\mahak{use the term interventions or actions?}
Algorithm \ref{cluster_based_policy} outlines our approach to learning a cluster-based policy ${\pi}_C$ parameterized by $\boldsymbol{\theta}$, %(initialized randomly), 
given simulated training data ($\{\textbf{s}_{U,k}\}_{k=1}^{K}$), initial cluster memberships ($\boldsymbol{\mathcal{M}}_1$), and user features ($\textbf{X}_1$) as input, with hyperparameters $\gamma, \eta_\theta, \eta_\phi, \delta$. % (described later). 
We first compute the state features of the clusters by averaging the state features of their associated members. Then, given the state features per cluster, we apply the current policy to obtain cluster-level actions $\textbf{a}_{C,z,k}$. %for tweets (\textbf{p}) and retweets (\textbf{q}). 
Next, we compute the cluster centroids and derive user-level actions $\textbf{a}_{U,z,k}$, based on the distance of the user to the centroids (see Alg.~\ref{GetUserInterventions}). 
%We normalize the user actions based on our budget constraint.  
Then we compute the expected reward based on the user-level actions (Alg.~\ref{GetExpectedReward}), and calculate user {\em payoff} and {\em contribution} features $\textbf{X}$ (described later) to recluster users into $\mathcal{C}$ clusters %$\{c_m\}_{m=1}^\mathcal{G}$ 
(see Alg.~\ref{UpdateClusters}). Finally, we update the policy parameters  $\theta$ by first computing the objective (see Alg.~\ref{GetTotalObjective}) based on the expected reward, and then using stochastic gradient descent with learning rates $\eta_\theta$ and $\eta_\phi$.
%
%We learn a policy function $\boldsymbol{\pi}_G$ that estimates interventions for the clusters given their state features. %i.e., $p_{G, \mathcal{T}, k}, q_{G, \Re, k} = \pi_G( s_{G,k})$, 
%corresponding to tweet and retweet intensities, respectively. %, as shown in line 7.
%maps the state features for the clusters $\pi_G: s_{G,k} \rightarrow p_{G, \mathcal{T}, k}, p_{G, \Re, k}$ to the interventions for the clusters, $p_{G, \mathcal{T}, k}, p_{G, \Re, k}$ corresponding to the tweet and retweet intensities, %i.e., $p_{G, \mathcal{T}, k}, p_{G, \Re, k} = \pi_G(s_{G,k})$. 
%After obtaining interventions for the clusters, 
%Then, we assign intervention estimated for the clusters to their respective members (users), %, and obtain interventions for the users 
%Then, we apply interventions for the clusters to their respective members, and impose a budget constraint.
%$p_{U, \mathcal{T}, k}, p_{U, \Re, k}$, as shown in line 9 of the Alg. \ref{cluster_based_policy}, and label G in Fig. \ref{flowchart}.
%After this, we obtain interventions for the users $p_{U, \mathcal{T}, k}, p_{U, \Re, k}$, using a function $\pi_U$ that assigns the intervention for the clusters to their respective members based on their variability from the cluster, i.e., $p_{U, \mathcal{T}, k}, p_{U, \Re, k} = \pi_U(p_{G, \mathcal{T}, k}, p_{G, \Re, k}|\mathcal{M}_k, X_k)$. 
%We obtain the interventions $a_{\mathcal{T},k}$ and $a_{\Re,k}$ to be added, respectively, to the tweet and retweet intensities of users, by imposing the budget constraint, in line 10. 
%Using interventions for the users, we compute the expected reward, and obtain clustering features to re-cluster users.
%Now, using the expected reward computed at the end of stage $k$, we obtain the features $X_{k+1}$ to cluster users for stage $k+1$. 
%Using these features along with the cluster centroids $Y_k$ at stage $k$, we re-cluster users for stage $k+1$, as shown in line 13.
%The above steps are repeated until we converge to a policy that maximizes our objective. 
%The policy function is parameterized by weights $\theta$ and $\phi$, that are initialized randomly. We update $\theta$ and $\phi$ using the total objective to be maximized, with learning rates $\eta_\theta$ and $\eta_\phi$, respectively.
%We compute the total objective to be maximized for learning optimal policy parameters $\theta$ and $\phi$. %, in line 15. 
%$\theta$ and $\phi$ are updated using stochastic gradient descent, with learning rates $\eta_\theta$ and $\eta_\phi$, respectively. 
The algorithm repeats until convergence and returns the final policy parameters and cluster memberships. 
%After running Alg. \ref{cluster_based_policy}, 
%In the end, we obtain converged clusters that are used to evaluate the learnt policy.
%We repeat the above steps for all stages, until we converge to a policy that maximizes our objective. 
We describe each component next. 

%\setlength{\textfloatsep}{1mm}
\begin{algorithm}[!t]
\caption{Dynamic Cluster-based Policy Learning and Optimization} 
\begin{algorithmic}[1]
\State \textbf{Input: $\{\textbf{s}_{U,k}\}_{k=1}^{K}, \boldsymbol{\mathcal{M}}_1, \textbf{X}_1, \gamma, \eta_\theta, \eta_\phi, \delta$}
%\State \textbf{Output: $\mathcal{M}^{*}$, $\theta^{*}$} 
%\State /* $\theta$ and $\phi$ are initialized randomly */
%\For {$e = 1, 2, ..., N_e$} /*episodes*/
%\State counter = 1, num\_skip\_stages = 1
\Repeat
    \For{$k = 1, ..., K$}
        %\State $s_{G,g,k} = (\sum\limits_{i=1}^N \mathcal{M}_{k, ig})^{-1} \sum \limits_{i=1}^N \mathcal{M}_{k,ig} s_{U,k,i}$, $\forall g \in [1, \mathcal{G}]$
        \State  {\small{/* Compute cluster state features */}}
        \State $\textbf{s}_{C,k,m} \!\!=\!\! \sum\limits_{i=1}^N \mathcal{M}_{k,i, m} \textbf{s}_{U,k,i}/\sum\limits_{i=1}^N \mathcal{M}_{k, i, m}$, $\forall m$
        %\State $s_{G,g,k} = \frac{\sum \limits_{i=1}^N \mathcal{M}_{k,ig} s_{U,k,i}}{\sum\limits_{i=1}^N \mathcal{M}_{k, ig}}$, $\forall g \in [1, \mathcal{G}]$ 
        %\State  {\small{/* Obtain cluster-level interventions */}}
        \State {\small{/* Get cluster-level actions */}}
        \State $\textbf{a}_{C, z, k} = \boldsymbol{\pi}_C(\textbf{s}_{C,k};\boldsymbol{\theta})$ 
        %\State $p_{U, \mathcal{T}, k}, p_{U, \Re, k} = \pi_U(p_{G, \mathcal{T}, k}, p_{G, \Re, k}|\mathcal{M}_k, X_k)$
        %\State $p_{U, z, k} = \pi_U(p_{G, z, k}|\mathcal{M}_k, X_k)$
        \State  {\small{/* Compute cluster centroids */}}
        %\State ${Y}_{G_g, k} = \frac{\sum\limits_{i=1}^N \mathcal{M}_{k,ig} {X}_{k,i}}{\sum\limits_{i=1}^N \mathcal{M}_{k,ig}}$, $\forall g \in [1, \mathcal{G}]$
        \State $\textbf{Y}_{k, m} = {\sum\limits_{i=1}^N \mathcal{M}_{k, i, m} \textbf{X}_{k,i}}/{\sum\limits_{i=1}^N \mathcal{M}_{k,i,m}}$, $\forall m$
        \State {\small{/* Obtain user-level actions with Alg. \ref{GetUserInterventions} ($\pi_U$) */}}
        \State $\textbf{a}_{U, z, k} = \pi_U(\textbf{a}_{C, z, k}, \textbf{X}_k, \textbf{Y}_k)$
        %\State {\small{/* Impose budget constraint by normalization */}}
        %\State $\textbf{a}_{d, k} = \frac{\textbf{p}_{d, k}}{||\textbf{p}_{d, k}||_1} \times C_{d,k}$ 
        \State $r_k$ = {\small{GetExpectedReward}}($\textbf{s}_{U,k}, \textbf{a}_{U, z, k}, \boldsymbol{\phi}, \gamma$)
        %\State Compute $\mathbb{E}[R^{k}(\textbf{s}^k, \textbf{a}^k, \boldsymbol{\vartheta}^k)]$  (Eq. \ref{expected_cumulative_reward})
        %\If {counter \% num\_skip\_stages == 0}
        %\State {\small{$\textbf{X}^{k+1}_i = (\alpha^{k+1}_i, \beta^{k+1}_i, \varrho^{k+1}_i, \Omega^{k+1}_i)$ (Eq. \ref{pf_past_feature}, \ref{user_expected_contribution_feature}) }}
        %\State ${Y}_{G_g, k} = (\sum\limits_{i=1}^N \mathcal{M}_{k,ig})^{-1} \sum\limits_{i=1}^N \mathcal{M}_{k,ig} {X}_{k,i}$, $\forall g \in [1, \mathcal{G}]$
        %\State ${X}_{k+1} = $ GetClusteringFeatures($a_{z, k}, a_{z, k-1}$)
        %\State ${X}_{k+1} =  f_C(a_{z, k}, a_{z, k-1})$
        \State {\small{Obtain}} $\textbf{X}_{k+1}$ {\small{using}} $\textbf{a}_{U, z, k}, \textbf{a}_{U, z, k-1}$ (Eq. \ref{pf_past_feature}, \ref{pf_user_expected_contribution_feature})
        \State $\boldsymbol{\mathcal{M}}_{k+1}$ = {\small{UpdateClusters}}($\textbf{Y}_{k}, \boldsymbol{\mathcal{M}}_k, \textbf{X}_{k+1}, \delta$) 
        %\State $V(s_{G,k})  = f(s_{G,k}; \phi)$ /* Value Function */
        %\State $\textbf{s}^{k'} = (\mathbb{E}[z^k], \mathbb{E}[\zeta^k], \mathbb{E}[\nu^k])$
        %\State $V(\textbf{s}^{k'}) = f(\textbf{s}^{k'}; \phi)$
        %\State $r^k = \mathbb{E}[R^{k}(\textbf{s}^k, \textbf{a}^k, \boldsymbol{\vartheta}^k)] + \gamma V(\textbf{s}^{k'})$
        %\EndIf
    \EndFor
    \State {\small{/* Learn Policy and update parameters */}}
    \State $ J_\theta, J_\phi$ = {\small{GetTotalObjective}}($\{r_k\}_{k=1}^K, \{\textbf{s}_{U,k}\}_{k=1}^K, \boldsymbol{\phi}, \gamma$)
    \State $\boldsymbol{\theta} = \boldsymbol{\theta} + \eta_\theta \boldsymbol{\nabla_\theta} J_\theta$, \: $\boldsymbol{\phi} = \boldsymbol{\phi} + \eta_\phi \boldsymbol{\nabla_\phi} J_\phi$
    %\State $\theta =$ ComputePolicyGradient($r_k, s_{G,k}, \eta_\theta, \eta_\phi$)
    %\State $\phi = \phi + \eta_\phi \nabla_\phi J_\phi$
    %\State $\mathcal{M}^1 = \mathcal{M}^{K_Tr}$ /* clusters obtained at the end of an epoch are used at the beginning of next epoch */
%\EndFor
\Until{$|\Delta \boldsymbol{\theta}| < \delta$} {\small{/* Convergence */}}
\State $\boldsymbol{\theta}^* = \boldsymbol{\theta}, \boldsymbol{\mathcal{M}}^{*} = \boldsymbol{\mathcal{M}}_{K}$%, $\phi^* = \phi$
\\\Return $\boldsymbol{\mathcal{M}}^{*}, \boldsymbol{\theta}^*$%, $\phi^*$
\end{algorithmic}
\label{cluster_based_policy}
\end{algorithm}


\subsubsection{State Features} \label{state_features}


%\mahak{bold for vectors/matrices?}
%We consider the number of events in the previous stage as features representing the state of the network at stage $k$, as also used in \cite{goindanisocial}.
%A common choice of features to parameterize point processes is the number of events in the previous stage (e.g. \cite{parikh2012conjoint}).%,\cite{qin2015auxiliary},\cite{farajtabar2017fake}.
%
%Thus, we use those to represent the network state. 
%We represent the user state $\textbf{s}_U$ as the number of events for different network activities \cite{parikh2012conjoint,qin2015auxiliary,farajtabar2017fake}, and compute the state features of the clusters $\textbf{s}_G$ by averaging the state features of their associated members. 
%To represent the state of the network at stage $k$, we use features based on the number of events in the previous stage (e.g. in \cite{parikh2012conjoint}).
%We represent the state of the network at stage $k$ as the number of events for different types of network activities (i.e. interactions) in the previous stage (e.g. \cite{qin2015auxiliary}).
We represent the network state $\textbf{s}_k \in \mathbb{R}^{dN}$ %(Sec. \ref{prob_def_fake_news})
at stage $k$ as the number of events for $d$ different network activities (i.e. interactions) in the previous stage (e.g. in \cite{qin2015auxiliary}).
Specifically, $s_{k,i,j}$ is the number of events for the $j^{th} (j \!\in\! [1,d])$ activity that user $i \!\in\! [1,N]$ has performed in stage $k\!-\!1$.
%
%The number of events in the past have been widely used to parameterize point processes (e.g. in \cite{farajtabar2017fake}).
%Let $z^T_{k,i}, z^F_{k,i}$ be the number of tweets, and $\zeta^T_{k,i}$, $\zeta^F_{k,i}$ be the number of retweets of user $i$ corresponding to true and fake news, respectively, during time $[\tau_{k-1}, \tau_k)$. 
%Specifically, $z^F_{k, i} = \mathcal{F}_i(\tau_{k+1}) - \mathcal{F}_i(\tau_{k})$,  $z^T_{k, i} = \mathcal{T}_i(\tau_{k+1}) - \mathcal{T}_i(\tau_{k})$, $\zeta^F_{k, i} = \Re^{F}_i(\tau_{k+1}) - \Re^{F}_i(\tau_{k})$, and $\zeta^T_{k, i} = \Re^{T}_i(\tau_{k+1}) - \Re^{T}_i(\tau_{k})$. 
%
%Let $n_{k, i}(t, c, z)$ represent the number of times user $i$ shares news in stage $k-1$. %, i.e. between time $[\tau_{k-1}, \tau_k)$. %, where $c$ = F or T, corresponding to fake or true news, and z = $\mathcal{T}$ or $\Re$, corresponding to tweet or retweet event. 
Let $n_{k, i}(h, z) = \mathcal{N}_i(\tau_{k}, h, z) \!-\! \mathcal{N}_i(\tau_{k-1}, h, z)$ represent the number of times user $i$ shares news in stage $k\!-\!1$, and $w_{k, i} = W_i(\tau_{k}) \!-\! W_i(\tau_{k-1})$ represent the number of likes received by user $i$. %in stage $k-1$.
%
%Let $s^{U,k}$ represent the state of the network at stage k, comprising of the state features of each user, that is $s^{U,k} = \{s^{U,k}_i\}_{i=1}^N$, where $s^{U,k}_i = (z^T_{k,i}, z^F_{k,i}, \zeta^T_{k,i}, \zeta^F_{k,i}, \nu^k_i)$.
%
Let $\textbf{s}_{U,k,i} = (n_{k, i}(T, \mathscr{T}), \break n_{k, i}(F, \mathscr{T}), n_{k, i}(T, \mathscr{R}), n_{k, i}(F, \mathscr{R}), w_{k, i})$ be the state feature for user $i$ that is input to Alg. \ref{cluster_based_policy}. %(Fig. \ref{flowchart}, `D').
%
We compute the state features for cluster $m$, at stage $k$, as the mean of the state features of its members %that is, $s_{G,g,k} = (\sum\limits_{i=1}^N \mathcal{M}_{k,ig})^{-1} \sum \limits_{i=1}^N \mathcal{M}_{k,ig} s_{U,k,i}$ (Alg. \ref{cluster_based_policy}, Line 6).
(Line 5, Alg. \ref{cluster_based_policy}). % of Alg. \ref{cluster_based_policy}.
%
Thus, there are $d=5$ network activities corresponding to
%Since we consider 
tweets (T/F), retweets (T/F), and likes, and
the dimensionality of the state representation 
is $5N$, which will be reduced to $5\mathcal{C}$ %$(\mathcal{C} \ll N)$ 
once we cluster users.% into $\mathcal{G}$ clusters.


\subsubsection{Reward}
%\mahak{updated reward to include sum over all users}
%As described in Sec.~\ref{prob_def}, number of exposures by time $t$ is given by $A_{.i} \cdot \mathcal{N}_{i}(t)$. Hence, the number of exposures in stage $k$ is given as $A_{.i} \cdot \mathcal{N}_{i}(\tau_{k+1}) - A_{.i} \cdot \mathcal{N}_{i}(\tau_{k})$.

The number of exposures by time $t$ is given by $\sum\nolimits_{i=1}^N \textbf{G}_{i,.} \cdot {\mathcal{N}}_i(t, h, z)$, which %in Thus, the number of exposures 
in stage $k$ is obtained as $\sum\nolimits_{i=1}^N [\textbf{G}_{i,.} \cdot {\mathcal{N}}_i(\tau_{k+1}, h, z) - \textbf{G}_{i,.} \cdot {\mathcal{N}}_i(\tau_{k}, h, z)]$, i.e. 
$\sum\nolimits_{i=1}^N \textbf{G}_{i,.} \cdot {n}_{k,i}(c,z)$. %, based on the state features described above.
Thus, the reward is:
%Using these, we can write, 

\begin{equation}\label{reward_eq}
\begin{aligned}
    R_z(\textbf{s}_{U,k}) %= \frac{1}{N} (\textbf{A} \textbf{n}_k(T, z))^\top \: \textbf{A} \textbf{n}_k(F, z) 
    = \frac{1}{N} (\textbf{n}_k(T, z))^\top \textbf{G}^\top \textbf{G} \: \textbf{n}_k(F, z)
\end{aligned}
\end{equation}

\noindent
%where $z = \mathcal{T}$ or $\Re$ indicates tweet or retweet event. 
%
%\subsubsection{Cumulative Reward due to Tweets and Retweets}
%
%We have separate intensities for tweet and retweet events, and the set of people reached by a user $i$'s tweet is different than those reached when user $j$ retweets user $i$. Thus, we consider a weighted sum of reward due to tweet and retweet events.
%As observed in \cite{vosoughi2018spread}, the spread of fake news is more due to retweets than tweets, we consider the cumulative reward $R$ as a weighted sum of the reward due to tweets and retweets, respectively. 
%\noindent Since, retweets are prominent in news diffusion compared to tweets (Sec. \ref{related_work}), 
\iffalse
The cumulative reward $R$ due to tweets and retweets is, %a weighted sum of the reward due to tweets and retweets, as follows. 

\vspace{-3mm}
\begin{equation}\label{cumulative_reward}
    %R^k(\textbf{s}^k) = \Finv \: \eth^k(\textbf{s}^k) + \aleph^k(\textbf{s}^k)
    R(\textbf{s}_{U,k}) = \: R_{\mathscr{T}}(\textbf{s}_{U,k}) + R_{\mathscr{R}}(\textbf{s}_{U,k})
\end{equation}
\vspace{-3mm}
\fi

%\noindent where $\zeta$ is the relative importance of reward from tweet activities compared to retweet activities.
%
%

\subsubsection{Objective} \label{objective}

%Our objective is to determine the amount of intervention to be applied to the tweet and retweet intensities for true news diffusion such that the expected reward is maximized. 
%We want our policy to have a have long-term impact, and therefore, we consider both immediate and future rewards. Additionally, the influence of a post diminishes with time, in online social networks \cite{farajtabar2015_event_prioritization}, implying that reward from recent stages is more important than that from further/later stages in time. Since, our reward is based on number of exposures to a post, we use the discounted rewards setting. 
Our goal is to learn a cluster-based policy $\pi_C$ to determine the interventions to be applied to users, at each stage, for true news diffusion process such that the total expected discounted reward for all stages, %$\mathbb{E}[\sum\limits_{k=0}^{K} \gamma^k R^{k+1}]$ = 
$J = \sum\limits_{k=1}^{K} \gamma^{k} \mathbb{E}[R(\textbf{s}_{U,k}, \textbf{a}_{U, \mathscr{T}, k}, \textbf{a}_{U, \mathscr{R}, k})]$ is maximized, where $\gamma \!\in\! (0,1]$ is the discount rate. %, used to assign relatively more importance to the immediate rewards than the future rewards.
%Specifically, we learn interventions such that the total expected discounted reward for all stages, $J = \sum\limits_{k=0}^{K-1} \gamma^{k} \mathbb{E}[R^{k}(s^k, \textbf{a}^k, \boldsymbol{\vartheta}^k)]$ is maximized, where $\gamma \in (0,1]$ is the discount factor used to assign relatively more importance to the immediate rewards than the future rewards. 
%
%Note that $a_{z, k}$ are actions in the MDP, where the space of all possible actions is given by ${O}^k = \{\textbf{a} \in R^N, \boldsymbol{\vartheta} \in R^N | \textbf{a} \geq 0, ||\textbf{a}||_1 = C_1^k\, \boldsymbol{\vartheta} \geq 0, ||\boldsymbol{\vartheta}||_1 = C_2^k\}$.
We map the interventions to actions in MDP. %\mahak{include this or not?: MDP based methods consider immediate as well as future rewards obtained on applying the policy, which is important for our policy to have a long-term impact.} 
%
We impose a budget constraint on the total amount of intervention that can be applied to all users i.e. $||\textbf{a}_{U,z,k}||_1 = B_{z,k}$, where $B_{z,k}$ is the total budget at stage $k$ %, as shown in 
(Line 8, Alg. \ref{GetUserInterventions}).
\iffalse
Thus, the space of all possible actions is given by $\textbf{A}_k = \{\textbf{a}_{U,z,k} \in R^N | \textbf{a}_{U,z,k} \geq 0, ||\textbf{a}_{U,z,k}||_1 = B_{z,k}\}$, where $B_{z,k}$ is the total budget at stage $k$. \mahak{$R^N$?}
\fi
%
Using Eq. \ref{reward_eq}, we can write,

\begin{equation} \label{expected_reward_eq}
\begin{aligned} 
    \mathbb{E}[R_z(\textbf{s}_{U,k}, \textbf{a}_{U, z, k})] = 
    %\frac{1}{N} \mathbb{E}[(\textbf{n}_k(T, z))^\top \: \textbf{A}^\top \textbf{A} \: \: \textbf{n}_k(F, z)]
     \frac{1}{N} \mathbb{E}[\textbf{n}_k(T, z)]^\top \: \textbf{G}^\top \textbf{G} \: \: \mathbb{E}[\textbf{n}_k(F, z)] \nonumber
\end{aligned}
\end{equation}

%Under the assumption that the diffusion of fake and true news is independent, we can decompose the expected reward due to these.
\noindent We assume that the diffusion of fake and true news is independent, and thus, decompose the expected reward. %\footnote{See \href{https://www.dropbox.com/s/ipqkhawu0joweel/Supplementary_Material_AAMAS_2020.pdf?dl=0}{Supplementary Material} for more details on $\mathbb{E}[\textbf{n}_k(c, z)]$.}  
%due to these. 
See \cite{farajtabar2017fake} for more details on %computation of
$\mathbb{E}[\textbf{n}_k(h, z)]$.
%for fake and true news diffusion processes due to our assumption of independence (Sec. \ref{problem_definition}). 
%Using Eq. \ref{cumulative_reward}, we calculate, 
The cumulative expected reward due to tweets and retweets is, $\mathbb{E}[R(\textbf{s}_{U,k}, \textbf{a}_{U, \mathscr{T},k}, \textbf{a}_{U, \mathscr{R},k})] =   \mathbb{E}[R_{\mathscr{T}}(\textbf{s}_{U,k}, \textbf{a}_{U, \mathscr{T}, k})] 
    + \mathbb{E}[R_{\mathscr{R}}(\textbf{s}_{U,k}, \textbf{a}_{U, \mathscr{R}, k})]$.
    
%\mahak{removed the equation, and added in the paragraph. It is referred in Alg 3 (getExpectedReward)}

\iffalse
\vspace{-3mm}
\begin{equation}\label{expected_cumulative_reward}
\begin{aligned} 
    %R^k(\textbf{s}^k) = \Finv \: \eth^k(\textbf{s}^k) + \aleph^k(\textbf{s}^k)
    \mathbb{E}[R(\textbf{s}_{U,k}, \textbf{a}_{U, \mathscr{T},k}, \textbf{a}_{U, \mathscr{R},k})] =  \: \mathbb{E}[R_{\mathscr{T}}(\textbf{s}_{U,k}, \textbf{a}_{U, \mathscr{T}, k})] 
    \\ + \: \mathbb{E}[R_{\mathscr{R}}(\textbf{s}_{U,k}, \textbf{a}_{U, \mathscr{R}, k})]
\end{aligned}
\end{equation}
\vspace{-4mm}
\fi


\subsubsection{Clustering Features} \label{clustering_features}

%To incorporate this, 
We design clustering features based on %based on the idea of 
{\em Difference Reward} (DR) %\cite{devlin2014potential} 
that use a user's contribution to \textit{shape} the reward signal and reduce noise in policy estimates. %This also helps to determine an efficient incentive allocation strategy under budget constraints.
%We want our clusters to determine how effective it is to provide incentive to a particular user given the contribution of other users under the policy applied.
%
%\noindent
%In lines 3 and 4 of Algorithm \ref{GetClusteringFeatures},
We define \textit{payoff} features that indicate how responsive a user is to the policy applied in the past, by measuring the change in a user's expected reward %of user $i$, 
after applying policy in stage $k-1$.
%$p_{z, k, i}$ ($z = \mathscr{T}, \mathscr{R}$) as the change in the expected reward of user $i$, after applying policy in stage $k-1$ . %We use these as indicators to determine 
%These indicate the likelihood that a user will utilize the incentive provided.
%This indicates whether providing incentive to a user was beneficial in the past or how likely a user will utilize the incentive provided based on her past actions.
%This indicates how responsive a user is to the policy applied in the past.
%
%We use the change in a user's contribution in the expected reward separately, due to tweet events and retweet events.
%
%Payoff measures the change in the expected reward of user, after applying policy in previous stage, %We use these as indicators to determine


\begin{equation}
%\vspace{-1mm}
\begin{aligned}
    p_{z, k,i} = \mathbb{E}_i[R_z(\textbf{s}_{U,k-1}, \textbf{a}_{U, z, k-1})] - \mathbb{E}_i[R_z(\textbf{s}_{U,k-2}, \textbf{a}_{U, z, k-2})]
\end{aligned} \label{pf_past_feature}
\end{equation}

\noindent
%effectiveness of a user in maximizing the reward, given the actions of other users.
We define \textit{contribution} features $q_{z, k,i}$ %($z = \mathcal{T}, \Re$) % and $\Omega_{\Re, k,i}$, 
to measure user $i$'s contribution in the expected reward, given the actions of other users. %due to tweet and retweet events, respectively.
%We measure the contribution of a user $i$ as 
Specifically, we calculate 
the difference in the total expected reward obtained on providing incentive to the user, to when no incentive is provided to the user. To compute the latter, we set the incentive for user $i$ as $0$. 
%
%Most of the Difference based reward shaping methods calculate the contribution of a user by subtracting the Reward obtained when all users apply the same policy, but one user is not applied any policy ($a_i^k = 0$), from the reward obtained when all users receive the incentive. 
%

%\begin{equation}
\begin{align}
    %& \varrho^{k}_i = \mathbb{E}[\eth^{k-1}(s^{k-1}, {a}^{k-1})] - \mathbb{E}[\eth^{k}(s^{k-1}, (\overline{a}_{-i}^{k-1}); a_i^{k-1} = 0)]  \\
    %& \Omega^{k}_i = \mathbb{E}[\aleph ^{k-1}(s^{k-1}, {\vartheta}^{k-1})] - \mathbb{E}[\aleph^{k}(s^{k-1}, (\overline{\vartheta}_{-i}^{k-1}); \vartheta_i^{k-1} = 0)] 
    q_{z, k, i} &= \mathbb{E}_i[R_z(\textbf{s}_{U,k-1}, \textbf{a}_{U, z, k-1})]  \label{pf_user_expected_contribution_feature}
    \\ &- \mathbb{E}_i[R_z(\textbf{s}_{U,k-1}, (\{{a}_{U, z, k, j}\}_{j=1, j \neq i}^N; a_{U, z, k-1, i} = 0))] \nonumber
\end{align} 
%\end{equation}

\noindent 
%where $\overline{\textbf{a}}_{U, z, k, -i} = \{{a}_{U, z, k, j}\}_{j=1, j \neq i}^N$.
\iffalse
where $\overline{a}_{U, z,k,j} = B_{z,k} \: \Tilde{a}_{U, z, k, j} (\sum\limits_{j=1;j \neq i}^N \Tilde{a}_{U, z, k, j})^{-1}$,\\ $\overline{\textbf{a}}_{U, z, k, -i} = \{\overline{a}_{U, z, k, j}\}_{j=1, j \neq i}^N$  
%$\overline{\vartheta}_{-i}^{k} = \{\overline{\vartheta}^{k}_j\}_{j=1, j \neq i}^N$ ; $\overline{\vartheta}_{j}^{k} = C_2^{k} \cdot {\varphi_{j}^{k}} ({\sum\limits_{j=1;j \neq i}^N \varphi_{j}^{k}})^{-1}$, 
%where $p^k, \varphi^k = \pi(s^{k-1};\theta)$, 
and $\boldsymbol{\Tilde{a}}_{U, z, k}$ is %the outputs of the policy function approximator, corresponding to 
the value of intervention action obtained %for the tweet and retweet intensities, respectively, 
before applying the budget constraint.
%that is the output of the Neural Network, before applying the budget constraint.
%
\fi
Thus, the complete set of features used for clustering users at the start of stage $k$ is %$\textbf{X}^k_i = (\alpha^{k}_i, \beta^{k}_i, \varrho^{k}_i, \Omega^{k}_i), i \in [1, N]$. 
$\textbf{X}_{k,i} = (p_{\mathscr{T},  k,i}, p_{\mathscr{R}, k,i}, \break  q_{\mathscr{T}, k,i}, q_{\mathscr{R}, k,i}), i \in [1, N]$. The similarity between two users $i$ and $j$ is based on the Euclidean distance between their respective feature vectors $\textbf{X}_{k,i}$ and $\textbf{X}_{k,j}$. 
%Clustering users with the above defined features allows the global reward and agent contributions to be used to learn a joint policy more efficiently than independent learning. 
%With these, we can use the past performance of a user to guide her policy learning in the future. %Note that we do not have the values of these features at the beginning of the first stage, since we do not have any policy estimates learnt before stage 0 (the start of the training procedure). 
%
%
%Our idea is to include each user's \textit{payoff} and \textit{contribution} as latent features to cluster users, that are input to the policy function approximator. %In this way, we are able to perform and help in joint policy learning, and is more efficient than %learning a separate policy function for each user, as is performed in the DR based reward shaping techniques. And, we can avoid
%In this way, we are able to perform efficient joint policy learning, described next, and avoid learning a complex policy function for each user %based on their individual contribution
%as in the standard reward shaping techniques.
%
We do not know the policy estimates apriori for the first stage, and 
%use features based on empirical reward in the Training Data to 
obtain initial clusters $C_1$ and membership $\boldsymbol{\mathcal{M}}_1$, using K-means++, %\cite{arthur2007k},
based on empirical rewards computed from training data. 
%We used K-Means++ with Euclidean distance as the similarity measure 
%(Fig. \ref{flowchart}, Arrow 2).
%we cannot compute the values of expected reward in the previous or the current stages, and thus, 
%we cannot use these features to obtain the initial clusters at the beginning of the first stage. 
%we use a modification of the above features to obtain the initial clusters. %, that we describe next. 
%
%Hence, we obtain the initial clusters and memberships $\mathcal{M}^0$, using Training Data. %data from the first $K_{P}(=10)$ stages that was used to learn the parameters for the MHPs. 
%We calculate the above defined features using the empirical reward rather than expected reward. 
This captures the \textit{natural policy}  %of users in the social network, that is, the 
or intrinsic behavior
of users to spread news, without external incentives. %We use K-means++ \cite{arthur2007k} to obtain initial clusters.
%
We incorporate the DR signals as input to the policy function approximator (via clustering features), rather than using them as explicit shaped reward signal that is different for each agent. %in output. 
This helps to %facilitate efficient joint policy learning, and 
avoid learning a separate model for each user %(that is impractical for large number of users) 
as in the standard DR shaping techniques (e.g. \cite{devlin2014potential}).

%
%\setlength{\textfloatsep}{2mm}
\begin{algorithm}[!t]
\caption{GetUserInterventions ($\pi_U$)}
\begin{algorithmic}[1]
\State \textbf{Input: $\textbf{a}_{C, z, k}, \textbf{X}_k, \textbf{Y}_k$} 
%\State \textbf{Output: $p_{U, \mathcal{T}, k}, p_{U, \Re, k}$} 
    \State {\small{Let $c_{k,i}$ be the cluster to which user $i$ belongs to, at stage $k$.}} %, i.e. $\mathcal{M}_{k,i,{g_{k,i}}} = 1$
    \\ {\small{/* Incentive per user for Tweet MHP */}}
    \State $\Tilde{a}_{U, \mathscr{T}, k, i} = a_{C, \mathscr{T}, k, {c_{k,i}}} ||\textbf{X}_{k,i} - \textbf{Y}_{k, {{c_{k,i}}}}||_2$, $\forall i \in [1,N] $
    %\\{{/* Incentive, per pair of users for retweets */}}
    \State {$\alpha_{U, \mathscr{R}, k, i, j} \!=\! a_{C, \mathscr{R}, k, {{c_{k,i}}, {c_{k,j}}}}  ||\textbf{X}_{k,i} \!\!-\! \textbf{Y}_{k, {{c_{k,i}}}}||_2  ||\textbf{X}_{k,j} \!\!-\! \textbf{Y}_{k, {{c_{k,j}}}}||_2$,} {$\forall i,j \in [1,N] $} {\small{/* Incentive, per pair of users for retweets */}}
    \\{\small{/* Weighted average to get incentive per user for Retweet MHP */}} %\mahak{changed the above comment to include weighted average}
    \State $\Tilde{a}_{U, \mathscr{R}, k, i} =  \frac{1}{N} \sum\limits_{j=1}^N \alpha_{U, \mathscr{R}, k, i, j} \Phi_{\mathscr{R}, ji}$, $\forall i \in [1,N] $ 
    %\State $a_i^k = C_1^k p_i^k (||p^k||_1)^{-1}$
    %\State $\varkappa^k_{ij} = C_2^k \varphi^k_{ij} (||\varphi^k||_1)^{-1}$
    %\State {{/* Impose budget constraint by normalization */}}
    \State $\textbf{a}_{U, z, k} = \frac{\boldsymbol{\Tilde{a}}_{U, z, k}}{||\boldsymbol{\Tilde{a}}_{U, z, k}||_1} \times B_{z,k}$  {\small{/* Budget Constraint */}}
\\\Return $\textbf{a}_{U, z, k}$ %$\textbf{a}_{U, \mathcal{T}, k}, \textbf{a}_{U, \Re, k}$
\end{algorithmic}
\label{GetUserInterventions}
\end{algorithm}
%

\subsubsection{Learning Cluster-based Policy} \label{policy_learning}

%\vspace{1mm}
%\noindent \underline{\emph{Application of Policy and Actions to Users}}

%\subsubsection{Policy Learning and Optimization}


%\subsubsection{Reward}
%\mahak{move to prob def}

%
%After this, we learn the actions of the users by first learning the actions for the clusters. 
%The idea/Our insight is that users belonging to the same cluster have similar performance (behavior), and therefore, will have similar actions, and we can apply \textit{similar} policies to the users of the same cluster. $\{s_{G,k,g}\}_{g=1}^\mathcal{G}$
Given cluster-level state features $\textbf{s}_{C,k}$, our goal is to learn a cluster-based policy %$\pi_G: s_{G,k} \rightarrow p_{G, \mathcal{T}, k}, p_{G, \Re, k}$, 
parameterized by $\theta$, i.e., $\textbf{a}_{C, \mathscr{T}, k}, \textbf{a}_{C, \mathscr{R}, k} \!=\! \pi_C(\textbf{s}_{C,k}; \boldsymbol{\theta})$.
$\{a_{C, \mathscr{T}, k, m}\}_{m=1}^\mathcal{C}$ is learned for each cluster $C_m$ and corresponds to the incentive for increasing the tweet activities of its members, and $\{a_{C, \mathscr{R}, k, m, {m^\prime}}\}_{m,m^\prime = 1}^\mathcal{C}$ is learned for each \textit{pair} of clusters $(m, {m^\prime})$ and indicates how much to incentivize a user of cluster $m$ to retweet the posts of a user in cluster ${m^\prime}$. %, corresponding to true news diffusion. 
%We use a neural network to approximate the policy function $\pi^G$.

%We represent the policy %$\textbf{a}^{k+1}$ as a function of state ($s^k$), parameterized by weights $\theta$, that is, $\textbf{a}^{k+1} = \pi(s^k; \theta)$, where $\pi$ is the function we want to learn. 
The value of the network state $\textbf{s}_{U,k}$ %is associated with a value,  %$V(\textbf{s}_{U,k})= \mathbb{E}[\sum\limits_{j=k}^K  \gamma^j R_j|(\textbf{s}_{U,k}, \pi_C, \pi_U)]$, 
%which 
is the total expected reward when in the given state following policies $\pi_C, \pi_U$, i.e. $V(\textbf{s}_{U,k}) = \mathbb{E}[\sum\limits_{j=k}^K  \gamma^j R_j|(\textbf{s}_{U,k}, \pi_C, \pi_U)]$. 
Since it is computationally expensive to compute $V(\textbf{s}_{U,k})$ from future rewards for every possible policy, we approximate the value as a function of the state parameterized by weights $\boldsymbol{\phi}$, i.e. $V(\textbf{s}_{U,k}) = f(\textbf{s}_{U,k}; \boldsymbol{\phi})$, as in \cite{kurutach2018model}. % \cite{zheng2018drn}
%
Policy gradient methods are more effective in high dimensional spaces, and can learn continuous policies. Thus, we use %state-of-the-art 
advantage actor-critic algorithm (e.g. \cite{schulman2015high_A2C}). % to find the optimal policy. 
%The details are presented in Algorithm \ref{training_algo}.

Let there be $K$ stages in the Simulated Training Data (STD) (Fig. \ref{flowchart}). Given state features at the beginning of stage $k$ (i.e. at time $\tau_k$), we learn policy function $\pi_C$ to obtain actions to be applied during stage $k$ (i.e. time-interval $[\tau_{k}, \tau_{k+1})$), using a multi-layer feed-forward neural network (NN) (see \cite{goindanisocial} for details on NN).
%Given state features for stage $k$, we learn policy function $\pi_G$ to be applied for stage $k+1$, using a multi-layer feed-forward neural network. %to learn this policy $\pi_G$. 
%
%Let $G_{g^k_i}$ be the cluster of user $i$ at stage $k$.
%(Alg. \ref{ApplyPolicyToUsers}, line 3).
%We obtain the cluster of user $i$ in line 3 of Alg . 
%The intervention for the tweet intensity for user $i$, $p^k_i$, and the estimate of incentive provided to user $i$ to retweet posts of user $j$ is obtained as,
%
%The intervention for the tweet intensity for user $i$ is estimated as $p^k_i = \dot{p}^k_{G_{g^k_i}} \: ||X^k_i - {Y}^k_{G_{g^k_i}}||^2$, and the estimate of incentive provided to user $i$ to retweet posts of user $j$ is obtained as,
%estimate for additional intensity with which user $i$ should retweet the posts of user $j$ is obtained as 
%$\varphi^k_{ij} = \dot{\varphi}^k_{G_{g^k_i}, G_{g^k_j}} \: ||X^k_i - {Y}^k_{G_{g^k_i}}||^2 \: ||X^k_j - {Y}^k_{G_{g^k_j}}||^2 $. 
%
%After we get the incentives for the clusters, we obtain the interventions for their respective members using a function $\pi_U$ described in Algorithm \ref{ApplyPolicyToUsers}. %based on their \textit{variability} from the cluster. 
% $p_{G, \mathcal{T}, k}, p_{G, \Re, k}$
%
%
%i.e., $p_{G, \mathcal{T}, k}, q_{G, \Re, k} = \pi_G( s_{G,k})$, 
%corresponding to tweet and retweet intensities, respectively.
We find intervention actions for the clusters, $\textbf{a}_{C, \mathscr{T}, k}, \textbf{a}_{C, \mathscr{R}, k} = \pi_C(\textbf{s}_{C,k})$, corresponding to tweet and retweet intensities, respectively, as output of the NN %\footnote{See \href{https://www.dropbox.com/s/ipqkhawu0joweel/Supplementary_Material_AAMAS_2020.pdf?dl=0}{Supplementary Material} for neural network architecture.}
%, shown in 
(line 7 of Alg. \ref{cluster_based_policy}). %and `F' in Fig. \ref{flowchart}. 
%Due to space constraints, we describe the architecture for NN in Supplementary Material. 
Then, in line 11, we obtain actions for users $\textbf{a}_{U, z, k}$ based on their \textit{variability} from their cluster, using Alg. \ref{GetUserInterventions}.
%, described in Alg. \ref{ApplyPolicyToUsers}. %This helps to capture the variability of the users from their respective clusters.
%In this way, we obtain the interventions for the users based on their \textit{variability} from their cluster.
%
%Lines 3, 4 and 5 in 
%Specifically, 
%
Alg. \ref{GetUserInterventions} computes the actions for the users by weighting the cluster actions by their distance to the centroid in lines 4 and 5. %show the computation of the interventions for the users as . %weighted by their distance to the cluster centroid,  that captures the \textit{variability} of users from their clusters. 
%that we compute as follows.
This helps to capture both similarity and variability in user behaviors.
%Let $\{\textbf{Y}^k_{G_g}\}_{g=1}^{\mathcal{G}}$ be the respective centroids of the $\mathcal{G}$ clusters at stage $k$, calculated using the performance features $\textbf{X}^{k}_i$, as $\textbf{Y}_{G_g}^k = (\sum\limits_{i=1}^N \mathcal{M}^k_{ig})^{-1} \sum\limits_{i=1}^N \mathcal{M}^k_{ig} \textbf{X}^k_{i}$.
%
%The cluster to which user $i$ belongs to, at stage $k$, is given by $G_{g^k_i}$, %where $g^k_i$ such that $\mathcal{M}^k_{i{g^k_i}} = 1$ 
%
%After this, we impose the budget constraints to obtain the amount of incentive to be added at stage $k$, to user $i$'s tweet intensity for true news diffusion (Eq \ref{true_news_tweet_intensity}) as $a_i^k = C_1^k p_i^k (||p^k||_1)^{-1}$, and the incentive to be provided to user $i$ to retweet user $j$'s posts
%additional intensity with which user $i$ should retweet the posts of user $j$ 
%(Eq \ref{true_news_retweet_intensity}) is obtained as $\varkappa^k_{ij} = C_2^k \varphi^k_{ij} (||\varphi^k||_1)^{-1}$.
%
Since retweets involve an interaction between pair of users, 
we consider incentives $\alpha_{U, \mathscr{R}, k, i,j}$ for each pair of users, where $\alpha_{U, \mathscr{R}, k, i,j}$ is the amount of incentive provided to user $i$ to retweet user $j$'s posts. However, due to high computational cost, we do not want to model an $N^2$-dimensional MHP for retweet activities. So instead, to reduce it to an $N-$dimensional MHP, we compute the weighted average of incentive actions %, i.e. $a_{U, \mathscr{R}, k, i} = \sum\limits_{j=1}^N \alpha_{U, \mathscr{R}, k,i,j} \: \Phi_{\mathscr{R}, ji}/N$ 
in line 7.
We normalize user actions based on our budget constraint in line 8. %(Sec. \ref{objective}).
%
%After this, we impose the budget constraint by normalizing, in line 12  of Alg. \ref{cluster_based_policy}, to obtain interventions $\textbf{a}_{z,k}$ %(Fig. \ref{flowchart}, `G') 
%that are used to compute the expected reward, %(Fig. \ref{flowchart}, `H'), 
%in line 13 of Alg. \ref{cluster_based_policy}. 
%
%Alg. \ref{GetExpectedReward} describes the computation of expected reward using cluster memberships obtained in stage $k$. 
Then, we compute the expected reward using these actions, %obtained for stage $k$,
as described in Alg. \ref{GetExpectedReward},
\iffalse
We compute the expected state features for users $\textbf{s}_{U, k^\prime}$ in line 3, obtained after applying the policy, %functions $\pi_G$ and $\pi_U$, %Using $s_{U, k^\prime}$, we obtain the expected state features for clusters $s_{G, k^\prime}$ in line 5,
and find the value of expected next state $V(\textbf{s}_{U, k^\prime})$ in line 4. $r_k$ represents the expected reward that is obtained by applying actions $\textbf{a}_{U, z,k}$ in state $\textbf{s}_{U,k}$, in line 5, that comes from the Bellman Optimality Equation. %\cite{bellman1957markovian_MDP}.
\fi
%the Bellman Optimality Equation \cite{bellman1957markovian_MDP}.
%We learn a policy function $\dot{\pi}: \dot{s}^{k} \rightarrow \dot{p}^k, \dot{\varphi}^k$, parameterized by weights $\dot{\theta}$, i.e., $\dot{p}^k, \dot{\varphi}^k = \dot{\pi}(\dot{s}^{k}; \dot{\theta})$, where, 
%\dot{p}^k \in \mathbb{R}^\mathcal{G}$ and $\dot{\varphi}^k \in \mathbb{R}^{\mathcal{G} \times \mathcal{G}}$ corresponds to the incentive for tweet and retweet intensity, respectively, for true news diffusion. 
%
%Exposure is defined in terms of the number of people reached by a post. 
%
%\setlength{\textfloatsep}{0pt}
\begin{algorithm}[!t]
\caption{GetExpectedReward}
\begin{algorithmic}[1]
\State \textbf{Input: $\textbf{s}_{U,k}, \textbf{a}_{U, z, k}, \boldsymbol{\phi}, \gamma$} 
%\State \textbf{Output: $r_k$} 
        \State Compute $\mathbb{E}[R_{k}(\textbf{s}_{U,k}, \textbf{a}_{U, z, k})]$ (Sec. \ref{dynamic_cluster_based_policy}, `Objective') %(Eq. \ref{expected_cumulative_reward}) 
        \State $\textbf{s}_{U, k^\prime} = (\mathbb{E}[\textbf{n}_k(h, \mathscr{T})], \mathbb{E}[\textbf{n}_k(h, \mathscr{R})], \mathbb{E}[\textbf{w}_k])$ %(Sec. \ref{objective})
        %\State $s_{G,g,k^\prime} = \frac{\sum \limits_{i=1}^N \mathcal{M}_{^\prime,ig} s_{U,k^\prime,i}}{\sum\limits_{i=1}^N \mathcal{M}_{k^\prime, ig}}$, $\forall g \in [1, \mathcal{G}]$
        \State $V(\textbf{s}_{U,k^\prime}) = f(\textbf{s}_{U,k^\prime}; \boldsymbol{\phi})$
        {\small{\State $r_k = \mathbb{E}[R_{k}(\textbf{s}_{U,k}, \textbf{a}_{U, \mathscr{T}, k}, \textbf{a}_{U, \mathscr{R}, k})] + \gamma V(\textbf{s}_{U, k^\prime})$}
        %\mahak{Bellman Optimality Eq}
        }
\\\Return $r_k$
\end{algorithmic}
\label{GetExpectedReward}
\end{algorithm}
%
%\setlength{\textfloatsep}{0pt}
\begin{algorithm}[!t]
\caption{GetTotalObjective}
\begin{algorithmic}[1]
\State \textbf{Input: $\{r_k\}_{k=1}^K, \{\textbf{s}_{U,k}\}_{k=1}^K, \boldsymbol{\phi}, \gamma$} %\mu, \Phi, \chi, \omega %
%\State \textbf{Output: $J_\theta, J_\phi$} 
%\State Initialize $\theta$ and $\phi$ randomly.
    \State $L_\theta = 0$, \: $L_\phi = 0$
    \For{$k = 1, ..., K$}
        \State $V(\textbf{s}_{U,k}) = f(\textbf{s}_{U,k}; \boldsymbol{\phi})$ {\small{/* Value Function */}}
        \State Let $D_k = \sum \limits_{j=k}^{K} \gamma^k r_k$ {\small{/* Total Discounted Reward */}}
        \State $B_k = D_k - V(\textbf{s}_{U,k})$ {\small{/* Advantage Function */}}
        \State $L_\theta = L_\theta +  B_k$; \hspace{2mm} $L_\phi = L_\phi +  ||V(\textbf{s}_{U,k}) -  D_k||_2 $
    \EndFor
    \State $ J_\theta = L_\theta $, \: $J_\phi = - L_\phi $
    %\State $\nabla_\phi J_\phi = - L_\phi $
\\\Return $J_\theta, J_\phi$
\end{algorithmic}
\label{GetTotalObjective}
\end{algorithm}
%
and the total objective for optimizing policy $\pi_C$ in Alg. \ref{GetTotalObjective}.
\iffalse
In Alg. \ref{GetTotalObjective}, we describe the computation of the total objective function used for optimizing policy $\pi_C$,
using the advantage function \cite{schulman2015high_A2C} that helps to reduce variance.
\fi
%Instead of simply using the expected reward for optimization, we use an advantage function that is obtained by subtracting the value of the state as baseline from the expected reward. This helps reduce variance. % in estimates.
%
%Lines 5-7 show the computation of advantage function for each state $s^k$. 
%Lines 4-6 show the computation of the total objective function that is used to update the policy parameters, $\boldsymbol{\theta}$ and $\boldsymbol{\phi}$. 
%In lines 20-21, we learn the optimal parameters $\theta$ and $\phi$, initialized randomly, using stochastic gradient descent, with learning rates $\eta_\theta$ and $\eta_\phi$, respectively.
%We want to find $\theta^* = \arg \max_\theta J_\theta$, where $J_\theta = \sum \limits_{k=1}^K \gamma^k E[A^{k}]$. 
%The value function that we approximated must be close to the expected reward for that stage under policy $\pi$, hence, we use squared difference between $x^k_\phi$ and $D^k$ to find the optimal parameters $\phi$ for value function. 
%\jen{does the NN also predict the state values as well? is it parameterized by $\theta, \phi$? Why doesn't it show in Alg 2?} \mahak
%{We use the same NN to learn policy $\pi$ and $f$, but they use different parameters and are independent, as shown in the figure in appendix. We can also use a different NN to estimate value, some people use shared and some people use a different one. The only thing common in between them is the state.}
%since the input state $s$ is common to both, 
%however the parameters are learnt independently of each other. 
%\jen{I don't see the MHPs refered to in Alg 2. I also don't see any ref to initializing the values of $\theta,\phi$. Shouldn't you output both?} \mahak{For evaluating the policy, we don't need $\phi$. $\theta,\phi$ are randomly initialized. We do not refer to the MHPs in algo, we need the parameters like $\Phi, \mu, \psi$. The expected value of z and $\nu$ need these parameters}.
%

%\setlength{\textfloatsep}{1mm}
\begin{algorithm}[!t]
\caption{UpdateClusters}
\begin{algorithmic}[1]
\State \textbf{Input: $\textbf{Y}_{k}, \boldsymbol{\mathcal{M}}_k, \boldsymbol{X}_{k+1}, \delta$} 
%\State \textbf{Output: $\mathcal{M}_{k+1}$} 

    \State Let $\boldsymbol{\ddot{Y}}_{k+1} = \textbf{Y}_{k}$, $\boldsymbol{\mathcal{M}}_{k+1} = \boldsymbol{\mathcal{M}}_k$
    \Repeat
        \State Let $\boldsymbol{\dot{y}} = \boldsymbol{\ddot{Y}}_{k+1}$ {\small{/* Centroids in previous iteration */}}
        %\\ {\small{/* Compute centroids using features for stage k+1 */}}
        \State $\boldsymbol{\dot{Y}}_{k+1, m} =  (\sum\limits_{i=1}^N \mathcal{M}_{k+1,i,m} \textbf{X}_{k+1, i}) / (\sum\limits_{i=1}^N \mathcal{M}_{k+1,i,m})$ 
        %\State $\dot{Y}_{G_g, k+1} = \frac{\sum\limits_{i=1}^N \mathcal{M}_{k+1,ig} X_{k+1, i}}{\sum\limits_{i=1}^N \mathcal{M}_{k+1,ig}}$
        %\\ {\small{/* Weighted centroid for stage k+1 */}}
        \State $\boldsymbol{\ddot{Y}}_{k+1, m} = \varepsilon_1 \boldsymbol{\dot{Y}}_{k+1, m} + \varepsilon_2 \textbf{Y}_{k, m}$
        \State $m_i = \arg \max \limits_{m = 1}^\mathcal{C} || \textbf{X}_{k+1,i} - \boldsymbol{\ddot{Y}}_{k+1, m}||^2$ %{\small{/* Closest cluster to user $i$*/}}
        \State $\mathcal{M}_{k+1, i, m_i} = 1$, and $\forall m \neq m_i, \mathcal{M}_{k+1,i,m} = 0$
    \Until{$||\boldsymbol{\dot{y}} - \boldsymbol{\ddot{Y}}_{k+1}||_2 < \delta$} {\small{/* Convergence */}}
\\\Return $\boldsymbol{\mathcal{M}}_{k+1}$
\end{algorithmic}
\label{UpdateClusters}
\end{algorithm}

%\vspace{1mm}
%\noindent \underline{\emph{Updating Cluster Centroids and Assignments}}
\subsubsection{Update Clusters}

Using actions $\textbf{a}_{U, z,k}$ learnt for stage $k$, we calculate the clustering features (Eq. \ref{pf_past_feature}-\ref{pf_user_expected_contribution_feature}) for the next stage, $\textbf{X}_{k+1}$. %$\textbf{X}^{k+1}_i = (\alpha^{k+1}_i, \beta^{k+1}_i, \varrho^{k+1}_i, \Omega^{k+1}_i), i \in [1, N]$.
Due to application of the policy, $\textbf{X}_{k+1,i}$ is different from $\textbf{X}_{k,i}$. Thus, we need to re-compute the centroids and cluster memberships.
%Due to these changes in feature values, the centroids of the clusters will change from those in stage $k$, and need to be re-computed for stage $k+1$. 
%Now, if we recalculate the centroids, then we need to re-assign the users to the clusters based on the updated centroids, and repeat this until the centroids and cluster assignments do not change. %Note that this is similar to the re-calculation of centroids and re-assignment of points (users) until convergence in the K-Means++ algorithm. 
%
%Recall that we need to cluster users at each stage in order to capture the dynamically changing users' performance based on their actions in the past stages. Now, since the cluster assignments and centroids change at each stage, the challenge is to \textit{align} the clusters across different stages so that the policy function approximater can estimate meaningful policy for each cluster, that is, it can align the policies and weights learnt for the clusters across multiple epochs to improve the policy estimates using stochastic gradient descent (SGD). 
%
%As explained above that due to the change in user performance/behavior as a result of the application of the policy, there will be a change in the cluster memberships, and therefore, the cluster centroids will change. 
%However, we do not want the centroids to change much in order to align the clusters across different stages. 
Additionally, we want the clusters to be aligned across different stages, so that
the policies can be optimized using the neural network, for different clusters across multiple epochs.
%the policy function approximator can align the policies for different clusters across multiple epochs to improvise them using gradient descent (GD).
%This is required so that the policy function approximator can align the policies for different clusters across multiple epochs to improvise them using stochastic gradient descent (SGD).
To achieve this, we define \textit{weighted centroids} that include the effect of centroids in the previous stage. % $k$ to cluster users in stage $k+1$. 
This helps to ensure that the centroids do not shift much and thus, we can
align clusters in stage $k+1$ with those in stage $k$. 
Alg. \ref{UpdateClusters} shows the steps to update clusters.
%Rephrase better: The idea behind using the weighted centroids to re-assign users to clusters is that we are able to use the information from previously converged cluster assignments and centroids to align the clusters for the next stage. Otherwise the centroids will shift, and we cannot ensure alignment between clusters.
%
%We propose a joint clustering approach to align the clusters across different stages, and simultaneously update the cluster assignments and centroids until convergence as follows. 
%
%
%For stage $k+1$, we start with the 
For clustering at stage $k+1$, we begin with the memberships from stage $k$ (line 2). This helps in faster convergence of clusters. % for stage $k+1$, since the clusters at stage $k$ are already converged.
Using $\textbf{X}_{k+1}$, we obtain the updated centroids $\boldsymbol{\dot{Y}}_{k+1, m} \forall m \in [1, \mathcal{C}]$ for stage $k+1$ (line 5). We define $\mathcal{C}$ \textit{weighted centroids} $\boldsymbol{\ddot{Y}}_{k+1, m} = \varepsilon_1 \boldsymbol{\dot{Y}}_{k+1, m} + \varepsilon \textbf{Y}_{k, m} \forall m \in [1, \mathcal{C}]$, (line 6), $\varepsilon_1 + \varepsilon_2 = 1$. $\varepsilon_1$, $\varepsilon_2$ indicate the importance assigned to the centroids from the previous stage and the current stage, respectively.
After updating the centroids, we update the membership matrix and repeat until  convergence. %, using threshold $\delta$ (line 9). 
%
%Specifically, there is less change in the cluster assignments and centroids in epoch $e^\prime + 1$ from those in epoch $e^\prime$, when $e^\prime$ is close towards convergence.
Additionally, since the change in policy estimates  across epochs reduces as optimization gets closer to convergence, %of policy optimization
the clustering features (which are dependent on these estimates) do not change much for the same stages across such epochs and we can start to reuse the learned clusters. % from  stage $k^\prime$ of epoch $e^\prime$ as the clusters for stage $k^\prime$ in epoch $e^\prime + 1$, without re-clustering users for any stage of epoch $e^\prime + 1$. 
%running the clustering algorithm for any stage of epoch $e'+ 1$.  
%Thus, we can obtain faster convergence of the clusters at each stage for the subsequent epochs by using the converged clusters obtained in stage $k'$ at epoch $e'$ as the clusters for stage $k'$ in epoch $e' + 1$.
%
%This idea of updating of cluster assignments across epochs is similar to
Similar to simulated annealing, we only update the cluster assignments every $\eta_e \in \mathbb{Z}^{+}$ epochs gradually increasing $\eta_e$ as the epoch number increases, which helps speed up convergence of policy learning.
%
%Thus, as the policy parameters $\theta$ move towards the saddle point, we expect less change in cluster memberships and thus, use the already converged clusters for the subsequent epochs as described above.
%thus faster convergence. 

%\mahak{where to include the converged clusters that are output of Alg 1. }

%The features for stage $0$ are based only on the base intensity of the users.

%The convergence of clusters at each stage is faster towards the saddle point of the policy optimization due to smaller change in policy parameter $\theta$, and thus, it takes less number of iterations for the convergence of centroids and cluster memberships as compared to the initial epochs. %when we randomly initialize the policy parameter $\theta$ and gradually update it every epoch in SGD. 
%This is because the performance features used for clustering depend on the policy learnt and as the policy estimates become better (converge) towards approaching the saddle point, the performance features of the users do not change much for the same stages across epochs. Due to this, the users will get assigned to the same clusters across epochs and we can use the same clusters from the previous epochs to learn the policies in the current epochs that are closer towards convergence. %leading to faster convergence of cluster centroids and memberships. 


\subsection{POLICY EVALUATION}


Since the Simulated Evaluation Data (SED) %(Fig. \ref{flowchart}, `I') 
is conditioned on STD, we use the clusters converge at the end of the policy learning %and thus, use those for 
to evaluate the estimated policy. %(Fig. \ref{flowchart}, Arrow 6).
This helps to avoid re-clustering at each stage of evaluation, and reduce running time for online evaluation. %that is high due to the simulation of MHPs for both tweet and retweet events, with large number of users.
%We use such assumption 
%This assumption is also justified 
%Moreover, the duration of our evaluation phase is not large enough so that the user behavior changes steeply and thus, we can avoid re-clustering users while running the policy online.
%
%To evaluate the learned policy, 
First, we find intervention actions %(Fig. \ref{flowchart}, `J')
for the network state obtained from events in SED. %We add the interventions, respectively, to the base exogenous intensities, $\mu^T$ and $\wp^T$ of the tweet and retweet intensities for true news diffusion, and measure performance using the following evaluation metric. 
%
%Now, we describe the setup for evaluating the policy learnt using the above clustering approach. perform an on-policy evaluation
Then, we generate events by simulating MHPs after adding interventions to the base intensities for true news diffusion, %(Fig. \ref{flowchart}, Arrow 5, `K'),
and use those to compute the following evaluation metric.
%To assess the learnt policy, we calculate the following evaluation metric.
%

\iffalse
To evaluate the estimated policy $\hat{\pi}_G$, we simulate data again from the MHPs. %for $K$ stages corresponding to time $[\tau_{2K+1}, \tau_{3K})$, that is conditioned on the last stage of STD (arrow 4, label I). 
Using the final clusters $G_K$, we obtain actions from the policy to add to the MHP intensity functions and generate evaluation data to assess empirical reward.
\fi



%\paragraph{Evaluation Metric}
%\vspace{1mm}
%\noindent \underline{\emph{Evaluation Metric}}
\subsubsection{Evaluation Metric}

%\mahak{Shorten this, and say that we use the same eval metric as in previous paper?}
%To evaluate different methods, we consider reward %\cite{farajtabar2017fake} %(Fig. \ref{flowchart}, `L') 
%and the fraction of users exposed to fake news that become exposed to true news \cite{goindanisocial}.  

% we multiply the reward by the fraction of users exposed to fake news that become exposed to true news (i.e. users who get mitigated) since evaluating different methods solely based on reward is not sufficient, and a better model is the one that mitigates more distinct number of users.
Comparing different methods solely based on reward (e.g. \cite{farajtabar2017fake}) does not suffice, and a better model is the one that mitigates more distinct number of users \cite{goindanisocial}.
%A better model is the one that mitigates more distinct number of users. 
Thus, instead of considering only the reward as in previous work (e.g. \cite{farajtabar2017fake}), 
we multiply the reward by the the fraction of users exposed to fake news that become exposed to true news, as also used in \cite{goindanisocial}.
%We use the same evaluation metric as in \cite{goindanisocial}, that considers the reward and the fraction of users exposed to fake news that become exposed to true news. 
This helps to assign more importance to the selection of distinct users over selection of few users with high exposures. Specifically, performance $\mathcal{P}$ is given as $\sum\limits_{k=1}^K R_k \times \frac{|L_{T,k} \cap L_{F,k}|}{|L_{F,k}|}$, where $L_{T,k} = \{i| i \in [1, N], \textbf{n}_{k}(T,z) \cdot \textbf{G}_{.i} > 0\}$ and $L_{F,k} = \{i|i \in [1, N], \textbf{n}_{k}(F,z) \cdot \textbf{G}_{.i} > 0\}$ are the sets of users exposed to true and fake news, respectively, during stage $k$. %In order 
%To assess the gains by making interventions, the performance of a method is measured relative to that obtained by applying no intervention. %, by computing the difference between the performance after applying the learned policy and that without applying a policy. Note that we cannot explicitly test if there is a reduction in fake news spread since we cannot make real-time interventions. %in online social networks.














==> ARXIV_Dynamic Cluster-based Policy Learning for Social RL/05-experiments.tex <==
\section{EXPERIMENTS}

We use real-world datasets, Twitter 2016 and Twitter 2015 \cite{ma2017detect_twitter_2016_2015,liu2018early}, with 749 and 2051 users, respectively. 
%Similar to \cite{goindanisocial},
%We observed that in our data around 75\% of the news last for 40 hours, so 
We consider time-horizon $\mathcal{T} = 40$, divided into 40 stages of $\Delta T = 1$ hour each. 
%
%We use the first 10 stages to estimate parameters for MHPs characterizing tweet, retweet and like events, using the same approach as in \cite{goindanisocial} and \cite{lemonnier2017multivariate}. 
%Due to space limitation, we provide more details on parameter estimation and choice of $\omega$ in the Supplementary Material. 
%
%We use the same setting for training and evaluation as in 
%Similar to \cite{goindanisocial}, we use data from first 10 stages (time $[0, 10$) to estimate parameters and obtain initial clusters that are used at the beginning of the training phase. We use the data from time $[T_{P}(= 10), T_{Tr}(= 20))$ ($[K_{P}(=10), K_{Tr}(=20))$ stages) as the \textit{training dataset} for simultaneously clustering users and learning interventions.
%We use the data from time $[T_{Tr}(= 20), T_{Te}(= 30)]$ ($[K_{Tr}(=20), K_{Te}(=30))$ stages) as \textit{evaluation dataset} to evaluate the learnt policy by measuring reward. We use data from time $[T_{Te}(= 30), T(= 40)]$ ($[K_{Te}(=30), K_{Tr}(=40))$ stages) as \textit{held-out dataset} to compute the effectiveness of users selected by the model/algorithm to spread true news.
%
%We use the data from time $[0, 10)$ as Training Data. STD corresponds to time $[10, 20)$, SED before and after applying interventions corresponds to time $[20, 30)$, and the data from time $[30, 40)$ is used as Held-Out Data.
The Training Data, STD, SED before and after applying interventions, and Held-Out Data (Fig.~\ref{flowchart}), respectively, correspond to time-intervals, $[0, 10)$, $[10, 20)$, $[20, 30)$, and $[30, 40)$.
%
We use ``tick" python library \cite{2017arXiv170703003B_tick} to perform
simulations of MHPs. %We used $C_1^k, C_2^k \sim N \cdot \mathcal{U}(0,1)$, and $\gamma = 0.7$.  
We consider $O_{z,k} \sim N \cdot \mathcal{U}(0,1)$, and $\gamma = 0.7$, as in \cite{goindanisocial, farajtabar2017fake}. 
\iffalse
We follow the same approach as in \cite{goindanisocial} to obtain the values of kernel decay parameter $\omega_{c,z}$. %for the different processes used to model user activities in real-world social networks. 
Specifically, we obtain, ($\omega_{F, \mathscr{T}} = 0.7, \omega_{T, \mathscr{T}} = 0.85$), ($\omega_{F, \mathscr{R}} = 0.35, \omega_{T, \mathscr{R}} = 0.65$) for Twitter 2016, and ($\omega_{F, \mathscr{T}} = 0.8, \omega_{T, \mathscr{T}} = 0.95$), ($\omega_{F, \mathscr{R}} = 0.45, \omega_{T, \mathscr{R}} = 0.75$) for Twitter 2015, and $\omega_{\mathscr{L}}=1$.
\fi

%Algorithm \ref{training_algo_cluster} describes our policy learning and optimization approach along with clustering as an intermediate model/framework for reducing the dimensionality of both state and action spaces by combining users based on similar performance. %Fig. \ref{flowchart} shows a flowchart showing the major steps involved in our algorithm. 

%\subsubsection{Comparison of tweet and retweet intensities}

%\mahak{move the fig to supplementary?}\jen{yes}
First, we test whether news diffusion patterns via tweet and retweet events are similar in the Twitter data. 
Fig. \ref{comparison_base_intensity_tweet_retweet_2015} shows a comparison of the distribution of respective base intensities across all users. 
%Notably, we observe differences in the distribution of base intensities across users, which indicate it is important to consider separate processes for tweet and retweet events , as mentioned in Sec. \ref{intro_ch_2}.
%We find that more number of users have higher retweet intensities for fake news, compared to true news. Also, the distribution of retweet intensities has more variance compared to tweet intensities. 
%These observations are consistent with \cite{vosoughi2018spread}, and indicate that it is important to consider separate processes for tweet and retweet events, as mentioned in Section \ref{intro}.
We observe differences in the distribution of base intensities, which %indicates it is important 
supports our approach
to consider separate network activities (tweet and retweet) to characterize different types of agent interactions. 
%processes for tweet and retweet activities in the social network, as mentioned in Sec. \ref{related_work}.
%as shown in 
%Fig \ref{comparison_base_intensity_tweet_retweet_2016} and \ref{comparison_base_intensity_tweet_retweet_2015} show the distribution for intensities for both fake and true news diffusion. %on Twitter 2016. %We obtained similar distributions on Twitter 2015.



\iffalse
\begin{figure}[!t]
%\hbox{
\subfloat[Fake News]{\includegraphics[scale = 0.23]{figures/tweet_retweet_base_intensity_2016_density_distribution_fake_news.png}}
\hspace{1ex}
\subfloat[True News]{\includegraphics[scale = 0.23]{figures/tweet_retweet_base_intensity_2016_density_distribution_true_news.png}}
%\caption{Performance on Synthetic Data}
%}
%\vspace{-3mm}
\caption{Tweet and Retweet Intensities for Twitter 2016}
\label{comparison_base_intensity_tweet_retweet_2016}
%\vspace{-6mm}
\end{figure}
\fi
%

\begin{figure}[!t]
\hbox{
\subfloat[Fake News]{\includegraphics[scale = 0.23]{figures/tweet_retweet_base_intensity_2015_density_distribution_fake_news.png}}
%\hspace{1ex}
\subfloat[True News]{\includegraphics[scale = 0.23]{figures/tweet_retweet_base_intensity_2015_density_distribution_true_news.png}}
%\caption{Performance on Synthetic Data}
}
\caption{Distribution for Tweet and Retweet Intensities}
\label{comparison_base_intensity_tweet_retweet_2015}
%\vspace{-5mm}
\end{figure}
%

\subsection{BASELINES}

In our best knowledge, our approach \textbf{\MethodName}, is the first to consider policy learning while dynamically clustering users in MARL for social networks and there are no other alternative dynamic approaches to compare to. We designed a dynamic Rule-based clustering approach, which uses thresholds to (re)group users, to use as a baseline for comparison. But it was always outperformed by \MethodName and since it’s a naive baseline, we did not include it due to space limit. %We can include in the final version for completeness.
%
%We did compare to KM-S, which corresponds to existing STATIC clustering methods (el Hassouni et al 2018, Zhu et al 2018), and observed that C-PF outperforms it since it does not capture dynamic user behavior. 
%
%We compare to non-clustering methods that consider all users to be in a single cluster and learn same policy for all (NC-1), and those that assume each user to be in a separate cluster and learn different policies (NC-N, NC-TR, NC-PF).
Thus, we compare to the static clustering methods \cite{zhu2018group, el2018personalization}, and the non-clustering methods that have also been used in \cite{zhu2018group, el2018personalization}, as described below. 

%The number of clusters for each method are determined using Bayesian Information Criterion and Within-Cluster Sum of Squared Distances. %, and the detailed scree-plots are shown in the Supplementary Material. 
%We consider $\mathcal{G} = 9$ for C-PF, based on scores of Bayesian Information Criterion (BIC) and Within-Cluster Sum of Squared Distances (WC-SSD).
\iffalse
We compare our model, called \textbf{C-PF}, against different baselines described below.
%We also evaluate the clusters obtained and more details including choice of $\mathcal{G}$, evaluation of cluster alignment across different stages, and other Experimental Settings are provided in the Supplementary Material.
We use Bayesian Information Criterion, and Within-Cluster Sum of Squared Distance, to select number of clusters $\mathcal{G}$\footnote{See \href{https://www.dropbox.com/s/ipqkhawu0joweel/Supplementary_Material_AAMAS_2020.pdf?dl=0}{Supplemental} for details on the choice of hyper-parameters $\mathcal{G}$, 
$\gamma$, $C_z$, $\omega$, $\varepsilon$.}.
%We provide the values of budget constraint $C_z$, discount factor $\gamma$
\fi

%\mahak{compare against other approaches for dim. reduction such as PCA or matrix factorization?}

%We propose the following baselines to compare the performance o
%We compare the performance of our approach with the following baselines. For the baselines that perform clustering, the state features for clusters are taken as the average of the state features of its members, similar to that in C-PF.

\iffalse
\subsubsection{RB-PF}
%\subsection{RB-PF}

We propose a rule-based method to group users, using clustering features in C-PF, based on some rules and thresholds. See Supplementary Material for more details. 

\fi
%\mahak{no dynamic baseline?}
%We use the reward based features to group users into 9 groups. We take two features, weighted difference in expected reward between stages, and the difference reward at the current stage. Then we use thresholds to decide the high, medium, and low performing groups of users for both features, and accordingly form 9 groups by taking intersection of the high and low performing group of users corresponding to the two reward features. After this, at every stage we group the users again to determine the policy. 

%As an alternative to clustering users at every stage, we propose a rule-based approach that groups users based on some rules, explained as follows. After every stage, we compute the \textit{performance features} same as those used in C-PF. We take a weighted average of the features based on user's past performance and user's expected contribution, for both tweet and retweet events. Specifically we compute $f_1^k = \iota_1 \alpha^k + \iota_2 \varrho^k$, and $f_2^k = \iota_1 \beta^k + \iota_2 \Omega^k$, where $\iota_1$ and $\iota_2$ are the weights (we take $\iota_1 = \iota_2 = 0.5$ for simplicity). 
%At stage $k$, we compute features $f_1^k$ and $f_2^k$ for all users, and assign them into three groups, for each feature, using the 25-th and 75-th percentile of the feature values. We call the users with features values greater than the 75-th percentile as high-performing, those with features values less than the 25-th percentile as low-performing, and the remaining as moderate-performing.
%Using the three groups for the two features, we obtain 9 groups by taking intersection of different combinations of the group type (high, moderate, low). After this, we obtain the state features for these groups and learn optimal interventions using the same procedure used in our `Clustering Model'. 
%Note that we can use this approach to dynamically group users, as the clusters will be automatically aligned based on the threshold, that is the clusters will remain fixed based on the thresholds (the groups represent users whose feature values are greater than the threshold), but the users can move between the groups when their performance (feature values) changes as a result of the policy applied. 
%In RB-PF, there is no need to worry about the issue of convergence as in the clustering based approaches. 

%\subsubsection{Same policy for all users (NC-1)}

\noindent \underline{\emph{Non-Clustering Methods}}

\paragraph{NC-1}

No Clustering. All users in same cluster ($\mathcal{C} = 1$). %(same policy for all users)

%We consider all users to belong to a single cluster($\mathcal{G} = 1$), and learn the same policy for all users. %(Performance is similar to the AVG policy learnt previously). %We do not have to cluster users after every stage in this case.

%\subsubsection{Separate policy for all users with identical post events (NC-N)}
\paragraph{NC-N}

MHP-U model in \cite{goindanisocial}: Identical actions learnt for tweet and retweet activities. Each user is in a separate cluster i.e. $\mathcal{C} = N$. We primarily compare to NC-N since %it has already been shown to 
it outperforms different non-clustering approaches (eg. \cite{farajtabar2017fake}).

%\subsubsection{Separate policy for all users with separate tweet and retweet events (NC-T-R)}
\paragraph{NC-TR}

Separate actions learnt for tweet and retweet activities (for true news diffusion), and $\mathcal{C} = N$.


%\subsubsection{Reward Features in State Representation (NC-PF)}
\paragraph{NC-PF}

%($\mathcal{G} = N$), and 

Same as NC-TR, but with clustering features (Eq. \ref{pf_past_feature}, \ref{pf_user_expected_contribution_feature}) added in the state representation of users, and $\mathcal{C} = N$.


\noindent \underline{\emph{Clustering Based Methods}}

%\subsubsection{Random Clustering (RND)}
\paragraph{RND}

Randomly assign users to $\mathcal{G}$ static (fixed) groups. %The same groups are considered for all stages. 

%\subsubsection{Clustering with Network Features (C-NET)}
\paragraph{C-NET}

Clusters obtained using K-Means++ with network features (degree, closeness centrality, clustering coefficient). %to obtain clusters.

%\subsubsection{K-Means++ with Reward Features (KM-R)}
\paragraph{KM-R}

%K-Means++ with reward based features from TD, 

\iffalse
We use initial clusters $G_1$ (Sec. \ref{clustering_features}),
%We use the same initial clusters, obtained using K-Means++, that are based on the empirical reward described in our Clustering Model. 
%The clusters remain fixed and 
however, do not update these dynamically along with policy learning. 
\fi
%This helps to test how good are the initial clusters obtained, and how much gain in performance can be achieved based on the initial clusters alone. 
%
%This helps to determine the gain in performance based on the initial clusters alone. %The number of clusters obtained is 9 and 8, respectively, for Twitter 2016 and 2015. 

Static Clusters are obtained using K-Means++ with empirical reward features, and are not updated dynamically.

%\subsubsection{K-Means++ with State and Reward Features (KM-S)}
\paragraph{KM-S}

\cite{el2018personalization, zhu2018group}.
%Clusters are obtained using K-Means++ with state and reward features from TD, and remain fixed, similar to \cite{el2018personalization}, \cite{zhu2018group}.
Static Clusters as in KM-R, but state features are also used for clustering.

\iffalse
In our best knowledge, our approach C-PF is the first to consider policy learning while dynamically clustering users in MARL for social networks and there are no other alternative dynamic approaches to compare to. We designed a dynamic Rule-based clustering approach, which uses thresholds to (re)group users, to use as a baseline for comparison. But it was always outperformed by C-PF and since it’s a naive baseline, we did not include it due to space limit. %We can include in the final version for completeness.
%
%We did compare to KM-S, which corresponds to existing STATIC clustering methods (el Hassouni et al 2018, Zhu et al 2018), and observed that C-PF outperforms it since it does not capture dynamic user behavior. 
%
%We compare to non-clustering methods that consider all users to be in a single cluster and learn same policy for all (NC-1), and those that assume each user to be in a separate cluster and learn different policies (NC-N, NC-TR, NC-PF).
Thus, we compare to the static clustering methods \cite{zhu2018group, el2018personalization}, and the non-clustering methods that have also been used in \cite{zhu2018group, el2018personalization}.
We primarily compare to NC-N \cite{goindanisocial} since %it has already been shown to 
it outperforms different non-clustering approaches (eg. \cite{farajtabar2017fake}).
%Since the method in \cite{goindanisocial} outperforms \cite{farajtabar2017fake}, we do not compare our proposed method against the latter.
%\mahak{Rule-Based?}
%Similar to KM-R, but we also use state features along with the reward features, to obtain initial clusters. 
%This helps to assess if the state features provide any additional information, apart from the performance features, in forming clustering so as to improve performance. 
%\cite{el2018personalization} and \cite{zhu2018group} also use state and reward features from historical data to obtain clusters that remain fixed. The number of clusters obtained is 9 for both Twitter 2016 and 2015.

\fi

\iffalse
\vspace{-1mm}
\subsection{Number of Clusters ($\mathcal{G}$)} \label{choosing_num_clusters}
\fi

%For our clustering model, we need to decide the number of clusters, and we use 
%We assume the number of clusters to be fixed, and provide a justification in the following subsections. To choose the appropriate number of clusters we use Bayesian Information Criterion (BIC) \cite{schwarz1978estimating} and Within Cluster Sum of Squared Distance (WC-SSD). More details are provided in the Supplementary Material.
The input to the policy function approximator (Sec. \ref{policy_learning}) %comprises of the state features for each cluster. The NN 
requires input and output of fixed dimensions, and hence, we assume fixed number of clusters $\mathcal{C}$. We use the scores of Bayesian Information Criterion, and Within Cluster Sum of Squared Distance to
select $\mathcal{C}$ for each clustering-based method. %(sum, over all clusters, of sum of squared euclidean distance between all points within a cluster).
%The input to the policy function approximator is fixed, and thus we need to  
%
%Since, we do not have apriori information about the dataset or ground truth for optimal clusters, we use the Bayesian Information Criterion (BIC) \cite{schwarz1978estimating} and the Within Cluster Sum of Squared Distance (WC-SSD) to find the appropriate number of clusters based on the explained variance. We provide the details regarding BIC and WC-SSD in the Supplementary Material. 
%
%We use the BIC \cite{schwarz1978estimating} to decide the number of clusters for each group. Additionally, we verify the number of clusters chosen using the Within-Cluster Sum of Square Distance (WC-SSD). 
\iffalse
Fig. \ref{BIC_Scores} and \ref{WCSSD_Scores}, respectively, show a scree plot for the BIC and WC-SSD scores for different values of $\mathcal{C}$, for our cluster-based policy learning method, C-PF. 
\fi
Table \ref{num_clusters_all_methods} reports the number of clusters ($\mathcal{C}$) obtained for different baselines, and we observe
that $C \in \{8,9\}$ is similar for different methods. %, and %$C \sim \{8,9\}$
%for all methods. 
%that all methods have 
%can see that the
%optimal number of clusters are 9 and 8, respectively, for Twitter 2016 and 2015. 
%
\iffalse
\begin{figure}[!t]
\vspace{-5mm}
\hbox{
\subfloat[Twitter 2016]{\includegraphics[scale = 0.275]{figures/BIC_2016.png}}
\hspace{1ex}
\subfloat[Twitter 2015]{\includegraphics[scale = 0.275]{figures/BIC_2015.png}}
%\caption{Performance on Synthetic Data}
}
\vspace{-1mm}
\caption{BIC Scores for Different Number of Clusters ($\mathcal{G}$)}
\label{BIC_Scores}
\end{figure}
%
\begin{figure}[!t]
\vspace{-5mm}
\hbox{
\subfloat[Twitter 2016]{\includegraphics[scale = 0.275]{figures/WCSSD_2016.png}}
\hspace{1ex}
\subfloat[Twitter 2015]{\includegraphics[scale = 0.275]{figures/WCSSD_2015.png}}
%\caption{Performance on Synthetic Data}
}
\vspace{-1mm}
\caption{WC-SSD Scores for Different Number of Clusters ($\mathcal{G}$)}
\label{WCSSD_Scores}
\vspace{-4mm}
\end{figure}
%
\fi
%

\begin{table}[!b]
%\vspace{-1mm}
\centering
\caption{Number of Clusters ($\mathcal{C}$) for Different Methods}
\label{num_clusters_all_methods}
\scalebox{0.9}
{
%\hspace{-6mm}
\begin{tabular}{cccccc}
    \toprule
    & \textbf{\MethodName} & \textbf{KM-R} & \textbf{KM-S} & \textbf{C-NET} & \textbf{RND} \\
    \midrule
    Twitter 2016 & 9  & 9 & 9 & 8 & 9 \\
    Twitter 2015 & 8  & 8 & 9 & 8 & 9 \\
\bottomrule
\end{tabular}
}
\label{table_results}
\end{table}


\subsection{RESULTS}

%\vspace{-1mm}
%\subsection{Evaluation of Learned Policies} \label{learned_policy_eval}


%We study the change in performance of different methods as a function of network size, relative importance of tweets and retweet events, and kernel decay parameter in MHP, described as follows.


%\vspace{-1mm}
%\subsubsection{Network Size}


%
%
\begin{table}[t!]
%\vspace{-1mm}
\centering
\caption{Relative Performance (Mean $\pm$ Std. Error)}
\label{relative_perf_all_methods}
\scalebox{0.88}
{
%\hspace{-6mm}
\begin{tabular}{c|c|c|c}
    \toprule
  {} &  {} & \textbf{Twitter 2016} & \textbf{Twitter 2015} \\
    \midrule
    %\rowcolor{red!50}
    \rowcolor{Yellow}
   \textbf{Clustering} & {DCPL}  & \textbf{98.19} $\pm$ 1.52  &  \textbf{95.175} $\pm$ 1.75 \\
   \rowcolor{Yellow}
     %{RB-PF}  & 91.26 $\pm$ \textbf{1.31}  & 85.725 $\pm$ \textbf{1.53}  \\
   {Based} & {KM-R} & 81.28 $\pm$ 1.78  &  73.98 $\pm$ 1.64  \\
   \rowcolor{Yellow}
   {Methods} & {KM-S} & 78.63 $\pm$ 1.82  & 70.37 $\pm$ 1.69\\
   \rowcolor{Yellow}
    & {C-NET} & 64.07 $\pm$ 1.98  &  51.52 $\pm$ 1.72 \\
    \rowcolor{Yellow}
    & {RND} & 55.52 $\pm$ 4.23  &  42.17 $\pm$ 4.94\\
     %\rowcolor{red!50}
     \cmidrule{1-4}
     \rowcolor{Green}
   \textbf{Non-Clustering} &  NC-PF  & 87.39 $\pm$ 3.46  & 80.73 $\pm$ 3.72   \\
   \rowcolor{Green}
   {Methods} & {NC-TR} & 77.83 $\pm$ 3.37  &  62.76 $\pm$ 3.51 \\
   \rowcolor{Green}
   {} & {NC-N} & 67.04 $\pm$ 3.21  &  56.10 $\pm$ 3.48 \\
    \rowcolor{Green}
    & NC-1 & 58.68 $\pm$ 1.02  & 47.12 $\pm$ 1.10 \\
    \bottomrule
\end{tabular} 
}
\end{table}
%\mahak{reorganize the table by separating into clustering and non-clustering baselines?}

Table \ref{relative_perf_all_methods} shows the relative performance of different methods. \MethodName is able to achieve highest reward. Also, NC-TR outperforms NC-N, implying that it is beneficial to decouple the different network activities. The clustering-based methods achieve greater performance than non-clustering methods.

%In Fig \ref{all_baselines_combined}, we can see that the NC-T-R, NC-N, and NC-1 have lower performances, 
%thus indicating that it is better to group similar users and learn similar policies for them, as opposed to 
%The non-clustering baselines, NC-T-R, NC-N, and NC-1 achieve a lower performance compared to other clustering-based methods, 

%Separate policies learnt for each user in 
%The non-clustering methods 
NC-N, NC-TR, NC-PF have larger variance and noisy estimates due to high dimensionality of state/action space. %representation. 
%A single policy learnt for all users 
NC-1 has high bias as it doesn't consider differences in agent behavior. Clustering based approaches achieve lower variance, %is less than that for the non-clustering based approaches, 
%implying that clustering 
which indicates that they
overcome sparsity and curse of dimensionality. %as they are able to reduce the variance in estimates.
%helps to reduce the noise. %due to sparse interactions. %and %by reducing the dimensionality of the state and action spaces and  thus, 
%learn better policies. %This answers \textit{RQ3} that clustering users is beneficial. 
%Since, NC-1 is trivial and achieves lower performance, we do not consider it for further experiments. 
%Clustering based methods reduce the variance and noisy estimates as compared to the non-clustering methods, and thus, are able to learn better policies. 
%The results demonstrate that clustering users is beneficial as compared to no clustering, that is, either learning a single policy for all users (NC-1) or separately? learning different policies for users. A single policy learnt for all users has high bias as it doesn't take into account the varied user behavior. And, learning a different policy for all users has higher variance and noisy estimates due to huge dimensionality of the state features.  
%
%Clustering users into groups helps to learn better policies, as we are able to reduce the noise in estimates of users that was high due to the increased dimensionality of input and output space
%
%Since we reduce the dimensionality, we are able to get better estimates of actions that can be applied to similar people in the cluster. This is also supported by the observation that the variance in estimates of actions reduces.

%Among the approaches that cluster users, 
Moreover, \MethodName that updates cluster assignments dynamically based on the policy applied outperforms those that assume fixed assignments (KM-R, KM-S, C-NET, RND). 
%cluster users once and assume those to remain fixed throughout (KM-R, KM-RS, C-NET). 
Notably, NC-PF that does not perform clustering %, and learns separate policies for users 
also outperforms these, %methods that assume fixed clusters, 
as it adjusts policy based on dynamic agent behavior. %by including the user performance features in the state representation. %This implies that it is important to capture the effect of policies applied in the past for learning better policies in the future. 
Thus, we need features indicative of agents' \textit{payoff} and \textit{contribution}, apart from state features, to get more accurate %policy 
estimates.
%However, NC-PF is computationally inefficient (Fig. \ref{num_epochs})
%has huge computational complexity
%as the continuous state space becomes larger/blows due to additional features.
%Thus, dynamic clustering of users is beneficial as it is able to estimate better policies by including the performance features through clusters and reduce the input dimensionality to lower the computational cost.
%

%\mahak{move the following paragraph to supplementary?}
The performance of KM-R is slightly greater than KM-S, implying that reward based features alone are useful for learning better estimates,
%and including state features only increases the computational cost. 
%without considering state features to cluster users.
without state features.
%it is sufficient to use the reward based features alone for clustering users, without including the state features. 
%
%We also observe that the clustering approach based on network properties, 
%Although C-NET converges faster, 
%C-NET achieves lower performance than non-clustering baselines, %This implies that the network features alone are not able to differentiate users based on the amount of intervention needed. %by them to increase the spread of true news. %separate users %based on their likelihood of maximizing the objective by utilizing the incentive provided.
%well such that similar incentives can be provided to users in the same cluster.
%Our key insight for clustering users is to separate them based on the amount of incentive that needs to be provided such that they can utilize it to maximize the objective (spread more true news). Network features are not able to separate the users effectively such that the interventions learnt for the cluster can be provided to its members. 
%to determine the amount of incentive to be provided to each group of users. 
%Thus, we conclude that it is important to include features based on reward (obtained in the past or expected reward in the future) as a result of the policy applied so that the users within the same cluster are similar in terms of the amount of incentive needed to maximize the objective. %can be given the same amount of incentive. 
%
\iffalse
%Thus, we conclude that
C-NET achieves lower performance than non-clustering baselines,
indicating that not all features are useful in %obtaining clusters reflective of %user's contribution and/or 
%differentiating 
clustering users to reflect the amount of incentive needed. %by them. 
The reward based features in C-PF consider network structure implicitly, and are better indicators of users' payoff and contribution. %and contribution. %, compared to network features. %(eg. in C-NET).
%The latent features based on reward help in learning better policies along with reducing the computational cost.
\fi
Notably, C-NET method that uses network-based features performed poorly. This indicates that not all similarity measures are useful for obtaining \textit{good} clusters, i.e. ones that increase efficiency without reducing effectiveness. These results support the claim that features indicative of expected reward and agent contribution are likely to be more helpful.
%
%And, using network features explicitly for clustering doesn't help to improvise the policy.

%\subsubsection{Number of Epochs}

%
%\vspace{-2mm}
\begin{figure}[!t]
\hbox{
\subfloat[Twitter 2016]{\includegraphics[scale = 0.275]{figures/P_vs_num_epochs_2016.png}}
\hspace{1ex}
\subfloat[Twitter 2015]{\includegraphics[scale = 0.275]{figures/P_vs_num_epochs_2015.png}}
%\caption{Performance on Synthetic Data}
}
\caption{Number of Epochs until Convergence}
\label{num_epochs}
\end{figure}
%\mahak{include any static clustering based approach in the figure?}
%
%To answer \textit{RQ2}, we compare the time taken until convergence, in terms of the number of epochs, by different methods in Fig. \ref{num_epochs} 
%the clustering-based approaches with those by the baselines that learn interventions for all users without clustering. 
%Fig \ref{num_epochs} shows the number of epochs for methods that converge fastest and slowest among all alternatives. We can see that the clustering based approaches (C-PF, RB-PF) achieve greater performance across all epochs, and converge much faster than the non-clustering based approaches (NC-T-R and NC-PF) (that do not perform clustering). 
%
%Fig \ref{num_epochs} shows the number of epochs taken until convergence by different methods. 
Fig. \ref{num_epochs} shows a comparison of the time taken until convergence %(number of epochs) 
by different methods.
%We observe that 
\MethodName converges faster than NC-PF and NC-TR, and achieves a greater performance for all epochs. %that do not cluster users for policy learning, 
%
%The performance of K-R and NC-PF is similar, however, NC-PF takes much longer to converge. 
NC-PF outperforms KM-R and NC-TR, but takes longer to converge, implying that the reward-based features (Eq. \ref{pf_past_feature}, \ref{pf_user_expected_contribution_feature}) %help in increasing performance 
are useful if included in state representation, however, lead to increased computational cost. %due to higher dimensionality of state features.
%
%it takes longer to converge since the state representation grows larger. %with additional features.
%
%Thus, with the help of clustering with performance features, we are able to achieve faster convergence as the exploration over the action space is improved without increasing the state space 
In \MethodName, the information about agents' payoff and contribution via clusters, helps in better exploration over the action space without increasing the state space. This helps the model to learn agents' effectiveness early on and converge faster to better policy. %Without using any additional discriminating information about users (eg. in NC-T-R), the model takes higher number of epochs to determine \textit{useful} users (relative contribution of users) and converge to an efficient allocation strategy/policy. %, especially in the case of joint learning with shared state and actions space of all users.

The above results, based on reward, serve as preliminary proof of concept that providing incentives helps to mitigate the impact of fake news \cite{goindanisocial}. Since we cannot make real-time interventions, we also compare different methods by measuring the impact of nodes selected for intervention, in terms of the people they actually reached in the real Held-Out Data.
Let $S(\tau)$ refer to the the set of users \textit{selected} in SED ($\tau \in [20, 30)$) to spread true news by time $\tau$, according to the model, i.e., $S(\tau) = \{i|(\mathcal{N}_i(\tau, T, z) - \mathcal{N}_i(20, T, z)) > 0\}$, %\cup \{i|(\Re^{T}_i(\tau) - \Re^{T}_i(T_{Te})) > 0\}$, 
and the remaining users are considered \textit{missed} ($M(\tau)$) by the model. We calculate the total number of users who retweeted the posts of users in $S(\tau)$ and $M(\tau)$ between time $[\tau^{'}, \tau^{'} + \Delta)$ where $\tau^{'} \!=\! \tau + g$, and 
$g \!=\! \{0, 2, 5, 8\}$ indicates the gap or number of stages after which we want to measure the impact of users (in the future). We considered different values of $\Delta \in \{1, 2, 3, 4, 5\}$ and Table \ref{comparison_impact_future} reports the average. We see that the impact of selected nodes (S) is greater than that of missed nodes (M) for \MethodName by a large margin. 
%
\begin{table}[!t]
\centering
\caption{Sum of retweets at $\tau + g$ for users selected at $\tau$}
\scalebox{0.73}
{
\hspace{-6mm}
\begin{tabular}{crrrrrrrr}
    \toprule
    \multirow{2}{*}[-0.5\dimexpr \aboverulesep + \belowrulesep + \cmidrulewidth]{{MODEL}}  & \multicolumn{2}{c}{$\tau^{'}=\tau + 0$}
    & \multicolumn{2}{c}{$\tau^{'}=\tau + 2$} & \multicolumn{2}{c}{$\tau^{'}=\tau + 5$} & \multicolumn{2}{c}{$\tau^{'}=\tau + 8$} \\
    \cmidrule(l){2-3} \cmidrule(l){4-5} \cmidrule(l){6-7} \cmidrule(l){8-9}
    & {S} & {M} & {S} & {M} & {S} & {M} & {S} & {M}  \\
    \midrule
    \rowcolor{Yellow}
DCPL & \textbf{1320.9} & \textbf{439.8} & \textbf{1289.1} & {393.2} & \textbf{912.5} & \textbf{352.4} & \textbf{853.3} & \textbf{208.2} \\ 
%RB-PF & 1382.8 & 452.2 & 1107.4 & 461.3 & 841.8 & \textbf{324.4} & 738.2 & \textbf{203.1} \\
\rowcolor{Yellow}
KM-R & 1181.2 & 546.6 & 875.6 & 381.2 & 667.4 & 419.6 & 473.2 & 366.8 \\
\rowcolor{Yellow}
KM-S & 1103.7 & 510.8 & 830.2 & \textbf{311.3} & 660.4 & 415.5 & 492.2 & 356.6 \\
\rowcolor{Yellow}
C-NET & 810.4 & 691.2 & 695.3 & 669.6 & 517.8 & 545.7 & 496.5 & 453.6 \\
\rowcolor{Yellow}
RND & 569.9 & 712.5 & 485.1 & 600.6 & 369.7 & 706.8 & 329.2 & 591.3 \\
\cmidrule{1-9}
\rowcolor{Green}
NC-PF & 1200.4 & 471.4 & 890.7 & 406.2 & 682.6 & 397.6 & 593.2 & 283.4 \\
\rowcolor{Green}
NC-TR & 1077.2 & 522.4 & 798.4 & 425.8 & 652.5 & 450.6 & 400.4 & 274.4 \\
\rowcolor{Green}
NC-N & 1022.5 & 498.8 & 735.1 & 378.3 & 621.8 & 378.3 & 528.3 & 297.6 \\ 
\bottomrule
\end{tabular}
}
\label{comparison_impact_future}
%\vspace{-1mm}
\end{table}

%Additionally, to evaluate how good are the clusters obtained 

\iffalse
%Due to space constraints, we describe the experiments for evaluating the clusters obtained, in Supplementary Material. 
We also evaluated the learned clusters\footnote{\label{supplemental}
Check \href{https://www.dropbox.com/s/ipqkhawu0joweel/Supplementary_Material_AAMAS_2020.pdf?dl=0}{Supplemental} for additional experiments on evaluation of clusters.} . %(see Supplemental).
%For the initial clusters, we observe that the users in the same clusters are more similar than those in different clusters, indicating ``good" clustering.
%We compare how well are the clusters aligned across multiple stages,
For C-PF, we compare the clusters across multiple stages, and observe the clusters to be indeed aligned. %that provide a proof of concept that C-PF is a able to ensure cluster alignment across different stages. 
We also %analyze the distribution of users 
analyze the movement of users between different clusters across multiple stages, in C-PF. We observe that users change clusters, justifying our approach to update cluster assignments dynamically. %to capture a change in user behavior as a result of the policy applied. 
%conjecture that there is a change in user behavior (features) due to the policy applied in the past, and it is important to capture this effect by updating the cluster assignments at each stage. We also conclude that users do not return back to the same clusters that they were in the previous stages
We compare the clusters obtained by different methods, and find that clusters of C-PF are most similar to those of KM-R, followed by KM-S, C-NET, RND, consistent with the decreasing %performance.
order of these methods, in terms of maximizing reward.
\fi

%the similarity between clusters decreases for KM-R, and C-NET, and the clusters of C-PF are least similar with those of RND, that is also consistent with the decreasing performance of these methods in maximizing the reward

%\subsubsection{Evaluation of Learned Clusters}

\iffalse
%We compare the clusters obtained by our model with those obtained by other baselines to study the gains in the performance of our method.
%
Fig. \ref{comparison_clusterings} shows contingency matrices comparing the clusters of C-PF with those obtained by other baselines. 
%We construct the contingency matrix as follows. 
%Specifically, the rows of the contingency matrix are ordered by the clusters in C-PF, and the columns are ordered by the clusters in the baseline method. The contingency matrix reports the intersection cardinality (number of common users) for every cluster pair from the two methods. %C-PF and RB-PF both dynamically update the cluster assignments with policy learning, whereas, KM-R (K-Means++ with reward-based features), C-NET (K-Means++ with network features) and RND (Random assignment of users to groups) assume fixed cluster assignments throughout. 
%Consider an $N \times N$ matrix $\boldsymbol{\mho}$, whose rows and columns represent the users ordered according to the cluster assignments such that the users belonging to the same clusters are next to each other
%
%
We see that 
%there is more similarity between clusters obtained by C-PF and RB-PF, 
the clusters obtained by C-PF are the most similar with those of KM-R, compared to other baselines. %This is consistent with RB-PF being the second best performing method after C-PF, in terms of maximizing the reward, as described in Sec. 4 in the main paper. 
And, the similarity between clusters decreases for KM-R, and C-NET, and the clusters of C-PF are least similar with those of RND, that is also consistent with the decreasing performance of these methods in in terms of maximizing the reward.
\fi

\iffalse
%\footref{supplemental}
We also conducted additional experiments
\footnote{We include the results for change in performance as a function of network size, relative importance of tweet and retweet activities, and the ratio of decay parameter for fake and true news diffusion, in the  \href{https://www.dropbox.com/s/ipqkhawu0joweel/Supplementary_Material_AAMAS_2020.pdf?dl=0}{Supplementary Material}.} to explore the effects of network characteristics on performance. 
They show that the performance of all methods decreases as network size $N$ decreases.
%We observe that %the relative importance of reward from tweet and retweet events 
%$\zeta$ (Eq. \ref{cumulative_reward}).  %on the performance of different methods. 
%with an increase in $\zeta$ (Eq. \ref{cumulative_reward}), i.e. decrease in the contribution by retweet events, there is a decrease in the performance of all methods. %, and C-PF is able to achieve high performance. 
\iffalse
We vary $\zeta$ and observe that retweets have more contribution in total reward, compared to tweets.
We vary the ratio of decay parameter for fake and true news, and observe a decrease in performance with increase in the ratio, due to presence of fewer true news events than fake, in later stages. 
\fi
\fi

%We also conducted additional experiments to 
We also explored the effects of network characteristics on performance. 
We down-sampled the datasets to compare the performance of different approaches as a function of network size $N$. Fig. \ref{rel_perf_vs_network_size} shows that the performance of all methods decreases with a decrease in $N$, and our method \MethodName outperforms for all network sizes considered.
%
%We down-sampled the datasets to compare the performance of different approaches as a function of network size (number of users). Fig. \ref{rel_perf_vs_network_size} shows, for all methods, the performance decreases with a decrease in the network size, and our method is able to outperform other baselines, for all network sizes.
%
%\vspace{-2mm}
\begin{figure}[!t] 
%\vspace{-3mm}
\hbox{
\subfloat[Twitter 2016]{\includegraphics[scale = 0.265]{figures/P_vs_semi_data_clustering_N_2016.png}}
\hspace{1ex}
\subfloat[Twitter 2015]{\includegraphics[scale = 0.265]{figures/P_vs_semi_data_clustering_N_2015.png}}
%\caption{Performance on Synthetic Data}
}
%\vspace{-2mm}
\caption{Relative Performance vs $N$}
%\vspace{-1mm}
\label{rel_perf_vs_network_size}
%\vspace{-2mm}
\end{figure}

%\subsubsection{Relative importance of Reward from Tweet and Retweet}
\iffalse
We vary $\zeta$, the relative importance of reward from tweet and retweet activities (Eq. 2 in Main paper). %as opposed to retweet events, $\zeta$ in Eq. \ref{cumulative_reward}. 
Fig. \ref{ratio_reward_weight} shows that with an increase in this ratio, that is a decrease in the contribution by retweet activities, the performance decreases for all methods. We also observe a relatively steep decrease in the performance after a ratio of 1 that corresponds to equal contribution of tweet and retweet activities in the reward. This suggests that retweet activities have a higher contribution in cumulative reward, and play more prominent in news diffusion than tweet activities,
%and retweet events play a more important role in news diffusion than tweet events, 
also consistent with \cite{vosoughi2018spread}. 
%
%
\begin{figure}[!t] 
%\vspace{-1mm}
\hbox{
\subfloat[Twitter 2016]{\includegraphics[scale = 0.265]{figures/P_vs_real_data_reward_ratio_weight_tweet_retweet_2016.png}}
\hspace{1ex}
\subfloat[Twitter 2015]{\includegraphics[scale = 0.265]{figures/P_vs_real_data_reward_ratio_weight_tweet_retweet_2015.png}}
%\caption{Performance on Synthetic Data}
}
%\vspace{-1mm}
\caption{Relative Importance of Tweets and Retweets}
\label{ratio_reward_weight}
%\vspace{-2mm}
\end{figure}
%

%\subsubsection{Effect of Kernel Decay Parameter}

%
\begin{figure}[!t]
%\vspace{-3mm}
\hbox{
\subfloat[Twitter 2016]{\includegraphics[scale = 0.275]{figures/P_vs_real_data_ratio_kernel_decay_tweets_2016.png}}
\hspace{1ex}
\subfloat[Twitter 2015]{\includegraphics[scale = 0.275]{figures/P_vs_real_data_ratio_kernel_decay_tweets_2015.png}}
%\caption{Performance on Synthetic Data}
}
%\vspace{-1mm}
\caption{Ratio of decay for tweeting true and fake news}
\label{ratio_kernel_decay_tweet}
\end{figure}
%
\begin{figure}[!t]
%\vspace{-2mm}
\hbox{
\subfloat[Twitter 2016]{\includegraphics[scale = 0.275]{figures/P_vs_real_data_ratio_kernel_decay_retweets_2016.png}}
\hspace{1ex}
\subfloat[Twitter 2015]{\includegraphics[scale = 0.275]{figures/P_vs_real_data_ratio_kernel_decay_retweets_2015.png}}
}
%\vspace{-1mm}
\caption{Ratio of decay for retweeting true and fake news}
\label{ratio_kernel_decay_retweet}
%\vspace{-4mm}
\end{figure}
%
%\vspace{1mm}
%\noindent \underline{\emph{Ratio of Kernel Decay Parameter}} %\mahak{Move this to Supplementary Material as similar graphs are in UAI Paper.}
Fig. \ref{ratio_kernel_decay_tweet} and \ref{ratio_kernel_decay_retweet}, respectively, show the change in performance with respect to the change in kernel decay parameter $\omega_{c,z}$ for tweeting ($z=\mathscr{T}$) and retweeting ($z=\mathscr{R}$) fake ($c=F$) and true ($c=T$) news. We keep the decay parameter for Tweet MHP fixed, while varying the decay parameter for Retweet MHP, and vice-versa.
As this ratio increases, the performance decreases, for both tweet and retweet activities. This is due to the fact that in the later stages, we have less true news events compared to fake news events. We mark the ratio corresponding to the settings described in Sec. \ref{learned_policy_eval}, with a vertical line.
We also observe a steeper decrease in performance for retweet activities, compared to tweet activities, implying that retweets have a major contribution in the reward, compared to tweets. 
%
\fi
%\section{ADDITIONAL EXPERIMENTS}

%\subsection{Experimental Settings}
%The number of clusters for each method are determined using BIC and WC-SSD, as described in Sec. \ref{choosing_num_clusters}.
%
%For C-PF, 
%the weights in computation of weighted centroid, 
%To compute the weighted centroids, we set $\varepsilon_1 = \varepsilon_2 = 0.5$ to assign equal importance to the centroids from previous and current stages.  We set the relative importance of reward from tweet activities compared to retweet activities $\zeta = 0.5$ (Equation 2, Main Paper).

%\vspace{-1mm}
%\subsection{EVALUATION OF LEARNED CLUSTERS}



\iffalse
%\vspace{-1mm}
\subsubsection{Evaluation of Initial Clusters for C-PF}

%To evaluate the initial clusters, %obtained using the Training Data, 
%we use the Silhoutte Coefficient (SC). %that is a widely used metric to evaluate unsupervised clustering. 
We obtain a higher Silhoutte Coefficient of 0.83 for the initial clusters, that indicates %that the clusters obtained are 
\textit{good} clustering. %obtained are ``good". 
%It is important to note that 
We use BIC and WC-SSD to select the number of clusters $\mathcal{G}$, and use %different measure, i.e. 
SC to evaluate the clusters, in order to ensure `fair' evaluation.
%make sure that the clusters we obtain are better, 
%instead of choosing k using a scree plot based on the different SC values for different k, 
%We believe that it is better to evaluate the clusters obtained, as output of clustering algorithm, with a measure different than the one used to choose $\mathcal{G}$ that is input to the algorithm. 
%
%We also evaluate the clusters using proximity matrix, and the details are provided in the Supplementary Material. 
%\mahak{Contingency matrix for comparing initial clusters with those of other baselines?}
%
We also evaluate the initial clusters %obtained using empirical reward based features in our method C-PF, 
using a proximity matrix that is computed based on the distance between users, ordered according to their clusters. 
\iffalse
Consider an $N \times N$ matrix $\boldsymbol{\mho}$, whose rows and columns represent the users ordered according to the cluster assignments such that the users belonging to the same clusters are next to each other. Specifically, the $N \times N$ matrix is represented as a $\mathcal{G} \times \mathcal{G}$ block matrix, whose rows and columns both are ordered by the users belonging to clusters, %in order $G_{g_1}, G_{g_2}, ..., G_{g_\mathcal{G}}$,
and the entry $\mho_{ij}$ represents the distance between users $i$ and $j$ that is $||\textbf{X}_{.,i} - \textbf{X}_{.,j}||_2$. 
\fi
Fig. \ref{proximity_matrix} represents a visualization of the proximity matrix. We see that the distance between users belonging to the same cluster is less (lighter shade) than that between users in different clusters (darker shade). Thus, clusters are well-separated, indicating a \textit{good} clustering of users. 
%
\begin{figure}[!t]
\vspace{-4mm}
\hbox{
\subfloat[Twitter 2016]{\includegraphics[scale = 0.35]{figures/proximity_matrix_2016.png}}
\hspace{2ex}
\subfloat[Twitter 2015]{\includegraphics[scale = 0.35]{figures/proximity_matrix_2015.png}}
%\caption{Performance on Synthetic Data}
}
\vspace{-2mm}
\caption{Proximity Matrix}
\label{proximity_matrix}
\end{figure}
\fi

%\vspace{-1mm}
%\subsubsection{Evaluation of Cluster Alignment}

%We check how well are the clusters at stage $k \geq 2$ aligned with those obtained at previous stage $k-1$. 
%To check how well are the clusters aligned for our proposed method C-PF, 
We also conducted additional experiments to assess the learned clusters. 
To evaluate cluster alignment across different stages, in our method \MethodName,
we compare the clusters at stage $k \geq 2$ with those obtained in the previous stage $k-1$. 
Figure \ref{cluster_alignment} shows the Adjusted Rand Index (ARI) and Normalized Mutual Information (NMI) scores. For stage 2, we compare with the initial clusters (Sec. \ref{clustering_features}) . %obtained using K-Means++ for stage 1.
%for clusters at stage k
%For the first stage, we compare against the initial clusters obtained at stage $0$ using k-means++. 
%
\begin{figure}[!t]
\centering %width=18cm
    {\includegraphics[width = 4cm]{figures/cluster_alignment.png}}
    \caption{Cluster Alignment Scores for DCPL}
    \label{cluster_alignment}
    %\mahak{update fig to map the section numbers later.}
\end{figure}
%
\iffalse
%
\begin{table}[!b]
%\vspace{-2mm}
\centering
\caption{ARI, NMI Scores of Clusters at Multiple Stages}
\mahak{change to figure. }
%\vspace{-2mm}
\scalebox{0.68}
{
\begin{tabular}{cccccccccc}
    \toprule
    \textbf{Stage} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{8} & \textbf{9} & \textbf{10} \\
    \midrule
    ARI &  0.907 & 0.907 & 0.919 & 0.927 & 0.920 & 0.916 & 0.930 & 0.949 & 0.944 \\
    NMI & 0.883 & 0.899 & 0.880 & 0.881 & 0.903 & 0.908 & 0.902 & 0.909 & 0.917 \\
    \bottomrule
\end{tabular}
}
\label{ARI_NMI_Scores}
%\vspace{-3mm} 
\end{table}
\fi
%
We see that both NMI and ARI scores are high, and this presents a proof of concept that clusters of \MethodName are indeed aligned.
%C-PF is able to ensure cluster alignment across different stages, 
%as required by the Neural Network to learn policy, across multiple stages, for input states ordered by clusters. %and epochs.
%the clusters at stage $k$ are aligned with those at stage $k-1$.
%for the alignment of the clusters at stage $k$ with those at previous stage $k-1$, and are approximately the same for all stages. 
%Thus, we can conclude that our algorithm based on weighted centroids helps to align the cluster assignment across stages, that is required by the policy function approximator to (map the policy for each cluster across epochs) learn the policy for each cluster.

%\vspace{-1mm}
%\subsubsection{User Movement between Clusters}

We %analyze the distribution of users 
studied the movement of users between different clusters across multiple stages. Fig. \ref{num_unique_clusters} and \ref{num_change_clusters}, respectively, show the distribution for the number of unique clusters that a user is in, and the number of times a user changes clusters, across all stages in the learning phase. %We see that majority of the users change clusters 4-6 times. 
We observe that users generally change clusters and do not return back to the same clusters. 
This shows that there is a change in user behavior (features) due to the policy applied in the past, justifying our approach to %it is important to capture this effect by  dynamically clustering users. %updating the cluster assignments at each stage.
update cluster assignments dynamically.
%We also conclude that users do not return back to the same clusters that they were in the previous stages. %before. %over time (stages).
%
\begin{figure}[!b]
%\vspace{-3mm}
\hbox{
\subfloat[Twitter 2016]{\includegraphics[scale = 0.23]{figures/num_unique_clusters_distribution_2016.png}}
\hspace{1ex}
\subfloat[Twitter 2015]{\includegraphics[scale = 0.23]{figures/num_unique_clusters_distribution_2015.png}}
%\caption{Performance on Synthetic Data}
}
%\vspace{-1mm}
\caption{Number of unique clusters across users}
\label{num_unique_clusters}
%\vspace{-1mm}
\end{figure}

\begin{figure}[!b]
%\vspace{-2mm}
\hbox{
\subfloat[Twitter 2016]{\includegraphics[scale = 0.23]{figures/num_change_clusters_distribution_2016.png}}
\hspace{1ex}
\subfloat[Twitter 2015]{\includegraphics[scale = 0.23]{figures/num_change_clusters_distribution_2015.png}}
%\caption{Performance on Synthetic Data}
}
%\vspace{-1mm}
\caption{Number of cluster transitions across stages}
\label{num_change_clusters}
%\vspace{-1mm}
\end{figure}
%

%\vspace{-1mm}
%\subsubsection{Comparison with clusters obtained from different baselines}

\begin{figure}[!b]
%\vspace{-3mm}
\hbox{
\subfloat[DCPL, KM-R]{\includegraphics[scale = 0.35]{figures/KM_R.png}}
\hspace{3ex}
\subfloat[DCPL, KM-S]{\includegraphics[scale = 0.35]{figures/KM_S.png}}
}
%\vspace{-1mm}
\hbox{
\subfloat[DCPL, C-NET]{\includegraphics[scale = 0.35]{figures/C_NET.png}}
\hspace{4ex}
\subfloat[DCPL, RND]{\includegraphics[scale = 0.35]{figures/RND.png}}
}
%\vspace{-1mm}
\caption{Contingency Matrix (DCPL vs other baselines)}
%\vspace{-5mm}
\label{comparison_clusterings}
\end{figure}
%
%We compare the clusters obtained by our model with those obtained by other baselines to study the gains in the performance of our method.
%
Fig. \ref{comparison_clusterings} shows contingency matrices comparing the clusters obtained by our method \MethodName with those obtained by other baselines. 
%We construct the contingency matrix as follows. 
%Specifically, the rows of the contingency matrix are ordered by the clusters in C-PF, and the columns are ordered by the clusters in the baseline method. The contingency matrix reports the intersection cardinality (number of common users) for every cluster pair from the two methods. %C-PF and RB-PF both dynamically update the cluster assignments with policy learning, whereas, KM-R (K-Means++ with reward-based features), C-NET (K-Means++ with network features) and RND (Random assignment of users to groups) assume fixed cluster assignments throughout. 
%Consider an $N \times N$ matrix $\boldsymbol{\mho}$, whose rows and columns represent the users ordered according to the cluster assignments such that the users belonging to the same clusters are next to each other
%
%
\iffalse
We see that 
%there is more similarity between clusters obtained by C-PF and RB-PF, 
the clusters obtained by C-PF are the most similar with those of KM-R. %, compared to other baselines. %This is consistent with RB-PF being the second best performing method after C-PF, in terms of maximizing the reward, as described in Sec. 4 in the main paper. 
And, the similarity between clusters decreases for KM-S, C-NET, clusters of C-PF are least similar with those of RND, that is also consistent with the decreasing performance of these methods in terms of maximizing the reward.
\fi
We compare the clusters obtained by different methods, and find that clusters of \MethodName are most similar to those of KM-R, followed by KM-S, C-NET, RND, consistent with the decreasing %performance.
order of these methods, in terms of maximizing reward.

\iffalse
\vspace{-2mm}
\subsection{Comparison of Tweet and Retweet Intensities}

Fig. \ref{comparison_base_intensity_tweet_retweet_2016} and \ref{comparison_base_intensity_tweet_retweet_2015} show a comparison of the distribution of respective base intensities, across all users.
We find that more number of users have higher retweet intensities for fake news, compared to true news. Also, the distribution of retweet intensities has more variance compared to tweet intensities. These observations are consistent with \cite{vosoughi2018spread}, and indicate that it is important to consider separate processes for tweet and retweet events, as mentioned in Sec. 1 in main paper. 

%
\begin{figure}[!t]
%\hbox{
\vspace{-3mm}
\subfloat[Fake News]{\includegraphics[scale = 0.23]{figures/tweet_retweet_base_intensity_2016_density_distribution_fake_news.png}}
\hspace{1ex}
\subfloat[True News]{\includegraphics[scale = 0.23]{figures/tweet_retweet_base_intensity_2016_density_distribution_true_news.png}}
%\caption{Performance on Synthetic Data}
%}
\vspace{-2mm}
\caption{Tweet and Retweet Intensities for Twitter 2016}
\label{comparison_base_intensity_tweet_retweet_2016}
\vspace{-4mm}
\end{figure}

\begin{figure}[!t]
\hbox{
\vspace{-3mm}
\subfloat[Fake News]{\includegraphics[scale = 0.23]{figures/tweet_retweet_base_intensity_2015_density_distribution_fake_news.png}}
\hspace{1ex}
\subfloat[True News]{\includegraphics[scale = 0.23]{figures/tweet_retweet_base_intensity_2015_density_distribution_true_news.png}}
%\caption{Performance on Synthetic Data}
}
%\vspace{-1mm}
\caption{Tweet and Retweet Intensities for Twitter 2015}
\label{comparison_base_intensity_tweet_retweet_2015}
\vspace{-4mm}
\end{figure}
%
\fi



==> ARXIV_Dynamic Cluster-based Policy Learning for Social RL/06-conclusion.tex <==
\section{CONCLUSION} \label{conclusion}
%Modeling negative reactions: future work. 

%In this paper, we defined the problem of {\em Social Reinforcement Learning}, where the goal is to learn RL models in domains with a large number of agents with complex interactions among them, in both collaborative and adversarial settings. We described a number of challenges for Social RL methods, and proposed ways to address those by utilizing properties of the social network structure, agent interactions.

%Specifically, Social RL is challenging due to the fact that models need to capture ${\sim}N^2$ dependencies between agents with only sparse (i.e., $O(N)$) interactions. We note that the social network structure and agent similarities can be exploited to overcome problems of high dimensionality, sparsity, non-stationarity, and partial observability, by obtaining a compact model that better captures agent dependencies and is much more efficient to solve. For example, we can cluster similar users and share information among them to overcome interaction sparsity and effectively capture ${\sim}N^2$ dependencies with reduced computational cost. 

This paper outlines a Dynamic Cluster-based Policy Learning approach, DCPL, for social reinforcement learning that considers domains with a large number of agents with complex interactions among them. Our approach helps to address the challenges of high-dimensionality and sparsity by exploiting the social network structure and agent similarities to obtain a compact model that better captures agent dependencies and is much more efficient to solve. 

Specifically, we use latent features to cluster users based on their payoff and contribution, and aggregate the interactions of similar agents. We learn policies for the clusters, and then easily use those to obtain actions for users based on their variability from the cluster. This allows for efficiently learning personalized policies, while still considering all agent dependencies given large number of users. Moreover, the number of effective policies is greatly reduced, thus lowering the computational complexity. 
%This results in a great reduction in the number of policies to be learnt, while still allowing personalized agent policies at the same time. 
Clustering adds a discriminative power to our model to differentiate between different types of users (and their activities), which helps in efficient and effective allocation of incentives among users under fixed budget.
Experiments show that dynamic clustering of users %along with policy learning 
helps the model to quickly learn better policy estimates, allowing it to outperform other static clustering-based and non-clustering alternatives. 

\iffalse
This paper outlines a dynamic cluster-based policy learning approach to address the challenges of high-dimensionality and sparsity in Social RL problems.  
%by exploiting the social network structure and agent correlations to obtain a compact model that better captures agent dependencies and is much more efficient to solve. %Specifically, we use latent features to cluster users 
Specifically, we exploit the social network structure and agent correlations to cluster users
based on their payoff and contribution, and aggregate the interactions of similar agents, for a more compact model. We learn policies for the clusters, and then use those to obtain actions for users based on their variability from the cluster, which enables efficient learning of personalized policies. %Moreover, the number of effective policies is greatly reduced, thus lowering the computational complexity. 
%This results in a great reduction in the number of policies to be learnt, while still allowing personalized agent policies at the same time. 
%Clustering adds a discriminative power to our model to differentiate between different types of users (and their activities), which helps in efficient and effective allocation of incentives among users under fixed budget.
Experiments show that dynamic clustering of users %along with policy learning
helps the model to learn quickly and outperform other static clustering-based and non-clustering alternatives.

\fi

